PVASS Reachability is Decidable

Reachability in pushdown vector addition systems with states (PVASS) is among the longest standing open problems in Theoretical Computer Science. We show that the problem is decidable in full generality. Our decision procedure is similar in spirit to the KLMST algorithm for VASS reachability, but works over objects that support an elaborate form of procedure summarization as known from pushdown reachability.

==> coverability_ek.tex <==
\section{Coverability}\label{Section:Coverability}

% Problem 1, Need for assistance: Treating lower grammars as terminals, in the sense that they are blackboxes that produce certain outcome configurations, given an input configuration.
% Problem 2, Need for assistance: Consider only one side, you need the exit value of a call subtree to move on to the next branch. 
% Insight: Close a branch upon a pump by calling perfect, this has to occur because of Jerome.

% Problem 3, Need for assistance: We need markings on both sides to discover pumping. 
% Insight: We can use a perf-call to find the downward closures of the reverse runs. If the non-developped side has strictly-less counters, then this is 
% a perf-call of lower dimension. 

% Caveat: The case where the number of concrete counters are equal.
% Insight: This case only naturally occurs when, ignoring the markings, the solution space is bounded. This boundedness allows us to finitely guess derivations, until one of the concrete counters is pumped to omega.


% Problem 4, Termination vs. Coverability: Termination is happy with a repeatable derivation that has no effect on the left side of the pump, we are not.
% Insight: There is another type of pumping that can occur. In the situations considered here, these pumps are guaranteed to eventually exist.
% Store them as trees witnessing said outcome values.

In \Cref{Section:Decomposition}, we have promised to handle the decomposition for the case where \perfectnesspumping or \perfectnesspumpingint do not hold.
%
Indeed, we keep our promise.
%
We organise this section into five subsections.
%
First, in \Cref{Section:WitnessingGrammars}, we study the coverability grammar, which can be seen as an extention of the Karp-Miller graph to the setting of NGVAS.
%
We discuss the fact that we can use the coverability grammar to determine whether \perfectnesspumping holds, and to provide a decomposition in the case that \perfectnesspumping does not hold.
%
The \Cref{Section:EffectiveWitnessGrammar} takes a closer look at the computability of the coverability grammar. 
%
Computing the coverability grammar is the goal of the rest of the section.
%
We observe that to compute the coverability grammar in the case of a linear NGVAS, we only need to compute the set of markings that a terminal can cover at the output, when given an input.
%
This can be handled by the reliability assumption on $\perfect$.
%
We handle the condition \perfectnesspumpingint similarly.
%
However, to compute the coverability grammar in the case of a non-linear NGVAS, we need to
compute the set of coverable output markings for all runs derivable from non-terminals.
%
Here, we employ an algorithm that searches for derivation trees that witness these coverable markings.
%
We take \Cref{Section:WitnessTrees} to develop the basic object we work with in this search, the witness trees.
%
The algorithm needs to work with a special class of witness trees called the useful witness trees in order to be complete.
%
These details are handled in \Cref{Section:UsefulWitnessTrees}.

\subsection{Coverability Grammar}\label{Section:WitnessingGrammars}

For the rest of \Cref{Section:Coverability}, fix $\anngvas$ to be an arbitrary NGVAS with $d$ counters.
%
When we refer to the components of $\anngvas$, we ommit the membership operator.
%
For example we write $\nonterms$, instead of $\anngvas.\nonterms$.

Towards computing the coverability grammar, we define $\postfuncN{\anngvas}:\Nomega^{d}\times(\nonterms\cup\terms)\to\powof{\Nomega^{d}}$ and $\prefuncN{\anngvas}:\Nomega^{d}\times(\nonterms\cup\terms)\to\powof{\Nomega^{d}}$ that return the ideal decomposition of the coverable markings.
%
\begin{align*}
    \prefuncNof{\anngvas}{\amarking, \asymbol}&=\iddecompof{\downclsof{\setcond{\amarkingp\in\Nomega}{\amarking\fires{\arun}\amarkingp,\; \arun\in\runsof{\asymbol}}}}\\
    \postfuncNof{\anngvas}{\amarking, \asymbol}&=\iddecompof{\downclsof{\setcond{\amarkingp\in\Nomega}{\amarkingp\fires{\arun}\amarking,\; \arun\in\runsof{\asymbol}}}}
\end{align*}
%
In this section, we use 
%
$$\runsof{\anonterm}=\setcond{\arun\in\runsof{\asentform}}{\asentform\in\terms^{*},\;\anonterm\to^{*}\asentform\text{ in }\anngvas}.$$
%
as a shorthand, where $\anonterm\in\nonterms$. 
%
We are now ready to define the coverability grammar.\\

\noindent\textit{Construction.}
A coverability grammar of $\anngvas$ is the grammar $\wtgrammar=(\wtnonterminals, \wtedges, \wtstartnt, \terms)$, where $\wtnonterminals\subseteq\Nomega^{d}\times\nonterms\times\Nomega^{d}$, and $\wtstartnt=(\acontextin, \startnonterm, \acontextout)$.
%
The construction of the external coverability grammar starts with $\wtnonterminals=\set{\wtstartnt}$, and $\wtedges=\emptyset$.
%
The algorithm iteratively extends the grammar by exploring the productions rules of $\anngvas$ until a fixed point is reached.
%
For each unexplored $(\amarking, \anonterm, \amarkingp)\in\wtnonterminals$ and rule $\anonterm\to\asymbol.\asymbolp\in \prods$, we compute the sets $K=\postfuncNof{\anngvas}{ \amarking, \asymbol}$, and $L=\prefuncNof{\anngvas}{\amarkingp, \asymbolp}$.
%
For each $\amarking_{\postfunc}\in K$ and $\amarkingp_{\prefunc}\in L$, we intend to construct annotations $\asymbol_{\annotated}$ and $\asymbolp_{\annotated}$ of $\asymbol$ and $\asymbolp$, and add the rule $(\amarking, \anonterm, \amarkingp)\to\asymbol_{\annotated}.\asymbolp_{\annotated}$ to $\wtedges$.
%
If one of $\asymbol$ or $\asymbolp$ is a terminal, then we do not annotate.
%
Assume that $\asymbol$ is indeed a non-terminal.
%
In order to obtain $\asymbol_{\annotated}$, we start with $(\amarking, \asymbolp, \amarkingp_{\prefunc})$ at hand.
%
We check whether a $(\amarking', \asymbolp, \amarkingpp')\in\wtnonterminals$ exists with $(\amarking_{\lesstag}, \amarkingpp_{\lesstag})<(\amarking, \amarkingp_{\prefunc})$, that can call $(\amarking, \anonterm, \amarkingp)$.
%
If not, then we let $\asymbol_{\annotated}=(\amarking, \asymbolp, \amarkingp_{\prefunc})$.
%
If there is such a $(\amarking_{\lesstag}, \asymbolp, \amarkingpp_{\lesstag})\in\wtnonterminals$, then we let $\asymbol_{\annotated}=(\amarking_{\omega}, \asymbolp, \amarkingpp_{\omega})$ where $(\amarking_{\omega}, \amarkingp_{\omega})$ is the vector with $(\amarking_{\omega}, \amarkingpp_{\omega})[i]=(\amarking, \amarkingp_{\prefunc})[i]=(\amarking_{\lesstag}, \amarkingpp_{\lesstag})[i]$ or $(\amarking_{\omega}, \amarkingpp_{\omega})[i]=\omega$ for all $i$.
%
The annotation $\asymbolp_{\annotated}$ is constructed similarly, but instead of starting with $(\amarking, \asymbolp, \amarkingp_{\prefunc})$, we start with $(\amarking_{\postfunc}, \asymbolp, \amarkingp)$.
%
An important detail is that, even though we write $\wtnonterminals\subseteq\Nomega^{d}\times\nonterms\times\Nomega^{d}$, we allow for multiple copies with the same annotation, just as in the construction of a coverability graph for plain VASS.
%
If no symbol with the same annotation as $\asymbol_{\annotated}$ or $\asymbolp_{\annotated}$ can call $\anonterm$, we add the respective symbol as a fresh symbol, and do not reference an already existing symbol in the newly constructed rule.


By the same argument to the construction of the Karp-Miller graph, we observe that the construction terminates.
%
The proof has been moved to the appendix.

\begin{lemma}\label{Lemma:WitnessGrammarTermination}
    The construction of $\wtgrammar$ terminates.
\end{lemma}

The coverability grammar has further similarities with the Karp-Miller graph.
%
The existence of an pump as described in \perfectnesspumping is intimately related to the external coverability grammar.
%
The proof has been moved to the appendix.

\begin{comment}
    In this section, we show that $\extcovnl$, as specified in \Cref{Lemma:ExtCovSpec}, is realizable via subcalls to certain coverability-related queries.
    %
    We break the proof down into two propositions, \Cref{Proposition:WitnessGrammarProp}, and \Cref{Proposition:WitnessGrammarEff}.
    %
    The backbone of the algorithm is the construction of \emph{external coverability grammar} for an NGVAS.
    %
    A \emph{external coverability grammar} for an NGVAS $\anngvas$ is the context-free grammar
    $\wtgrammar=(\wtnonterminals, \wtedges, \wtalph)$, constructed by the external coverability algorithm, where $\wtnonterminals\subseteq\natomega\times\anngvas.\nonterminals\times\natomega$, and $\wtalph\subseteq\natomega\times\anngvas.\analph\times\natomega$
    annotations of non-terminals and terminals of $\anngvas$.
    %
    We will cover the construction shortly.
    %
    Same as a coverability graph for plain VASS, this structure is intended to witness the existence of a external coverability sequence if there is one, and expose a kind of boundedness if the sequence is not present.
    %
    The boundedness then yields an NGVAS with lower rank.
    %
    The first proposition, \Cref{Proposition:WitnessGrammarProp}, formalizes this notion.
\end{comment}


\begin{lemma}\label{Lemma:WitnessGrammarProp}
    Let $\wtgrammar=(\wtnonterminals, \wtedges, \wtstartnt, \terms)$ be the coverability grammar of $\anngvas$.
    %
    We have $(\inof{\startnonterm}, \startnonterm, \outof{\startnonterm})\in\wtnonterminals$, if and only if $\anngvas$ has a pumping sequence.
\end{lemma}

Given the coverability graph of $\anngvas$, we can compute a decomposition if \perfectnesspumping does not hold for $\anngvas$.

\begin{proposition}\label{Proposition:WitnessGrammarDecomp}
    Let $\wtgrammar=(\wtnonterminals, \wtedges, \wtstartnt, \terms)$ be the coverability grammar of $\anngvas$, and let \perfectnesspumping not hold for $\anngvas$.
    %
    We can compute a decomposition $\adecomp$ of $\anngvas$ from $\wtgrammar$, that is elementary in the size of $\wtgrammar$.
    %
    Furthermore, for all $\anngvas'\in\adecomp$, we have $\srankof{\anngvas'}<\srankof{\anngvas''}$ for any NGVAS $\anngvas''$ with the same terminals, boundedness information, and index.
\end{proposition}

We give an overview of the construction for \Cref{Proposition:WitnessGrammarDecomp}.
%
The details can be found in the appendix.
%
To obtain a decomposition, we consider the strongly connected components of $\wtgrammar$.
%
A strongly connected component of $\wtgrammar$ corresponds to an NGVAS, with (sequences of) lower strongly connected components as its children.
%
Here, the main challenge is the difference between the form of $\wtgrammar$ and the definition of an NGVAS.
%
Namely the input and output markings of a non-terminal in $\wtgrammar$ may have sets of $\omega$ counters that are unrelated to each other.
%
However, if we only consider either the input or the output, the set of markings that are $\omega$ is the same across a strongly connected component of $\wtgrammar$.
%
Also, since \perfectnesspumping does not hold, any non-terminal in $\wtgrammar$ has at least one counter marked concrete.
%
These facts lead to a main branch, where to one direction of this main branch, a counter remains bounded (on the exits of lower strongly connected components), and in the other, we only generate non-terminals that coresspond to lower strongly connected components.
%
This allows us to construct an NGVAS for the strongly connected component that has more bounded counters, or linearity than $\anngvas$.

\ek{Maybe a picture?}

\begin{comment}
    The external coverability, as a concept, combines the forward- and backward-covering sequences in a plain VASS.
    %
    For this reason, the construction of the external coverability grammar relies on calls $\postfunc$ and $\prefunc$ that determine maximally coverable markings in a given direction from a given marking.
    %
    We formulate these calls as restricted reachability calls, $\postfunc:\ngvas\partto\finpowof{\natomega}$, $\prefunc:\ngvas\partto\finpowof{\natomega}$
    %
    Similarly to the $\perfect$ and $\extcovnl$, we define a notion of reliability.
    %
    Let $\anngvas$ be an NGVAS.
    %
    We say that $\postfunc$ is reliable for $\anngvas$, if, given $\anngvas.\outmarking=\anngvas.\outfuncof{\anngvas.\startnt}$, the function $\postfunc:\anngvas\partto\finpowof{\natomega}$ terminates with 
    %
    $$\downarrow\postfunc(\anngvas)=\downarrow\setcond{\amarkingp}{\anngvas.\inmarking\fires{\aword}\amarkingp,\aword\in\natlangof{\anngvas}}.$$
    %
    Similarly, we say that $\prefunc$ is reliable for $\anngvas$, if, given $\anngvas.\inmarking=\anngvas.\infuncof{\anngvas.\startnt}$, then the function $\prefunc:\anngvas\partto\finpowof{\natomega}$ terminates with 
    %
    $$\downarrow\prefunc(\anngvas)=\downarrow\setcond{\amarkingp}{\anngvas.\outmarking\backfires{\aword}\amarkingp,\aword\in\natlangof{\anngvas}}.$$


    In the following, we often use $\postfunc$ and $\prefunc$ to find the maximal output values obtained while exiting a non-terminal $\anonterminal\in\anngvas.\nonterminals$, starting from various markings.
    %
    To ease the notation, we write $\postfunc(\amarking, \anonterminal)$ and $\prefunc(\amarkingp, \anonterminal)$ to denote $\postfunc(\anngvas_{(\amarking, \anonterminal, \anngvas.\outfunc(\anonterminal))})$ and $\prefunc(\anngvas_{(\anngvas.\infunc(\anonterminal), \anonterminal, \amarkingp)})$ where $\anngvas$ is an NGVAS, $\anonterminal\in\anngvas.\nonterminals$, $\amarking\omegaleq\anngvas.\infuncof{\anonterminal}$, and $\amarkingp\omegaleq\anngvas.\outfuncof{\anonterminal}$.
    %
    Similarly, we write $\postfunc(\amarking, \aterminal)$ and $\prefunc(\amarking, \aterminal)$ to denote $\postfunc$ and $\prefunc$ calls on the NGVAS obtained from $\aterminal\in\anngvas.\analph$ by replacing the input resp. output marking with the $\omegaleq$-specialization $\amarking$.
    %
    We move on to the construction of the external coverability grammar.
\end{comment}


\subsection{Computing the coverability grammar}\label{Section:EffectiveWitnessGrammar}

The decomposition we get from \Cref{Proposition:WitnessGrammarDecomp} is exactly the result of $\extcovnl$ ($\extcovlin$) calls.
%
The main consequence of this proposition is the following.
%
If we show that we can compute $\postfuncN{\anngvas}$ and $\prefuncN{\anngvas}$ for an NGVAS $\anngvas$, then we can compute $\extcovnlof{\anngvas}$.

\begin{lemma}\label{Lemma:ExtCovBase}
    Let $\anngvasp$ be an NGVAS.
    %
    If $\postfuncNof{\anngvasp}{\amarkingin, \asymbol}$ and $\prefuncNof{\anngvasp}{\amarkingout, \asymbol}$ can be computed for $\asymbol\in\anngvasp.\nonterms\cup\anngvasp.\terms$ and $\amarkingin, \amarkingout\in\Nomega^{d}$ with $\omegaof{\acontextin}\subseteq\omegaof{\amarkingin}$, $\omegaof{\acontextout}\subseteq\omegaof{\amarkingout}$, $\amarkingin\sqsubseteq\inof{\anonterm}$, and $\amarkingout\sqsubseteq\outof{\anonterm}$, then $\extcovnlof{\anngvasp}$ is computable.
\end{lemma}
%
This is because we only need $\postfuncN{\anngvas}$ and $\prefuncN{\anngvas}$ to compute $\wtgrammar$.
%
In the case of linear NGVAS, we can deduce a stronger conclusion.
%
Notice that we only use the values of $\postfuncNof{\anngvas}{\amarking, \anonterm}$ or $\prefuncNof{\anngvas}{\amarking, \anonterm}$ for some $\anonterm\in\nonterms$ in the construction of $\wtgrammar$ if a production rule produces two non-terminals.
%
Since this does not happen in the linear case, we only need to compute the $\postfunc$ and $\prefunc$ functions for terminals.

\begin{lemma}\label{Lemma:LinCovBase}
    Let $\anngvasp$ be a linear NGVAS.
    %
    If $\postfuncNof{\anngvasp}{\amarkingin, \aterm}$ and $\prefuncNof{\anngvasp}{ \amarkingout, \aterm}$ can be computed for $\aterm\in\terms$ and $\amarkingin, \amarkingout\in\Nomega^{d}$ with $\omegaof{\anngvasp.\acontextin}\subseteq\omegaof{\amarkingin}$, $\omegaof{\anngvasp.\acontextout}\subseteq\omegaof{\amarkingout}$, $\amarkingin\sqsubseteq\inof{\aterm}$, and $\amarkingout\sqsubseteq\outof{\aterm}$, then $\extcovnlof{\anngvasp}$ is computable.
\end{lemma}

For the internal pumping sequence in \Cref{Lemma:LinCovSpec}, we exchange the production directions, i.e. from $\anonterm\to\aterm.\anontermp$, to $\anontermp\to\anonterm.\aterm$, in order to get the needed decomposition.


We observe that $\postfuncN{\anngvas}$ and $\prefuncN{\anngvas}$ are already computable for $\aterm\in\terms$ using the common premise of \Cref{Lemma:ExtCovSpec} and \Cref{Lemma:LinCovSpec}.
%
This and \Cref{Lemma:LinCovBase} already imply \Cref{Lemma:LinCovSpec}.

\begin{lemma}\label{Lemma:CovComputableForTerminals}
    Let $\perfect$ be reliable up to $\rankof{\anngvas}$, and let $\aterm\in\terms$.
    %
    Further let $\amarkingin, \amarkingout\in\Nomega^{d}$ with $\omegaof{\acontextin}\subseteq\omegaof{\amarkingin}$, $\omegaof{\acontextout}\subseteq\omegaof{\amarkingout}$, $\amarkingin\sqsubseteq\inof{\aterm}$, and $\amarkingout\sqsubseteq\outof{\aterm}$.
    %
    Then $\postfuncNof{\anngvas}{\amarkingin, \aterm}$ and $\prefuncNof{\anngvas}{\amarkingout, \aterm}$ are computable.
\end{lemma}

The proof of the \Cref{Lemma:CovComputableForTerminals} relies on the fact that if the context information of an NGVAS is made more concrete, then the rank is guaranteed to go down.
%
Since the rank of a child of $\anngvas$ is less than $\rankof{\anngvas}$, the reliability of $\perfect$ applies.
%
A detailed argument can be found in the appendix.


The non-linear case is more involved.
%
As we mentioned, in this case we perform a search for witnesses.
%
We develop said search throughout the rest of \Cref{Section:Coverability}.
%
We use $\witnessfuncN{\anngvas}$ to denote the witness search procedure for $\postfuncN{\anngvas}$, and $\bckwitnessfuncN{\anngvas}$ to denote the witness search procedure for $\prefuncN{\anngvas}$.

\begin{proposition}\label{Proposition:MainCovProp}
    Let $\anngvas$ be a non-linear, and fulfill the perfectness conditions \perfectnesssolnospace, \perfectnesscountersnospace, \perfectnessprodsnospace, \perfectnesschildperiodsnospace, \perfectnesschildrennospace, and let $\anonterm\in\nonterms$. 
    %
    Further let $\perfect$ be reliable up to rank $\rankof{\anngvas}$.
    %
    Then for $\witnessfuncN{\anngvas}$ and $\bckwitnessfuncN{\anngvas}$ we have the termination values  
    \begin{align*}
        \downclsof{\witnessfuncNof{\anngvas}{\anonterm, \amarkingin}}&=\downclsof{\postfuncNof{\anngvas}{\anonterm, \amarkingin}}\\
        \downclsof{\bckwitnessfuncNof{\anngvas}{\anonterm, \amarkingout}}&=\downclsof{\prefuncNof{\anngvas}{\anonterm, \amarkingout}}
    \end{align*}
    for $\amarkingin, \amarkingout\in\Nomega^{d}$ with $\omegaof{\acontextin}\subseteq\omegaof{\amarkingin}$, $\omegaof{\acontextout}\subseteq\omegaof{\amarkingout}$, $\amarkingin\sqsubseteq\inof{\anonterm}$, and $\amarkingout\sqsubseteq\outof{\anonterm}$.
\end{proposition}

The main challenge we address while implementing $\witnessfuncN{\anngvas}$ is termination.
% 
If we search naively, we do not know when to terminate the search for witness trees.
%
The solution is to restrict their complexity, while maintaining completeness.
%
To this end, the $\witnessfuncN{\anngvas}$ algorithm exploits the iteration lemma on key occasions.
%
Note that we are unable to require possessing a pumping sequence \perfectnesspumping, which would allow us to apply the \Cref{TheoremIterationLemmaNonLinearOverview} directly.
%
The reason is the following.
%
As we observed in \Cref{Section:WitnessingGrammars}, we already rely on $\postfuncN{\anngvas}/\prefuncN{\anngvas}$ in the decomposition case for \perfectnesspumping.
%
So, expecting \perfectnesspumping would amount to circular reasoning.
%
We get around this problem in two ways.
%
First, we underapproximate the set of markings from which there is a pumping sequence and use this information to apply \Cref{TheoremIterationLemmaNonLinearOverview}.
%
Second, we check a version of \perfectnesspumping that depends on strictly less counters, and apply a simpler decomposition if it does not hold.
%
This allows us to use the reliability of $\perfect$.
%
We show that for large enough trees, one of these conditions will hold, and we will not need to explore further.


Before we move on to \Cref{Section:WitnessTrees}, we develop some notation.
%
For the rest of the section, assume $\anngvas$ and $\amarkingin$ to be as described in \Cref{Proposition:MainCovProp}, and let $\anonterminalin\in\nonterms$.
%
We write $\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \amarkingp}$ to denote the NGVAS obtained from $\anngvas$ by replacing the initial symbol with $\anonterm$, and the context information with $(\N^{d}, (\amarking, \amarkingp))$.
%
Let $\omegaincount=\omegaof{\amarkingin}$, and let $\omegaoutcount$ be the set of output markings in the support of $\homchareq{\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \outof{\anonterm}}}$ for $\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \outof{\anonterm}}$.
%
Further, let $\concincount=[1, d]\setminus\omegaincount$, and $\concoutcount=[1, d]\setminus\omegaoutcount$ be the complements of these sets.
%
In the following, we show \Cref{Proposition:MainCovProp} and discuss $\witnessfuncN{\anngvas}$ in detail.
%
To prove \Cref{Proposition:MainCovProp} for $\bckwitnessfuncN{\anngvas}$, one only needs to exchange directions.

\subsection{Witness Trees}\label{Section:WitnessTrees}

As we stated, the search of a witness tree is the core of our algorithm.
%
In this section, we make the notion of witness trees concrete, and discuss their basic properties.
%
Intuitively, a witness tree is a marked parse tree in the grammar of $\anngvas$, whose leaves are marked soundly wrt. the reachability relation.
%
To make this precise, we write $\amarking\fires{K}\amarkingp$ for a set $K\subseteq\updates^{*}$, to denote the existence of $\amarkingp_{0}, \amarkingp_{1},\ldots \in\Nomega^{d}$ and $\arun_{0}, \arun_{1},\ldots \in K$ with $\amarking\fires{\arun_{i}}\amarkingp_{i}$ for all $i\in\N$, and $\lim_{i\in\N}\amarkingp_{i}=\amarkingp$.
%
The witness trees also allow for a certain type of pumping we will discuss shortly.
%
Formally, a \emph{witness tree} is a labeled tree $\atree=(\atree, \nodemarking)$ with a labeling $\nodemarking:\atree\to\Nomega^{d}\times(\nonterms\cup\terms)\times\Nomega^{d}$ where the following hold.
%
We write $\atree.\rootlabel$ for $\nodemarkingof{\anode}$ where $\anode$ is the root of $\atree$, and $\atree.\rootlabel=(\atree.\inlabel, \atree.\symlabel, \atree.\outlabel)$ to denote the respective components.
%


\begin{itemize}
    \item For any node label $(\amarking, \asymbol, \amarkingp)$, we have $\omegaof{\amarking}\subseteq\omegaof{\amarkingp}$.
    \item For any $\anode$ with children $\anodep,\anodepp$ in $\atree$, we have $\nodemarkingof{\anode}=(\amarking, \anonterm, \amarkingp)$, $\nodemarkingof{\anodep}=(\amarking, \asymbol, \amarkingpp)$,  $\nodemarkingof{\anodepp}=(\amarkingpp, \asymbolp, \amarkingp')$, $\amarkingp'\sqsubseteq\amarkingp$, and $\anonterm\to\asymbol.\asymbolp\in\prods$.
    \item For any leaf $\aleaf\in\atree$, if $\nodemarkingof{\aleaf}=(\amarking,\asymbol,\amarkingp)$ we have $\amarking\fires{\runsof{\asymbol}}\amarkingp$.
    \item Let $\atreep$ a subtree of $\atree$.
        %
        Then, $\atreep\sqsubseteq\pumpingof{\atreep}.\outlabel$.
\end{itemize}

The first condition states that $\atree$ is a parse tree in the grammar of $\anngvas$.
%
The next condition states that the leaves are marked with markings consistent with the reachability relation of the child NGVAS resp. the sequence of child NGVAS derivable from a non-terminal.
%
The final condition concerns the type of pumping that we are yet to discuss, denoted by $\pumpingof{\atreep}$.
%
Intutively, $\pumpingof{\atreep}$ is $\atreep$, where the output marking of the root node has been pumped as much as possible using the so called side-pumps present in the tree $\atreep$.
%
Formally, $\pumpingof{\atreep}$ is the same as $\atreep$ up to the output marking $\pumpingof{\atreep}.\outlabel$.
%   
For the output marking, we have $\pumpingof{\atreep}\sqsubseteq\amarkingp$, where $\nodemarkingof{\anode}=(\amarking, \anode, \amarkingp)$, and $\anode$ the rightmost child node of the root in $\atreep$.
%
Furthermore, $\pumpingof{\atreep}.\outlabel[i]=\omega$, if there is a node $\anode$ in $\atreep$ where $\nodemarkingof{\anodep}=(\atreep.\inlabel, \anonterm, \amarkingp')$, $\amarkingp'\leq\amarkingp$, and $\amarkingp'[i]<\amarkingp[i]$.
%
The $\omega$'s are justified as follows.
%
If one finds such a node $\anode$ in $\atreep$, then it means that there is a context from the root to $\anode$ that (i) produces a sequence with $0$ effect on the left side that is enabled from $\atreep.\inlabel$, and (ii) generates a sequence with strictly positive effect that is enabled from $\amarkingp'$ on the right side.
%
This means that repeating this context results in enabled sequences, and it does not change the markings on the input side, while increasing the markings for the output side.

\ek{It would be fitting to have a picture for the side-pump here.}

We argue that the output values witnessed by the witness trees are indeed sound.
%
The key observation here is that the soundness of side-pumping.

\begin{lemma}\label{Lemma:WitnessTreeSound}
    Let $\atree$ be a witness tree with $\atree.\symlabel\in\nonterms$.
    %
    Then we have $\atree.\inlabel\fires{\runsof{\atree.\symlabel}}\atree.\outlabel$.
\end{lemma}

The argument for completeness (with respect to coverable concrete markings) is simpler, since witness trees admit all relevant marked derivation trees (up to collapsing the derivation trees of the child NGVAS).

\begin{lemma}\label{Lemma:WitnessTreeComplete}
    If $\amarking\fires{\runsof{\anonterm}}\amarkingp$ for some $\amarking, \amarkingp\in\Nomega^{d}$ and $\anonterm\in\nonterms$ with $\omegaof{\amarking}=\omegaof{\amarkingp}$, then there is a witness tree $\atree$ with $\atree.\inlabel=\amarking$ and $\atree.\outlabel=\amarkingp$.
\end{lemma}

Even though witness trees are sound and complete, they are hardly useable for algorithmic purposes in this form.
%
We address this in the next section, where we define a restricted class of witness trees.

\subsection{Searching Useful Witness Trees}\label{Section:UsefulWitnessTrees}

In this section, we define useful witness trees, a restricted form of witness tree that allows for an algorithmic treatment.
%
A key assumption assures that we do not lose any output marking while moving from witness trees to useful witness trees.
%
We argue that given any depth, we can construct all possible useful witness trees up to this depth.
%
Finally, we prove that we can detect a maximal depth, beyond which we do not find any new useful witness trees.
%
This implies an algorithm: we construct all the useful witness trees up to this depth, and return the witnessed markings, proving \Cref{Proposition:MainCovProp}.

A fundamental ingredient in the definition of useful witness trees is the following observation.
%
If we can decompose $\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \amarkingp}$ in any way that lowers the rank below that of $\anngvas$, then we can use the reliability of $\perfect$ to get the precise output values.
%
The decomposition of choice is $\extcovnl$ on lower dimensional inputs.
%
The reason behind this choice is the stronger statement on the ranks of output NGVAS provided in \Cref{Proposition:WitnessGrammarDecomp}.
%
Since we have modified the context information of $\anngvas$ to get $\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \amarkingp}$, we need this assumption to guarantee that the rank gets below $\rankof{\anngvas}$.
%
Formally, we say that a marking $(\amarking, \anonterm, \amarkingp)\in\Nomega^{d}\times\nonterms\times\Nomega^{d}$ is \emph{simply decomposable}, denoted $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$, if there are $i, j\in\concincount$ with 
$\amarking_{\omega}=\settoomega{\omegaincount\cup\set{i}}{\amarking}$, $\amarkingp_{\omega}=\settoomega{\omegaoutcount\cup\set{j}}{\amarkingp}$ where
$\extcovnlof{{\otherctxNGVAS{\anngvas}{\amarking_{\omega}, \anonterm, \amarkingp_{\omega}}}}$ is a decomposition.
%
Here, for $X\subseteq [1, d]$ and $\amarking\in\Nomega^{d}$, the vector $\settoomega{X}{\amarking}\in\Nomega^{d}$ has $\settoomega{X}{\amarking}[i]=\omega$ if $i\in X$, and $\settoomega{X}{\amarking}[i]=\amarking[i]$ else.
%
While we cannot yet decide $\postfuncNof{\anngvas}{\amarking, \anonterm}$, we can decide a limited version that requires reachability on certain positions.
%
We formalize this notion.
%
For $\amarking, \amarkingp\in\Nomega^{d}$, $X\subseteq\concincount$, and $\anonterm\in\nonterms$, let $\postfuncNrof{\anngvas}{X, \amarkingp}{\amarking, \anonterm}$ be the set of elements 
\begin{align*}
    \mathsf{Id}(\downclsof{\setcond{\amarkingp'\in\Nomega^{d}}{\amarking\fires{\asymbol}\amarkingp', \amarkingp'[i]=\amarkingp[i]\text{ for all }i\in X}}).
\end{align*}

We observe that for simply decomposable markings, we can compute $\postfuncNr{\anngvas}{\concoutcount, \amarkingp}$.
%
We only need to compute the decomposition $\extcovnl$, but by \Cref{Proposition:WitnessGrammarDecomp}, we only need the $\postfuncN{\anngvas}$ and $\prefuncN{\anngvas}$ calls from the lower dimensions to achieve this goal.
%
Since the dimension of $\anngvas$ is a part of the rank, the reliability of $\perfect$ provides this.

\begin{lemma}\label{Lemma:SimplyDecomposable}
    Let $\perfect$ be reliable up to $\rankof{\anngvas}$, and $(\amarking, \anonterm, \amarkingp)$ a marking.
    %
    Then whether $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$ holds is effectively checkable.
    %
    If $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$, we can compute $\postfuncNrof{\anngvas}{\concoutcount, \amarkingp}{\amarking, \anonterm}$.
\end{lemma}

The other key observation that allows the definition of useful witness trees is \Cref{Lemma:UsefulRestriction}.
%
It states that we can compute a bound $\domainconst\in\N$ that applies in one of two ways depending on $\anngvas$.
%
In the first case, we observe that if a counter value grows beyond $\domainconst$ in a witness tree, then the marking must be simply decomposable.
%
In the second case, we observe that for markings that are not simply decomposable, that agree with the characteristic equations, and that have one counter larger than $\domainconst$, we can directly infer a sound output value that is maximal.
%
We formalize this by the notions of equation-justifiedness and equation-maximality.
%
A marking $(\amarking, \anonterm, \amarkingp)$ is \emph{equation-justified}, if $\omegaof{\amarking}=\omegaincount$, $\omegaof{\amarkingp}\subseteq\concoutcount$, and there is an $\asol\in\solof{\chareq{\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \amarkingp}}}$ for $\otherctxNGVAS{\anngvas}{\amarking, \anonterm, \amarkingp}$ with $\amarkingp\sqsubseteq\asol[\avar_{\acontextout}]$.
%
The marking is called \emph{equation-maximal}, if $\amarkingp$ is maximal among $\amarkingp'$ that make $(\amarking, \anonterm, \amarkingp')$ equation-justified.
%
With this formalism at hand, we state the result.
%
The proof has been moved to the appendix.

\begin{lemma}\label{Lemma:UsefulRestriction}
    Let $\perfect$ be reliable up to $\rankof{\anngvas}$.
    %
    We can compute a constant $\domainconst\in\N$ larger than any concrete value in $\amarkingin$, and a flag $\booleanflagof{\domain}\in\set{\top, \bot}$ where the following holds depending on $\booleanflagof{\domain}$.
    %
    \begin{itemize}
        \item $\booleanflagof{\domain}=\bot$.\  For any witness tree $\atree$ with root label $(\amarkingin, \anonterminalin, \amarkingpp)$, and any node labeled $(\amarking, \anonterm, \amarkingp)$ in $\atree$, if $\amarking[i]\geq \domainconst$ for some $i\in\concincount$, then $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$.
        \item $\booleanflagof{\domain}=\top$.\  For any $\amarking, \amarkingp\in\Nomega^{d}$ and $\anonterm\in\nonterms$ where $(\amarking, \anonterm, \amarkingp)$ is equation-maximal, we have $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$ or $\amarking\fires{\runsof{\anonterm}}\amarkingp$.
    \end{itemize}
\end{lemma}

Now, we are ready to define useful witness trees.
%
Let 
%
$$\domain=[0, \domainconst]^{\concincount}\times\omega^{\omegaincount}.$$
%
A witness tree $\atree$ is a \emph{useful witness tree}, if for each node $\anode$, with label $(\amarking, \asymbol, \amarkingp)$, the following hold.
%
\begin{itemize}
    \item For the subtree $\atreep$ with root $\anode$, $\amarkingp=\pumpingof{\atreep}.\outlabel$ holds.
    \item There is no successor of $\anode$ with the label $(\amarking, \asymbol, \amarkingp)$.
    \item If $\asymbol\in\terms$ then $\anode$ is a leaf with $\amarkingp\in\postfuncNof{\anngvas}{\amarking, \asymbol}$.
    \item If $\omegaincount\subset\omegaof{\amarking}$, then $\anode$ is a leaf with $\amarkingp\in\postfuncNof{\anngvas}{\amarking, \asymbol}$.
    \item If $\amarking\not\in\domain$, and $\asymbol=\anonterm\in\nonterms$, then $\anode$ is a leaf where 
    \begin{itemize}
        \item $(\amarking, \anonterm, \amarkingp)\in\simplydecomps$ and $\amarkingp\in\postfuncNrof{\anngvas}{\concoutcount, \amarkingp}{\amarking, \anonterm}$, or 
        \item $b_{\domain}=\top$ and $(\amarking, \anonterm, \amarkingp)$ is equation-maximal.
    \end{itemize}
\end{itemize}

As an implication of \Cref{Lemma:UsefulRestriction}, we see that useful witness trees are complete when it comes to witnessing coverability of bounded markings.

\begin{lemma}\label{Lemma:UWTCompleteness}
    Let $\atree$ be a witness tree with root labeled $(\amarkingin, \anonterminalin, \amarkingp)$ where $\omegaof{\amarkingin}=\omegaof{\amarkingp}$.
    %
    Then, there is a useful witness tree $\atreep$ with root labeled $(\amarkingin, \startnonterm, \amarkingp')$ where $\atree.\outlabel\leq\amarkingp'$.
\end{lemma}

Let $\witnessset^{(i)}$ be the set of useful witness trees with a root node labeled $(\amarking, \anonterm, \amarkingp)$ for $\amarking\in\domain$.
%
We observe that for all $i\in\N$, we can effectively construct $\witnessset^{(i)}$.
%
This is done by combining the trees present in $\witnessset^{(i-1)}$, and closing nodes using \Cref{Lemma:UsefulRestriction} and \Cref{Lemma:SimplyDecomposable}.
%
Note that $\concoutcount$ is precisely the set of output counters that matter for closing nodes.
%
This is because the remaining counters on the output, which are $\omegaoutcount$, are ignored by simple-decomposability, and are bound to be $\omega$ for equation-maximal markings.
%
The key observation for \Cref{Lemma:UWTVerification} is that given an input marking, there are finitely many values for the output counters in $\concoutcount$, and these can be guessed.

\begin{lemma}\label{Lemma:UWTVerification}
    Let $\perfect$ be reliable up to $\rankof{\anngvas}$ and let $i\in\N$.
    %
    Then, we can compute $\witnessset^{(i)}$.
\end{lemma}

It also follows that if we do not find any new useful witness trees for a certain depth, then we do not find any new ones for larger depths.

\begin{lemma}\label{Lemma:UWTFPStabilization}
    Let $i\in\N$ and $\witnessset^{(i)}=\witnessset^{(i+1)}$.
    %
    Then, $\witnessset^{(i+1)}=\witnessset^{(i+2)}$.
\end{lemma}

This implies that if we find a fixed point, we have collected all the output values that can be witnessed by useful witness trees.

\begin{corollary}\label{Corollary:UWTFPCompleteness}
    Let $i\in\N$ and $\witnessset^{(i)}=\witnessset^{(i+1)}$.
    %
    Then, for all useful witness trees $\atree$, with root label $(\amarking, \anonterm, \amarkingp)$ and $\amarking\in\domain$, we have $\atreep\in\witnessset^{(i)}$ with $\atreep.\inlabel=\atree.\inlabel$, $\atreep.\symlabel=\atree.\symlabel$, and $\atree.\outlabel\leq\atreep.\outlabel$.
\end{corollary}

Then, upon reaching such a fixed point, we can invoke \Cref{Lemma:UWTCompleteness}, \Cref{Corollary:UWTFPCompleteness}, \Cref{Lemma:WitnessTreeComplete}, and \Cref{Lemma:WitnessTreeSound}, and conclude that the downward closure of the output values we have collected is exactly $\downclsof{\postfuncNof{\anngvas}{\amarkingin, \anonterminalin}}$. 
%
It only remains to argue that the computation indeed reaches a fixed point.

\begin{lemma}\label{Lemma:UWTFPGuaranteedStabilization}
    There is an $i\in\N$ with $\witnessset^{(i)}=\witnessset^{(i+1)}$.
\end{lemma}

The detailed argument has been moved to the appendix.
%
To give an intuition, the finiteness of each $\witnessset^{(i)}$ leads to a sequence of useful witness trees $\atree_{0}, \atree_{1}, \ldots$ where the earlier trees are included in the later ones.
%
Because $\domain$ is finite, there are only finitely many input values for non-leaf nodes.
%
Using this, we can apply a WQO argument to detect infinitely growing output values.
%
This implies infinitely many side-pumps.
%
But this means that the number of $\omega$'s in the output grows infinitely, but there can at most be $d$ many $\omega$'s.
%
This is a contradiction.


%\begin{lemma}\label{Lemma:UWTCompleteness}
%    Let $\atree$ be a witness tree with $\omegaof{\atree.\inlabel}=\omegaof{\atree.\outlabel}$.
    %
%    There is a useful witness tree $\atreep$ with $\atree.\inlabel=\atreep.\inlabel$, $\atree.\outlabel\leq\atreep.\outlabel$.
%\end{lemma}


%\begin{lemma}\label{Lemma:UWTCompleteness}
%    Let $\atree$ be a witness tree with root labeled $(\amarkingin, \anonterminalin, \amarkingpp)$ and $\omegaof{\amarkingin}=\omegaof{\amarkingpp}$.
%    %
%    There is a useful witness tree $\atreep$ with root labeled $(\amarkingin, \startnonterm, \amarkingpp')$ and $\atree.\outlabel\leq\amarkingpp'$.
%\end{lemma}



==> extcovgraph.tex <==
\section{The External Coverability Grammar}



==> iterationlemma_backup_2025.tex <==
\section{Iteration Lemma}
\begin{theorem}
Let $\anngvas$ be perfect with restriction $\restrictions = \baseeffect+\periodeffect^*$. 
Let $\baseeffectchoice\in\restrictions$ and let $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Then there is $\aconst_0\in\N$ so that for every $\aconst\geq \aconst_0$ there is a run $\iterrundef\in\runsof{\agram}$ with $\acontextin\fires{\iterrundef}\acontextout$ and $\paramparikhof{\updates}{\iterrundef} =  \baseeffectchoice + \periodeffect\cdot \aconst\cdot \periodeffectchoice$. %\in \restrictions$ so that $\paramparikhof{\updates}{\arun^{k}}\geq \avec + k \sum\asetvec$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
We proceed by Noetherian induction on the nesting depth and consider the non-linear case first.
Consider $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Perfectness (P0) gives us a solution $\asol$ to $\chareq{\anngvas}$ with $\asol[\updvar]=\baseeffectchoice$ and a full homogeneous solution $\ahomsol$ to $\homchareq{\anngvas}$ with $\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsection{Non-Linear Case}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Reaching Derivation}
We define $\asol' = \asol+ \maxconst\cdot \ahomsol$ as a new solution to $\chareq{\anngvas}$ ($\ahomsol$ is homogeneous) that is large enough to embed non-negative runs for all instances of all childNGVAS. 
The situation is the following. 
The derivation induced by $\asol'$ will introduce several instances of the terminal symbols $\anngvasp\in\terms$. 
Each instance $\anngvasp$ is a childNGVAS that now has to provide its own derivation. 
There are two requirements on the derivations of $\anngvasp$ we are looking for.
\begin{itemize}
\item[(1)] The run given by the derivation has to be fireable.  
\item[(2)] The derivations of all $\anngvasp$ instances together have to give the number of updates $\asol'[\updvardef]$, to guarantee the reachability property we are after.   
\end{itemize}
To achieve (1), our plan is to use the perfectness property~(P4) for all instances of $\anngvasp$ except one. 
Property~(P4) gives us a derivation whose run is guaranteed to be fireable and  correspond to the base vector $\baseeffectdef$ of the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$. 
This, however, does not yet guarantee~(2). 
The solution $\asol'$ may also ask for repetitions of the period vectors in~$\periodeffectdef$. 
For the one instance of $\anngvasp$ that we left out, we obtain the non-negative run by invoking the induction hypothesis with appropriate $\baseeffectchoicedef$ and~$\periodeffectchoicedef$. 
The universal quantification over these vectors in the theorem thus makes it possible to hand over outer constraints on the repetition count of the period vectors to the childNGVAS. 
The constant $\maxconst$ will be chosen large enough to cover the enabling constant $\aconst_{0, \anngvasp}$ for all $\anngvasp$.  
We turn to the details.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We first define $\maxconst$.
Let $\anngvasp\in\terms$ with $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$.  
To invoke the induction hypothesis, we let $\baseeffectchoicedef$ include the base vector of the restriction $\baseeffectdef$ and repetitions of the period vectors as required by $\asol$. 
For $\periodeffectchoicedef$, we follow the full homogeneous solution:
\begin{align*}
\baseeffectchoicedef\ &=\ \baseeffectdef + \periodeffectdef\cdot \asol[\periodeffectvardef]\\
\periodeffectchoicedef\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
As $\anngvasp$ is perfect by (P6) and $\periodeffectchoicedef\geq 1$ by (P3), we can invoke the induction hypothesis. 
It yields a repetition count $\aconst_{0, \anngvasp}\in\N$ so that for every $\aconst\geq \aconst_{0, \anngvasp}$ we have a run $\iterrunchilddef\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunchilddef}=\baseeffectchoice_{\anngvasp} +  \periodeffectdef \cdot \aconst\cdot  \periodeffectchoicedef$. 
We let $\maxconst = \max\setcond{\aconst_{0, \anngvasp}}{\anngvasp\in\terms}\cup\set{1}$, meaning $\asol'$ will contain at least one copy of $\ahomsol$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We show that the solution $\asol'$ induces a derivation and discuss its properties.
Since~$\asol'$ solves Esparza-Euler-Kirchhoff, since it contains a copy of $\ahomsol$, and since $\ahomsol[\prodvar]\geq 1$ by~(P2), we can invoke Theorem~\ref{Theorem:EEK} to obtain a derivation $\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach$. 
By Lemma~\ref{Lemma:EEKConverse}, $\asentformreach$ is a sequence of terminal symbols in $\anngvas$. 
Thanks to $\ptof{\anngvas}{\avar_{\prods}, \avar_{\terms}}$, we even have $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$.  
Each terminal in $\asentformreach$ is an update $\anupd\in\Z^{\adim}$ or a childNGVAS $\anngvasp$.
\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We still have to derive runs for the childNGVAS~in~$\asentformreach$. 
Together, we then have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach\xrightarrow{\aprodseqreachterms}\arun_1\ldots \arun_{\cardof{\asentform}} = \reachrun\ .
\end{align*}
The production sequence $\aprodseqreachterms$ concatenates production sequences $\aprodseqreachtermsindex$ for the terminal symbols in $\asentform$. 
If $\seqat{\asentform}{\mathit{i}}$ is an update $\anupd$, then $\aprodseqreachtermsindex=\varepsilon$, the production sequence is empty and $\arun_i=\anupd$. 
If $\seqat{\asentform}{\mathit{i}}$ is the first instance of a childNGVAS $\anngvasp$, then $\aprodseqreachtermsindex$ is a production sequence that yields the run $\arun_i=\arun_{\anngvasp}^{(\maxconst)}$ defined above.  
If $\seqat{\asentform}{\mathit{i}}$ is another occurrence of $\anngvasp$, then we use the production sequence which exists by (P4) and results in a run $\arun_i=\baserundef$ with effect $\baseeffectdef$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We show that the run $\reachrun$
transforms the initial marking $\asol'[\invar]\sqsubseteq \acontextin$ into the final marking $\asol'[\outvar]\sqsubseteq\acontextout$, as long as we ignore non-negativity.
That the run may fall below zero is a problem we adress later. 
Thanks to the marking equation $\meof{\anngvas}{\invar, \updvar, \outvar}$, all we have to show is that we provide the expected number of updates:
\begin{align}
\paramparikhof{\updates}{\arun}\ = \ \asol'[\avar_{\updates}]\ = \ \restrictto{\asol'[\avar_{\terms}]}{\updates} + \sum_{\anngvasp\in\terms}\asol'[\avar_{\anngvasp, \updates}]\ .\tag{UPDATES-REACH}\label{Equation:UpdatesReach} 
\end{align}
The latter equation is due to $\computeupdatesof{\anngvas}{\termvar, \updvar}$.\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We already argued that $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$. 
As a first consequence, $\paramparikhof{\updates}{\asentformreach}=\restrictto{\asol'[\avar_{\terms}]}{\updates}$, the number of updates in $\reachrun$ that stem from $\asentformreach$ is as expected by $\asol'$. 
As a second consequence, we know that $\asentformreach$ contains  $\asol'[\termvar[\anngvasp]]$ many instances of~$\anngvasp$. 
We show that the runs of all these instances together provide the number of updates $\asol'[\avar_{\anngvasp, \updates}]$.  
Except for the first instance, we used (P4) to construct a run with the number of updates $\baseeffectdef$. 
For the first instance, we used the run $\iterrunchilddefmax$.  
According to $\computeupdatesof{\anngvasp}{\termvar, \updvar}$, we have to show that $\iterrunchilddefmax$ contributes the updates $\baseeffectdef+\periodeffectdef\cdot \asol'[\periodeffectvardef]$. 
This holds with the following reasoning: 
\begin{align*}
&\ \paramparikhof{\updates}{\iterrunchilddefmax} \\
\argument{Induction hypothesis}=&\ \baseeffectchoicedef+\periodeffectdef\cdot \maxconst\cdot \periodeffectchoicedef\\
\argument{Definition of $\baseeffectchoicedef$ and~$\periodeffectchoicedef$} =& \baseeffectdef+\periodeffectdef\cdot \asol[\periodeffectvardef]+ \periodeffectdef \cdot \maxconst\cdot \ahomsol[\periodeffectvardef]\\
\argument{Definition of $\asol'$}=&\ \baseeffectdef + \periodeffectdef\cdot \asol'[\periodeffectvardef]\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The run $\reachrun$ is not guaranteed to stay non-negative. 
Neither do the updates in $\asentformreach$ guarantee non-negativity, nor do the runs of the childNGVAS guarantee non-negativity on the counters from $\adimset$. 
We now address this problem. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Pumping Derivation and Embedding}
To enable $\reachrun$, the idea is to surround it by a number of up- and down-pumping sequences.  
This means we wish to repeatedly apply the pumping derivation $\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq$ that exists by perfectness (P5).  
Unfortunately, we cannot even insert a single copy of $\aprodseqpump$ without running the risk of jeopardizing reachability, the fact that the run $\reachrun$ takes the input marking to the output marking. 
The way out is to embed the pumping derivation into a homogeneous solution. 
Embedding the pumping derivation into a homogeneous solution means we provide another derivation 
$\startnonterm\xrightarrow{\aprodseqdiff}\diffrunleft.\startnonterm.\diffrunright$ that can be understood as the difference between the homogeneous solution and the pumping derivation. 
Formally, the two derivations together,  
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq\xrightarrow{\aprodseqdiff}\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq \ ,
\end{align*}
should have the effect prescribed by the homogeneous solution. 
We turn to the details. 
%We make the embedding precise, the construction of an appropriate homogeneous solution and the definition of $\aprodseqdiff$. 
\\\\
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
We begin by inspecting the pumping derivation. 
We can assume $\aprodseqpump=\aprodseqpumpanngvas.\aprodseqpumpterms$ so that $\aprodseqpumpanngvas$ contains the productions of $\anngvas$ and $\aprodseqpumpterms$ contains the productions of the childNGVAS and their descendants. 
This means $\aprodseqpumpanngvas$ will produce a sequence of terminals in $\anngvas$, we have $\startnonterm \xrightarrow{\aprodseqpumpanngvas} \asentformpumpleft.\startnonterm.\asentformpumpright$ with $\asentformpumpleft, \asentformpumpright\in\terms^*$. 
With Lemma~\ref{Lemma:EEKConverse}, we can conclude that $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
We can assume $\aprodseqpumpterms$ is a concatenation of production sequences $\aprodseqpumpanngvaspindex$, one sequence for every instance of a childNGVAS in $\asentformpumpleft.\asentformpumpright$. 
We have the guarantee that $\startnonterm_{\anngvasp}\xrightarrow{\aprodseqpumpanngvaspindex}\arundefindex$\rfm{Fix.} with $\paramparikhof{\updates}{\arundefindex}\in \restrictionsdef^*$. 
 \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The homogeneous solution $\ahomsol$ we are given may not be large enough to embed $\aprodseqpump$.  
We scale it to $\scaleconst\cdot\ahomsol$ with $\scaleconst = \embedconst+\enableconst$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The constant $\embedconst$ should be understood as the least natural number large enough so that $\embedconst\cdot \ahomsol$ embeds $\aprodseqpump$. 
Embedding $\aprodseqpump$ is made formal with two requirements we give next. 
These requirements are monotonic: if they hold for $\embedconst\cdot \ahomsol$, then they will hold for $\scaleconst\cdot \ahomsol$. 
The first requirement is that we want to be able to subtract $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ from $(\embedconst\cdot \ahomsol)[\prodvar]$.
Even more, in the difference we want to retain a copy of each production to be able to invoke Esparza-Euler-Kirchhoff.  
So $\embedconst$ has to be large enough so that 
\begin{align}
(\embedconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1\ .\tag{R1}\label{Equation:EmbeddingProductions}
\end{align} 
This can be achieved as the productions belong to the support, due to (P2) in perfectness.
An important consequence (that we prove in a moment) is 
\begin{align}
(\embedconst\cdot \ahomsol)[\termvar] - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\geq 0\ . \tag{$\spadesuit$}\label{Equation:EmbeddingConsequence}
\end{align} 
The next requirement is that $\embedconst\cdot \ahomsol$ has to cover the updates produced by $\aprodseqpump$. 
For the updates in $\asentformpumpleft.\asentformpumpright$ that are produced by~$\aprodseqpumpanngvas$, we already have the inequality $(\embedconst\cdot \ahomsol)[\updvar] - \paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright} \geq 0$. 
This is due to~\eqref{Equation:EmbeddingConsequence} combined with $\computeupdatesof{\anngvas}{\termvar, \updvar}$. 
However, we also have to cover the updates produced by the instances of the childNGVAS in $\asentformpumpleft.\asentformpumpright$.  
Consider the childNGVAS~$\anngvasp$ with restriction $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$.  
With Inequality~\eqref{Equation:EmbeddingConsequence} and $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we are sure $(\embedconst\cdot \ahomsol)[\updvardef]$ contains precisely one copy of the base vector $\baseeffectdef$ for every instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
However, the pumping sequence $\aprodseqpump$ may also produce copies of the period vectors. 
Let $\periodeffectpumpdef\in\N^{\periodeffectdef}$ count the period vectors in all runs $\arundefindex$ that belong to an instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$.
For every childNGVAS $\anngvasp\in\terms$, we want 
\begin{align}
(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0\ .\tag{R2} \label{Equation:EmbeddingEffect}
\end{align} 
This can be achieved as the period vectors of all childNGVAS belong to the support,  (P3). \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
Inequality~\eqref{Equation:EmbeddingConsequence} follows from Inequality~\eqref{Equation:EmbeddingProductions} by
\begin{align*}
&\ (\embedconst\cdot \ahomsol)[\termvar] - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\\
\argument{$\ptof{\anngvas}{\prodvar, \termvar}$ and Lemma~\ref{Lemma:EEKConverse}}=&\ \effof{\terms}\cdot (\embedconst\cdot \ahomsol)[\prodvar]  - \effof{\terms}\cdot \paramparikhof{\prods}{\aprodseqpumpanngvas}\\
\argument{Linearity}=&\ \effof{\terms}\cdot ((\embedconst\cdot \ahomsol)[\prodvar]  - \paramparikhof{\prods}{\aprodseqpumpanngvas})\\
\argument{Inequality~\eqref{Equation:EmbeddingProductions} and monotonicity of $\effof{\terms}$}\geq &\ \effof{\terms}\cdot 1\\
\argument{Monotonicity of $\effof{\terms}$}\geq &\ 0\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Difference Derivation}
We now define the production sequence $\aprodseqdiff$. 
We proceed in two steps and first define the productions in $\anngvas$ followed by the productions in the childNGVAS and their descendants, $\aprodseqdiff = \aprodseqdiffanngvas.\aprodseqdiffterms$. 
As we move along, we define the constant $\enableconst$ that has been missing. 
Recall that the goal is to turn the difference $(\scaleconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ into a non-negative run. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The production sequence $\aprodseqdiffanngvas$ should derive a terminal word in $\anngvas$. 
We plan to obtain it with an invokation of Esparza-Euler-Kirchhoff. 
To see that the result applies, note that $\scaleconst\cdot \ahomsol$ solves $\homeekof{\anngvas}{\prodvar}$ as $\ahomsol$ does. 
Moreover, we argued above that also $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
Hence, $(\scaleconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
By Requirement~\eqref{Equation:EmbeddingProductions} on $\embedconst$, we have $(\scaleconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1$. 
Theorem~\ref{Theorem:EEK} thus yields a derivation $\startnonterm\xrightarrow{\aprodseqdiffanngvas} \asentformdiffleft.\startnonterm.\asentformdiffright$ with $\paramparikhof{\prods}{\aprodseqdiffanngvas} = (\scaleconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now construct the production sequence $\aprodseqdiffterms$ that turns the instances of the childNGVAS in $\asentformdiffleft.\asentformdiffright$ into non-negative runs: 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqdiffanngvas}\asentformdiffleft.\startnonterm.\asentformdiffleft\xrightarrow{\aprodseqdiffterms}\diffrunleft.\startnonterm.\diffrunright\ . 
\end{align*}
We proceed as in the construction of the base run.
When the childNGVAS~$\anngvasp$ occurs in~$\asentformdiffleft.\asentformdiffright$ for the first time, we use the derivation of a run $\arun'^{(\enableconst)}_{\anngvasp}$ that is given by the induction hypothesis. 
The task of this run is to compensate the $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0$ excess in period vectors from the pumping derivation, and the definition will be given in a moment. 
For the remaining occurrences of $\anngvasp$, we use the derivation of the run $\baserundef$ that we have by (P4).\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To construct $\arun'^{(\enableconst)}_{\anngvasp}$ that compensates the excess in period vectors, we invoke the induction hypothesis with the following vectors: 
\begin{align*}
\baseeffectchoicedef'\ &=\ \baseeffectdef + \periodeffectdef\cdot [ (\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef]\\
\periodeffectchoicedef'\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
As the childNGVAS $\anngvasp$ is perfect by (P6) and as $\periodeffectchoicedef'\geq 1$ by (P3), the induction hypothesis applies. 
It gives us a repetition count $\aconst_{0, \anngvasp}'\in\N$ from which $\anngvasp$ has non-negative runs: for every $\aconst\geq \aconst_{0, \anngvasp}'$ we have $\arun'^{(\aconst)}_{\anngvasp}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\arun'^{(\aconst)}_{\anngvasp}}=\baseeffectchoice_{\anngvasp}' +  \periodeffectdef\cdot \aconst \cdot \periodeffectchoicedef'$. 
The missing scaling factor is then  $\enableconst = \max\setcond{\aconst_{0, \anngvasp}'}{\anngvasp\in\terms}\cup\set{1}$. 
It covers the repetition count for every childNGVAS and is defined in analogy to $\maxconst$ from above. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To sum up, we now have $\startnonterm\rightarrow^*\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq$ using the production sequence $\aprodseqpump.\aprodseqdiff$ with $\aprodseqpump = \aprodseqpumpanngvas.\aprodseqpumpterms$ and $\aprodseqdiff=\aprodseqdiffanngvas.\aprodseqdiffterms$. 
We check that the number of updates in the terminal sequence is the one expected by $\scaleconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}\ =\
(\scaleconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-PUMP-DIFF}\label{Equation:UpdatesPumpDiff}
\end{align} 
We rely on $\computeupdatesof{\anngvas}{\termvar, \updvar}$ to see that 
\begin{align*}
(\scaleconst\cdot\ahomsol)[\updvar]\ =\ \restrictto{(\scaleconst\cdot\ahomsol)[\termvar]\ }{\updates}+\sum_{\anngvasp\in\terms}(\scaleconst\cdot\ahomsol)[\updvardef]\ .
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We first show that
\begin{align*}
\paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright.\asentformdiffleft.\asentformdiffright}\ = \ \restrictto{(\scaleconst\cdot\ahomsol)[\termvar]\ }{\updates}\ .
\end{align*}
The equation says that the number of updates produced directly by $\anngvas$ is as expected by the scaled homogeneous solution. 
With Lemma~\ref{Lemma:EEKConverse} and $\ptof{\anngvas}{\prodvar, \termvar}$, it suffices to realize that 
\begin{align*}
&\ \paramparikhof{\prods}{\aprodseqpumpanngvas}+\paramparikhof{\prods}{\aprodseqdiffanngvas}\\ 
\argument{Definition $\aprodseqdiffanngvas$}=&\ \paramparikhof{\prods}{\aprodseqpumpanngvas}+ (\scaleconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\\
 =&\ (\scaleconst\cdot \ahomsol)[\prodvar]\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now consider the childNGVAS $\anngvasp$ with restriction $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$. 
The task is to show that $\aprodseqpumpterms$ and $\aprodseqdiffterms$ together create precisely $(\scaleconst\cdot\ahomsol)[\updvardef]$ many updates 
in the runs derived from the $\anngvasp$ instances. 
By $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we have
\begin{align*}
(\scaleconst\cdot\ahomsol)[\updvardef]\ =\ \baseeffectdef\cdot (\scaleconst\cdot\ahomsol)[\termvar[\anngvasp]] - \periodeffectdef\cdot (\scaleconst\cdot\ahomsol)[\periodeffectvardef]\ .
\end{align*}
With the argument from the previous paragraph, we know that $\aprodseqpumpanngvas$ and $\aprodseqdiffanngvas$ together create precisely $(\scaleconst\cdot\ahomsol)[\termvar[\anngvasp]]$ many instances of $\anngvasp$. 
Moreover, the run we derive from such an instance using $\aprodseqpumpterms$ and $\aprodseqdiffterms$ contains at least the number of updates prescribed by the base vector $\baseeffectdef$. 
The run may contain further updates that together make up copies of the period vectors. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
It remains to check that the expected number of copies of the period vectors $(\scaleconst\cdot\ahomsol)[\periodeffectvardef]$  coincides with the number of copies produced by $\aprodseqpumpterms$ and $\aprodseqdiffterms$. 
This holds by
\begin{align*}
&\ \periodeffectpumpdef\quad +\quad  (\embedconst\cdot \ahomsol)[\periodeffectvardef]-\periodeffectpumpdef + \enableconst\cdot \periodeffectchoicedef'\\
 =& \ (\embedconst\cdot \ahomsol)[\periodeffectvardef] + (\enableconst\cdot \ahomsol)[\periodeffectvardef]\\
 =& \ (\scaleconst\cdot \ahomsol)[\periodeffectvardef]\ . 
\end{align*}
To explain the equations, recall that $\aprodseqpumpterms$ produces $\periodeffectpumpdef$ many copies of the period vectors. 
For $\aprodseqdiffterms$, we get $(\embedconst\cdot \ahomsol)[\periodeffectvardef]-\periodeffectpumpdef$ many copies from $\baseeffectchoicedef'$. 
The repetition contributes another $\enableconst\cdot \periodeffectchoicedef'$ copies.  
The second equation then replaces  $\periodeffectchoicedef'$ with its definition and cancels $\periodeffectpumpdef$.
The last is by $\scaleconst=\embedconst+\enableconst$. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Pumping}
We now make the reaching run fireable by surrounding the reaching derivation by repetitions of the pumping derivation and the difference derivation. 
Here is what we know.
The runs $\upseq$ and $\downseq$ generated by the pumping derivation have a strictly positive resp.~a strictly negative effect on the unbounded counters.
Together, the runs $\upseq.\downseq$ and $\diffrunleft.\diffrunright$ from the pumping derivation and from the difference derivation have effect zero on the unbounded counters.
This means $\upseq.\diffrunleft.\diffrunright$ will have a strictly positive effect on the unbounded counters.
Repeating the pumping and the difference derivation in a naive way then yields
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^k}\upseq^k.\startnonterm.\downseq^k\xrightarrow{\aprodseqdiffanngvas^k}&\ \upseq^k.\asentformdiffleft^k.\startnonterm.\asentformdiffright^k.\downseq^k\\
\xrightarrow{\aprodseqdiffterms^k}&\ \upseq^k.\diffrunleft^k.\startnonterm.\diffrunright^k.\downseq^k \xrightarrow{\aprodseqreach}\upseq^k.\diffrunleft^k.\reachrun.\diffrunright^k.\downseq^k\ .
\end{align*}
The problem is that $\diffrunleft$ and $\diffrunright$ are not placed next to each other, but we first generate the copies of $\diffrunleft$ and later the copies of $\diffrunright$. 
Unfortunately, there is no guarantee that $\upseq.\diffrunleft$ has a positive effect on the unbounded counters.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
The way out is to use the wide tree theorem on the difference derivation. 
Then the hurdle required by the copies of the difference run will only grow logarithmically in the number of tokens produced by the pumping run.
This will eventually make the run fireable.
We turn to the details.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We first argue that the wide tree theorem applies. 
By definition, the NGVAS~$\anngvas$ is non-linear, strongly connected, and only has useful non-terminals. 
We already observed that $\prodsvec = \paramparikhof{\prods}{\aprodseqdiffanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
We can thus arrange $\aconst$ copies of $\prodsvec$ in a parse tree $\atreeofdef$ of height $\ceilof{1+\log \aconst}\cdot \normof{\prodsvec}$, for every $\aconst\geq 1$. 
Let the yield by $\yieldof{\atreeofdef}=\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}$. 
The theorem moreover guarantees that for every prefix $\asentform$ of $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$, the number of incomplete copies of $\termsvec=\effof{\terms}\cdot \avec_{\prods}$ is bounded by $\ceilof{1+\log \aconst}$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the derivation we are after, it remains to turn every copy of $\termsvec$ in $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$ into a run using $\aprodseqdiffterms$. 
Then we have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^{\aconst}}\upseq^{\aconst}.\startnonterm.\downseq^{\aconst}\xrightarrow{\text{wide tree theorem}}&\ \upseq^{\aconst}.\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqdiffterms^{\aconst}}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\startnonterm.\arun_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqreach}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\reachrun.\arun_{\aconst, 2}.\downseq^{\aconst}\ =\ \iterrundef\ .
\end{align*}
These are runs $\iterrundef$ we are after.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
It remains to determine a constant~$\aconst_0$ from which the runs $\iterrundef$ stay non-negative. 
We estimate the hurdle we have to meet with the up-pumping sequence. 
We first consider the incomplete copies of~$\termsvec$.
We iterate over all sentential forms~$\asentform$ that could result from them and over all runs $\arun$ that could be derived from $\asentform$ using $\aprodseqdiffterms$, and determine the maximal hurdle:
\begin{align*}
\maxhurdle\ = \ \max\setcond{\hurdleof{\arun}}{\paramparikhof{\terms}{\asentform}<\termsvec\text{ and } \asentform\xrightarrow{\aprodseqdiffterms}\arun}\ .
\end{align*}
We slightly abuse the notation here. 
Actually, we do not use the full $\aprodseqdiffterms$ but only the productions for the childNGVAS~$\anngvasp$ that occur in~$\asentform$. 
For one instance of $\anngvasp$, there is a choice of whether to derive $\baserundef$ or $\arun'^{(\enableconst)}_{\anngvasp}$. 
The above notation is meant to cover all cases.\\\\  
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
Recall that $\upseq.\diffrunleft.\diffrunright$ has a strictly positive effect on the unbounded counters. 
This means a complete copy of $\termsvec$ does not add to the hurdle.
So the maximal hurdle we have to expect due to incomplete copies of $\termsvec$ is $\maxhurdle\cdot \ceilof{\log \aconst+1}$. 
To enable the above run, we still have to add $\hurdleof{\reachrun}$.
With this analysis, the run  $\iterrundef$ will stay non-negative as long as $\aconst\geq \aconst_0$, with $\aconst_0$ the least natural number satisfying
\begin{align*}
\aconst_0\quad \geq\quad \maxhurdle\cdot \ceilof{\log \aconst_0+1}\ +\ \hurdleof{\arun}\ . \\
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that each run $\iterrundef$ with $\aconst\geq \aconst_0$ has the properties formulated in the iteration lemma: 
it solves reachability and uses a number of updates that is as desired.
Thanks to the marking equations, we can study these properties on a Parikh equivalent run. 
We use
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\reachrun.\diffrunright^\aconst.\downseq^{\aconst}}\ =\
\paramparikhof{\updates}{\upseq^{\aconst}.\arun_{\aconst, 1}.\reachrun.\arun_{\aconst, 2}.\downseq^{\aconst}}\ =\ \ \paramparikhof{\updates}{\iterrundef}\ .
\end{align*}
To see that the first equality, note that the tree $\atreeofdef$ has the same productions as $\aprodseqdiffanngvas^k$.
By Lemma~\ref{Lemma:EEKConverse}, we have $\paramparikhof{\terms}{\asentformdiffleft^\aconst.\asentformdiffright^\aconst}=\paramparikhof{\terms}{\asentform_{\aconst, 1}.\asentform_{\aconst, 2}}$. 
We then apply the same derivations to the childNGVAS in these sentential forms.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that we solve reachability. 
Since $\asol'$ is a solution to the characteristic equations and $\scaleconst\cdot \ahomsol$ is a solution to the homogeneous variant of the characteristic equations. 
Hence, also $\asol''=\asol'+\aconst\cdot \scaleconst\cdot \ahomsol$ solves the charateristic equations.
Due to $\meof{\anngvas}{\invar, \updvar, \outvar}$, this in particular means $\asol''[\invar]+\effof{\updates}\cdot \asol''[\updvar]=\asol''[\outvar]$. 
By \eqref{Equation:UpdatesReach}, we have  $\paramparikhof{\updates}{\reachrun}=\asol'[\updvar]$. 
By \eqref{Equation:UpdatesPumpDiff}, we have $\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}=\scaleconst\cdot \ahomsol[\updvar]$.
Hence, $\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\reachrun.\diffrunright^\aconst.\downseq^{\aconst}}=\asol''[\updvar]$. 
This means the Parikh vector satisfies the marking equation.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We have to show that the number of updates belongs to $\baseeffectchoice + \N\cdot \periodeffect\cdot \periodeffectchoice$. 
We just argued that the number of updates is $\asol''[\updvar]$, so we can calculate as follows
\begin{align*}
&\ \asol''[\updvar]\\
\argument{Definition $\asol''$}=&\ \asol'[\updvar]+\aconst\cdot \scaleconst\cdot \ahomsol[\updvar]\\
\argument{Definition $\asol'$}=&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot \scaleconst\cdot \ahomsol[\updvar]\\
\argument{$\asol[\updvar]=\baseeffectchoice$}=&\ \baseeffectchoice+(\maxconst+\aconst\cdot \scaleconst)\cdot\ahomsol[\updvar]\\
\argument{$\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$}=&\ \baseeffectchoice+(\maxconst+\aconst\cdot \scaleconst)\cdot\periodeffect\cdot \periodeffectchoice\ .
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

\subsection{Linear Case}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

%\rfm{Warum die Menge $R$: Iterieren unten und oben klappt sonst nicht unabhängig voneinander.}



==> iterationlemma_linear_case_backup.tex <==
\subsection{Linear Case}
We construct runs $\iterrundef$ of this form
\begin{align*}
\underbrace{\upseq^{\aconst}.\diffrunleft^{\aconst}.\reachrunleft.\downseqint^{\aconst}}_{\text{Lambert pumping}}.\reachruncenterdef.\underbrace{\upseqint^{\aconst}.\diffrunright^{\aconst}.\reachrunright.\downseq^{\aconst}}_{\text{Lambert pumping}}\ .
\end{align*}
The reader familiar with Lambert's iteration lemma for VAS reachability will already see that we have created two pumping situations, one on the left and one on the right. 

What is new, not only compared to VAS reachability but also compared to the non-linear case,  is that the reaching run for the center $\reachruncenterdef$ changes with the iteration count $\aconst$. 
Here is why. 
To solve reachability, the number of updates in the overall run has to take the form $\at{(\asol+\abound\cdot \ahomsol)}{\updvar}$ for some $\abound\in\N$. 
If we only iterate the pumping and the difference derivation, however, we do not quite obtain a homogeneous solution. 
What we are missing are repetitions of the period vectors for the childNGVAS in the center. %, which the homogeneous solution may also contribute.
%The homogeneous solution may also contribute repetitions of the period vectors in the childNGVAS that belong to the center,  
Indeed, in the homogeneous characteristic equations, the variables $\periodeffectvardefcenter$ are not forced to be zero.
If they receive positive values in $\ahomsol$, the homogeneous solution expects pumping to happen in the children. 
By making $\reachruncenterdef$ dependent on the number of iterations, we can incorporate this pumping. 

Why have we not seen the problem in the non-linear case? 
In the non-linear case, every production variable belongs to the support by \perfectnessprodsnospace, and hence receives a positive value in the (full) homogeneous solution. 
Since every terminal symbol occurs on the right-hand side of a production, every derivation corresponding to the homogeneous solution creates at least one instance of each terminal.
This in particular holds for the combination of pumping and difference derivation. 
Now, if the homogeneous solution expects pumping in a childNGVAS, we carry out this pumping in the new instance of the child. 
In the linear case, the center production cannot be repeated and we have not created a variable for it. 
Hence, the trick does not apply. 
The trick again works for the runs $\reachrunleft$ and $\reachrunright$.
We turn to the construction of the runs. 

We construct $\reachrunleft$ and $\reachrunright$ by first invoking Theorem~\ref{Theorem:EEK}.
We then have to produce runs for the children. 
For all instances of a child except one, we use \perfectnessbasenospace.
For the one instance that is left, we use a run that exists by the induction hypothesis.  
The details are like in the non-linear case except for one aspect.  
The runs $\reachrunleft$, $\reachrunright$, and $\reachruncenterzero$ have to agree on the factor $\maxconst$ by which to scale the homogeneous solution.  
We achieve this by defining $\maxconst$ as the maximum over all $\initconstdef$, independent of the direction to which $\anngvasp$ belongs.

For $\reachruncenterdef$, we start from the terminal sequence given by the center production. 
To construct the runs for the children, consider the first instance of $\anngvasp\in\termscenter$. 
Constant~$\maxconst$ allows us to invoke the induction hypothesis.
Rather than invoking it with $\maxconst$, however, we invoke it with $\maxconst+\aconst\cdot \sumconst$, with $\sumconst$ defined below. 
This makes the run dependent on $\aconst$. 
For the remaining instances of $\anngvasp$, we again rely on~\perfectnessbasenospace.

To be able to construct the difference runs, we first have to modify the requirements on the embedding constant so as to take into account the internal pumping sequence and the directions. 
Let $\periodeffectpumpdefdir$ and $\periodeffectpumpintdefdir$ with $\mydir\in\set{\myleft, \myright}$ be the numbers of period vectors produced by the pumping resp. the internal pumping sequence in the given direction.  
Embedding requires 
\begin{align*}
\at{(\embedconst\cdot \ahomsol)}{\prodvar} - \paramparikhof{\prods}{\aprodseqpumpanngvas.\aprodseqpumpintanngvas}&\geq 1\\
\at{(\embedconst\cdot \ahomsol)}{\periodeffectvardefdir} - (\periodeffectpumpdefdir+\periodeffectpumpintdefdir)&\geq 0\ .
\end{align*} 

For the construction of the difference runs, we start by calling Theorem~\ref{Theorem:EEK}. 
Note that this needs the first embedding requirement. 
To also construct runs for the children, we again combine \perfectnessbase with an invokation of the induction hypothesis for one instance per childNGVAS.
In this invokation,  when the child is $\anngvasp$ and the direction is $\mydir$, we use the base vector $\baseeffectdef + \at{(\embedconst\cdot \ahomsol)}{\periodeffectvardefdir} - (\periodeffectpumpdefdir+\periodeffectpumpintdefdir)$. 
Once the pumping sequences are added to the base vector, we have $\at{(\embedconst\cdot \ahomsol)}{\periodeffectvardefdir}$ repetitions of the period vectors. 
For enabledness, we determine a factor $\enableconst$ that is common to both directions, similar to what we have seen for the reaching runs. 
We then set $\sumconst=\embedconst+\enableconst$. 


The runs have the following properties with $\mydir\in\set{\myleft, \myright}$:
\begin{align*}
\paramparikhof{\updates}{\reachrundir}\ &=\ (\asol+\maxconst\cdot \ahomsol)[\updvardir]\\
\paramparikhof{\updates}{\reachruncenterdef}\ &=\ (\asol+(\maxconst+\aconst\cdot \sumconst)\cdot\ahomsol)[\updvarcenter]\\
\paramparikhof{\updates}{\upseq.\diffrunleft.\downseqint}\ &=\ (\sumconst\cdot \ahomsol)[\updvarleft]\\
\paramparikhof{\updates}{\upseqint.\diffrunright.\downseq}\ &=\ (\sumconst\cdot \ahomsol)[\updvarright]
\end{align*}


\rfm{Check whether we track bounded counters in the center.}

To argue that the run $\iterrundef$ is enabled, we study the effect that 
the homogeneous solution has on a counter. 
The following applies to all directions $\mydir\in\set{\myleft, \mycenter, \myright}$, because the reachability constraint is the same for all of them. 
It also holds for concatenations of directions, say from $\acontextinleft$ to $\acontextoutcenter$, due to the equality constraints between the markings reached in the directions. 
(i) If counter $\acounter$ is concrete in input and output, $\at{\acontextindir}{\acounter}, \at{\acontextoutdir}{\acounter}\in\N$, then the updates $\updvardir$ given by the homogeneous solution have effect zero, $\at{(\effof{\updates}\cdot \updvardir)}{\acounter}=0$.
This holds by the definition of $\zeroof{\acontextindir}$ and $\zeroof{\acontextoutdir}$. 
(ii) If the counter is concrete in the input but $\omega$ in the output, the homogeneous solution has a positive effect. 
This holds because the counter is in the support.
(iii) Vice versa, if the counter is $\omega$ in the input but concrete in the output, then the homogeneous solution has a negative effect on the counter.

\rfm{Fix boundedness.}

Enabledness for the run on the left is by Lambert's pumping argument. 
We focus on the center run $\reachruncenterdef$. 
As the NGVAS is in weak Chomsky normal form, the center production creates at most two terminal symbols, say $\anonterm\rightarrow \anngvasp_1.\anngvasp_2$. 
Let the corresponding runs be $\arun_{\aconst, j}$ with $j\in\set{1, 2}$. 
The runs stem from the induction hypothesis or \perfectnessbase, and both of them yield $\anngvasp_j.\acontextin\fires{\arun_{\aconst, j}}\anngvasp_j.\acontextout$. 
By the boundedness information, we moreover have $\anngvasp_1.\acontextin=\acontextincenter$ and $\anngvasp_2.\acontextout=\acontextoutcenter$. 
We consider a counter $\acounter$ that is concrete in the input and distinguish the cases. 
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\paragraph*{Case $\at{\acontextincenter}{\acounter}=\omega$ and $\at{\acontextoutcenter}{\acounter}\in\N$} 
We argue for the enabledness of $\arun_{\aconst, 1}$. 
As counter $\acounter$ is $\omega$ in the input marking, 
the homogeneous solution has a positive effect in the left-hand side run, by (ii) above. 
Hence, by pumping the left-hand side run, we can produce arbitrarily many tokens on $\acounter$.
Using the fact that $\anngvasp_1.\acontextin\fires{\arun_{\aconst, 1}}\anngvasp_1.\acontextout$, the pumping will eventually enable $\arun_{\aconst, 1}$.
For the enabledness of $\arun_{\aconst, 2}$, we reason backwards. 
The counter is concrete in the output marking.
Since moreover $\anngvasp_2.\acontextin\fires{\arun_{\aconst, 2}}\anngvasp_2.\acontextout$ holds, we know that $\arun_{\aconst, 2}$ is enabled from the counter value $\at{\acontextoutcenter}{\acounter}-\at{\vaseffof{\arun_{\aconst, 2}}}{\acounter}$. 
By the marking equation,  this is precisely the value reached by the left-hand side run combined with $\arun_{\aconst, 1}$. 
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\paragraph*{Case $\at{\acontextincenter}{\acounter}\in\N$ and $\at{\acontextoutcenter}{\acounter}\in\N$}. 
We can simply invoke 
$\anngvasp_2.\acontextin\fires{\arun_{\aconst, 2}}\anngvasp_2.\acontextout$ to justify the enabledness of $\arun_{\aconst, 1}$.  
For $\arun_{\aconst, 1}$, we reason backwards as before. 
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\paragraph*{Case $\at{\acontextincenter}{\acounter}\in\N$ and $\at{\acontextoutcenter}{\acounter}=\omega$}. 
The run $\arun_{\aconst, 1}$ is enabled as before. 
We need to have a look at the output marking ....
By (ii) above, we moreover know that the homogeneous solution has a positive effect in the center. 






has en
We argue that $\arun_{\aconst}$

The construction guarantees the following.  
The run $\arun_{\aconst, 1}$ stems from the induction hypothesis. 
If $\anngvasp_1=\anngvasp_2$, then $\arun_{\aconst, 2}$ is the base run from \perfectnessbasenospace. 
If $\anngvasp_1\neq \anngvasp_2$, then also this runs stems from the induction hypothesis. 
The hypothesis and~\perfectnessbase both yield $
\anngvasp_2.\acontextin\fires{\arun_{\aconst, 2}}\anngvasp_2.\acontextout$. 
Moreover, by \rfm{fix} the boundedness information, $\anngvasp_2.\acontextout=\acontextoutcenter$, meaning the counter is concrete in the output marking. 
Combined with the marking equation, these two facts show that the run $\arun_{\aconst, 2}$ . 
We moreover know that the run on the left combined with $\arun_{\aconst, 1}$ yield precisely~$\abound_{\aconst}$. 
The question is whether $\arun_{\aconst, 1}$ is enabled in a marking that leads to $\abound_{\aconst}$. 
With (ii) in the discussion above, the homogeneous solution has a strictly positive effect on the left part.
Moreover, we know that $\arun_{\aconst, 1}$ is enabled for large enough values on counter $\acounter$. 
We can thus select 
We can thus produce tokens
With (i) in the discussion above, the homogeneous solution will have zero effect when combining the left part and the center.
With (ii), it has a strictly positive effect on the left part.
The consequence is that 
 is enabled in a large enough marking and wil
Let $\abound$ be the value of $\acounter$ in 
We analyze the run in the center and assum
With (ii), we have a positive effect on the counter in $\upseq.\diffrunleft.\downseqint$. 
With (iii), we have a negative effect in the pumping phase of the children. 
By \perfectnessbase, 
The runs of the childNGVAS in the center that we take from \perfectnessbase will be enabled for large enough values of $\acounter$. 
For the runs that stem from an invokation of the induction hypothesis, we also have enabledness for large enough input markings.
The problem is that these markings may grow with the iteration count $\acounter$.

\begin{comment}
Recall that in the non-linear case, there was no argument that $\upseq.\diffrunleft$ would have a positive effect and we had to invoke the wide tree theorem.
The problem vanishes here. 
Thanks to linearity, we could set up a different characteristic system that forces a visit to $\acontextinint$. 
In the homogeneous variant, the system forbids counter changes.  
Different from the non-linear case, we now know that $\upseq.\diffrunleft$ has a positive effect. 
The reason is that we constructed the characteristic equations differently so that
\end{comment}


==> iterationlemma_max.tex <==
\section{Iteration Lemma}
\begin{theorem}
Let $\anngvas$ be perfect with restriction $\restrictions = \baseeffect+\periodeffect^*$. 
Let $\baseeffectchoice\in\restrictions$ and let $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Then there are natural numbers $\initconst, \scaleconst\geq 1$ so that for every $\aconst\geq \initconst$ there is a run $\iterrundef\in\runsof{\agram}$ with $\acontextin\fires{\iterrundef}\acontextout$ and $\paramparikhof{\updates}{\iterrundef} =  \baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
We proceed by Noetherian induction on the nesting depth and consider the non-linear case first.
Consider $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Perfectness (P0) gives us a solution $\asol$ to $\chareq{\anngvas}$ with $\asol[\updvar]=\baseeffectchoice$ and a full homogeneous solution $\ahomsol$ to $\homchareq{\anngvas}$ with $\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsection{Non-Linear Case}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Reaching Derivation}
We define $\asol' = \asol+ \maxconst\cdot \ahomsol$ as a new solution to $\chareq{\anngvas}$ ($\ahomsol$ is homogeneous) that is large enough to embed non-negative runs for all instances of all childNGVAS. 
The situation is the following. 
The derivation induced by $\asol'$ will introduce several instances of the terminal symbols $\anngvasp\in\terms$. 
Each instance $\anngvasp$ is a childNGVAS that now has to provide its own derivation. 
There are two requirements on the derivations of $\anngvasp$ we are looking for.
\begin{itemize}
\item[(1)] The run given by the derivation has to be fireable.  
\item[(2)] The derivations of all $\anngvasp$ instances together have to give the number of updates $\asol'[\updvardef]$, in order to guarantee the reachability property we are after.   
\end{itemize}
To achieve (1), our plan is to use the perfectness property~(P4) for all instances of $\anngvasp$ except one. 
Property~(P4) gives us a derivation whose run is guaranteed to be fireable and  correspond to the base vector $\baseeffectdef$ of the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$. 
This, however, does not yet guarantee~(2). 
The solution $\asol'$ may also ask for repetitions of the period vectors in~$\periodeffectdef$. 
For the one instance of $\anngvasp$ that we left out, we obtain the non-negative run by invoking the induction hypothesis with appropriate $\baseeffectchoicedef$ and~$\periodeffectchoicedef$. 
The universal quantification over these vectors in the theorem thus makes it possible to hand over outer constraints on the repetition count of the period vectors to the childNGVAS. 
We turn to the details.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We first define $\maxconst$.
Let $\anngvasp\in\terms$ with $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$.  
To invoke the induction hypothesis, we let $\baseeffectchoicedef$ include the base vector of the restriction $\baseeffectdef$ and repetitions of the period vectors as required by $\asol$. 
For $\periodeffectchoicedef$, we follow the full homogeneous solution:
\begin{align*}
\baseeffectchoicedef\ &=\ \baseeffectdef + \periodeffectdef\cdot \asol[\periodeffectvardef]\\
\periodeffectchoicedef\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
As $\anngvasp$ is perfect by (P6) and $\periodeffectchoicedef\geq 1$ by (P3), we can invoke the induction hypothesis. 
It yields $\initconstdef$ and $\scaleconstdef$ so that for every $\aconst\geq \initconstdef$ we have a run $\iterrunchilddef\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunchilddef}=\baseeffectchoice_{\anngvasp} +  \periodeffectdef \cdot \aconst\cdot \scaleconstdef\cdot \periodeffectchoicedef$.\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
Recall that $\asol'=\asol+\maxconst\cdot \ahomsol$. 
This means the choice of $\maxconst$ has to be independent of the childNGVAS: for every~$\anngvasp$ there has to be $\maxconstdef\geq \initconstdef$ so that $\maxconst=\maxconstdef\cdot \scaleconstdef$ holds. 
An appropriate choice is 
\begin{align*}
\maxconst\ =\ \max\setcond{\initconstdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstdef\ .
\end{align*}
The definition makes sure $\maxconst$ is divisible by every $\scaleconstdef$, and after the division we are left with $\maxconstdef\geq \initconstdef$. 
Note that since the $\initconstdef$ and the $\scaleconstdef$ are positive by the induction hypothesis, $\asol'$ will contain at least one copy of $\ahomsol$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We show that the solution $\asol'$ induces a derivation and discuss its properties.
Since~$\asol'$ solves Esparza-Euler-Kirchhoff, since it contains a copy of $\ahomsol$, and since $\ahomsol[\prodvar]\geq 1$ by~(P2), we can invoke Theorem~\ref{Theorem:EEK} to obtain a derivation $\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach$. 
By Lemma~\ref{Lemma:EEKConverse}, $\asentformreach$ is a sequence of terminal symbols in $\anngvas$. 
Thanks to $\ptof{\anngvas}{\avar_{\prods}, \avar_{\terms}}$, we even have $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$.  
Each terminal in $\asentformreach$ is an update $\anupd\in\Z^{\adim}$ or a childNGVAS $\anngvasp$.
\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We still have to derive runs for the childNGVAS~in~$\asentformreach$. 
Together, we then have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach\xrightarrow{\aprodseqreachterms}\arun_1\ldots \arun_{\cardof{\asentform}} = \reachrun\ .
\end{align*}
The production sequence $\aprodseqreachterms$ concatenates production sequences $\aprodseqreachtermsindex$ for the terminal symbols in $\asentform$. 
If $\seqat{\asentform}{\mathit{i}}$ is an update $\anupd$, then $\aprodseqreachtermsindex=\varepsilon$, the production sequence is empty and $\arun_i=\anupd$. 
If $\seqat{\asentform}{\mathit{i}}$ is the first instance of a childNGVAS $\anngvasp$, then $\aprodseqreachtermsindex$ is a production sequence that yields the run $\arun_i=\arun_{\anngvasp}^{(\maxconstdef)}$ defined above.  
If $\seqat{\asentform}{\mathit{i}}$ is another occurrence of $\anngvasp$, then we use the production sequence which exists by (P4) and results in a run $\arun_i=\baserundef$ with effect $\baseeffectdef$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We show that the run $\reachrun$
transforms the input marking $\asol'[\invar]\sqsubseteq \acontextin$ into the output marking $\asol'[\outvar]\sqsubseteq\acontextout$, as long as we ignore non-negativity.
That the run may fall below zero is a problem we adress later. 
Thanks to the marking equation $\meof{\anngvas}{\invar, \updvar, \outvar}$, all we have to show is that we provide the expected number of updates:
\begin{align}
\paramparikhof{\updates}{\arun}\ = \ \asol'[\avar_{\updates}]\ = \ \restrictto{\asol'[\avar_{\terms}]}{\updates} + \sum_{\anngvasp\in\terms}\asol'[\avar_{\anngvasp, \updates}]\ .\tag{UPDATES-REACH}\label{Equation:UpdatesReach} 
\end{align}
The latter equation is due to $\computeupdatesof{\anngvas}{\termvar, \updvar}$.\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We already argued that $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$. 
As a first consequence, $\paramparikhof{\updates}{\asentformreach}=\restrictto{\asol'[\avar_{\terms}]}{\updates}$, the number of updates in $\reachrun$ that stem from $\asentformreach$ is as expected by $\asol'$. 
As a second consequence, we know that $\asentformreach$ contains  $\asol'[\termvar[\anngvasp]]$ many instances of~$\anngvasp$. 
We show that the runs of all these instances together provide the number of updates $\asol'[\avar_{\anngvasp, \updates}]$.  
Except for the first instance, we used (P4) to construct a run with the number of updates $\baseeffectdef$. 
For the first instance, we used the run $\iterrunchilddefmax$.  
According to $\computeupdatesof{\anngvasp}{\termvar, \updvar}$, we have to show that $\iterrunchilddefmax$ contributes the updates $\baseeffectdef+\periodeffectdef\cdot \asol'[\periodeffectvardef]$. 
This holds with the following reasoning: 
\begin{align*}
&\ \paramparikhof{\updates}{\iterrunchilddefmax} \\
\argument{Induction hypothesis}=&\ \baseeffectchoicedef+\periodeffectdef\cdot \maxconstdef\cdot\scaleconstdef\cdot  \periodeffectchoicedef\\
\argument{Definition of $\baseeffectchoicedef$, $\maxconst$, and~$\periodeffectchoicedef$} =&\ \baseeffectdef+\periodeffectdef\cdot \asol[\periodeffectvardef]+ \periodeffectdef \cdot \maxconst\cdot \ahomsol[\periodeffectvardef]\\
\argument{Linearity and definition of $\asol'$}=&\ \baseeffectdef + \periodeffectdef\cdot \asol'[\periodeffectvardef]\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The run $\reachrun$ is not guaranteed to stay non-negative. 
Neither do the updates in $\asentformreach$ guarantee non-negativity, nor do the runs of the childNGVAS guarantee non-negativity on the counters from $\adimset$. 
We now address this problem. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Pumping Derivation and Embedding}
To enable $\reachrun$, the idea is to surround it by a number of up- and down-pumping sequences.  
This means we wish to repeatedly apply the pumping derivation $\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq$ that exists by perfectness (P5).  
Unfortunately, we cannot even insert a single copy of $\aprodseqpump$ without running the risk of jeopardizing reachability, the fact that the run $\reachrun$ takes the input marking to the output marking. 
The way out is to embed the pumping derivation into a homogeneous solution. 
Embedding the pumping derivation into a homogeneous solution means we provide another derivation 
$\startnonterm\xrightarrow{\aprodseqdiff}\diffrunleft.\startnonterm.\diffrunright$ that can be understood as the difference between the homogeneous solution and the pumping derivation. 
Formally, the two derivations together,  
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq\xrightarrow{\aprodseqdiff}\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq \ ,
\end{align*}
should have the effect prescribed by the homogeneous solution. 
We turn to the details. 
%We make the embedding precise, the construction of an appropriate homogeneous solution and the definition of $\aprodseqdiff$. 
\\\\
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
We begin by inspecting the pumping derivation. 
We can assume $\aprodseqpump=\aprodseqpumpanngvas.\aprodseqpumpterms$ so that $\aprodseqpumpanngvas$ contains the productions of $\anngvas$ and $\aprodseqpumpterms$ contains the productions of the childNGVAS and their descendants. 
This means $\aprodseqpumpanngvas$ will produce a sequence of terminals in $\anngvas$, we have $\startnonterm \xrightarrow{\aprodseqpumpanngvas} \asentformpumpleft.\startnonterm.\asentformpumpright$ with $\asentformpumpleft, \asentformpumpright\in\terms^*$. 
By Lemma~\ref{Lemma:EEKConverse}, we have that $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$.  
We can assume the production sequence $\aprodseqpumpterms$ is a concatenation of sequences $\aprodseqpumptermsindex$, one for every terminal symbol in $\asentformpumpleft.\asentformpumpright$. 
For updates $\seqat{(\asentform_1.\asentform_2)}{\anindex}=\anupd$, this sequence will be empty, $\aprodseqpumptermsindex=\varepsilon$. 
For instances of childNGVAS $\seqat{(\asentform_1.\asentform_2)}{\anindex}=\anngvasp$, perfectness gives us the guarantee that $\startnonterm_{\anngvasp}\xrightarrow{\aprodseqpumptermsindex}\arundefindex$ with $\paramparikhof{\updates}{\arundefindex}\in \restrictionsdef$. 
 \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The homogeneous solution $\ahomsol$ we are given may not be large enough to embed $\aprodseqpump$.  
We scale it to $\sumconst\cdot\ahomsol$ with $\sumconst=\embedconst+\enableconst$. 
The constant $\embedconst$ should be understood as the least natural number large enough so that $\embedconst\cdot \ahomsol$ embeds $\aprodseqpump$. 
Embedding $\aprodseqpump$ is made formal with two requirements we give next. 
These requirements are monotonic: if they hold for $\embedconst\cdot \ahomsol$, then they will hold for $\sumconst\cdot \ahomsol$. 
The first requirement is that we want to be able to subtract $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ from $(\embedconst\cdot \ahomsol)[\prodvar]$.
Even more, in the difference we want to retain a copy of each production to be able to invoke Esparza-Euler-Kirchhoff.  
So $\embedconst$ has to be large enough so that 
\begin{align}
(\embedconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1\ .\tag{R1}\label{Equation:EmbeddingProductions}
\end{align} 
This can be achieved as the productions belong to the support, due to (P2) in perfectness.
An important consequence (that we prove in a moment) is 
\begin{align}
(\embedconst\cdot \ahomsol)[\termvar] - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\geq 0\ . \tag{$\spadesuit$}\label{Equation:EmbeddingConsequence}
\end{align} 
The next requirement is that $\embedconst\cdot \ahomsol$ has to cover the updates produced by $\aprodseqpump$. 
For the updates in $\asentformpumpleft.\asentformpumpright$ that are produced by~$\aprodseqpumpanngvas$, we already have the inequality $(\embedconst\cdot \ahomsol)[\updvar] - \paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright} \geq 0$. 
This is due to~\eqref{Equation:EmbeddingConsequence} combined with $\computeupdatesof{\anngvas}{\termvar, \updvar}$. 
However, we also have to cover the updates produced by the instances of the childNGVAS in $\asentformpumpleft.\asentformpumpright$.  
Consider the childNGVAS~$\anngvasp$ with restriction $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$.  
With Inequality~\eqref{Equation:EmbeddingConsequence} and $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we are sure $(\embedconst\cdot \ahomsol)[\updvardef]$ contains precisely one copy of the base vector $\baseeffectdef$ for every instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
However, the pumping sequence $\aprodseqpump$ may also produce copies of the period vectors. 
Let $\periodeffectpumpdef\in\N^{\periodeffectdef}$ count the period vectors in all runs $\arundefindex$ that belong to an instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$.
For every childNGVAS $\anngvasp\in\terms$, we want 
\begin{align}
(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0\ .\tag{R2} \label{Equation:EmbeddingEffect}
\end{align} 
This can be achieved as the period vectors of all childNGVAS belong to the support,  (P3). \\\\
Requirement~(R3) is that $\embedconst$ should be a multiple of $\maxconst$. 
Since $\maxconst$ is strictly positive and (R1) and (R2) are inequalities, this can be achieved. 
The requirement is needed to use $\maxconst$ as the scaling factor $\scaleconst$ we promised in the induction hypothesis, and will become clearer when we construct the overall run $\iterrunof{\aconst}$. 
\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
Inequality~\eqref{Equation:EmbeddingConsequence} follows from Inequality~\eqref{Equation:EmbeddingProductions} by
\begin{align*}
&\ (\embedconst\cdot \ahomsol)[\termvar] - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\\
\argument{$\ptof{\anngvas}{\prodvar, \termvar}$ and Lemma~\ref{Lemma:EEKConverse}}=&\ \effof{\terms}\cdot (\embedconst\cdot \ahomsol)[\prodvar]  - \effof{\terms}\cdot \paramparikhof{\prods}{\aprodseqpumpanngvas}\\
\argument{Linearity}=&\ \effof{\terms}\cdot ((\embedconst\cdot \ahomsol)[\prodvar]  - \paramparikhof{\prods}{\aprodseqpumpanngvas})\\
\argument{Inequality~\eqref{Equation:EmbeddingProductions} and monotonicity of $\effof{\terms}$}\geq &\ \effof{\terms}\cdot 1\\
\argument{Monotonicity of $\effof{\terms}$}\geq &\ 0\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Difference Derivation}
We now define the production sequence $\aprodseqdiff$. 
We proceed in two steps and first define the productions in $\anngvas$ followed by the productions in the childNGVAS and their descendants, $\aprodseqdiff = \aprodseqdiffanngvas.\aprodseqdiffterms$. 
As we move along, we define the constant $\enableconst$ that has been missing. 
Recall that the goal is to turn the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ into a non-negative run. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The production sequence $\aprodseqdiffanngvas$ should derive a terminal word in $\anngvas$. 
We plan to obtain it with an invokation of Esparza-Euler-Kirchhoff. 
To see that the result applies, note that $(\sumconst\cdot \ahomsol)[\prodvar]$ solves $\homeekof{\anngvas}{\prodvar}$, because $\ahomsol[\prodvar]$ does. 
Moreover, we argued above that also $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
Together, we get that the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
By Requirement~\eqref{Equation:EmbeddingProductions} on $\embedconst$, we have $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1$. 
Theorem~\ref{Theorem:EEK} thus yields $\startnonterm\xrightarrow{\aprodseqdiffanngvas} \asentformdiffleft.\startnonterm.\asentformdiffright$ with $\paramparikhof{\prods}{\aprodseqdiffanngvas} = (\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now construct the production sequence $\aprodseqdiffterms$ that turns the instances of the childNGVAS in $\asentformdiffleft.\asentformdiffright$ into non-negative runs: 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqdiffanngvas}\asentformdiffleft.\startnonterm.\asentformdiffright\xrightarrow{\aprodseqdiffterms}\diffrunleft.\startnonterm.\diffrunright\ . 
\end{align*}
We proceed as in the construction of the reaching run in the previous section.
For the first instance of the childNGVAS~$\anngvasp$ in~$\asentformdiffleft.\asentformdiffright$, we use the derivation of a run $\iterrunpchilddefenable$ that is given by the induction hypothesis. 
The task of this run is to compensate the $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0$ excess in period vectors from the pumping derivation, and the definition will be given in a moment. 
For the remaining occurrences of $\anngvasp$, we use the derivation of the run $\baserundef$ that we have by (P4).\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To construct $\iterrunpchilddefenable$ that compensates the excess in period vectors, we invoke the induction hypothesis with the following vectors: 
\begin{align*}
\baseeffectchoicedef'\ &=\ \baseeffectdef + \periodeffectdef\cdot [ (\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef]\\
\periodeffectchoicedef'\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
The definition uses Requirement~\eqref{Equation:EmbeddingEffect} on $\embedconst$, the choice of period vectors $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef$ has to be non-negative. 
As $\anngvasp$ is perfect by~(P6) and as $\periodeffectchoicedef'\geq 1$ by (P3), the induction hypothesis applies and yields $\initconstpdef$ and $\scaleconstpdef$ so that for every $\aconst\geq \initconstpdef$ we have a run $\iterrunpdefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunpdefof{\aconst}}=\baseeffectchoice_{\anngvasp}' +  \periodeffectdef\cdot \aconst \cdot \scaleconstpdef\cdot \periodeffectchoicedef'$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We define $\enableconst$ as 
\begin{align*}
\enableconst\ =\ \maxconst\cdot \max\setcond{\initconstpdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstpdef\ .
\end{align*}
The $\enableconstdef$ we have been looking for is $\enableconst$ divided by $\scaleconstpdef$. 
We use $\maxconst$ for divisibility reasons, like we have done with $\embedconst$. 
Apart from that, the definition is similar to the one for $\maxconst$ itself. 
\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To sum up, we now have $\startnonterm\rightarrow^*\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq$ using the production sequence $\aprodseqpump.\aprodseqdiff$ with $\aprodseqpump = \aprodseqpumpanngvas.\aprodseqpumpterms$ and $\aprodseqdiff=\aprodseqdiffanngvas.\aprodseqdiffterms$. 
We check that the number of updates in the terminal sequence is the one expected by $\sumconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}\ =\
(\sumconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-PUMP-DIFF}\label{Equation:UpdatesPumpDiff}
\end{align} 
We rely on $\computeupdatesof{\anngvas}{\termvar, \updvar}$ to see that 
\begin{align*}
&(\sumconst\cdot\ahomsol)[\updvar]\ =\ 
 \restrictto{(\sumconst\cdot\ahomsol)[\termvar]\ }{\updates}+\sum_{\anngvasp\in\terms}(\sumconst\cdot\ahomsol)[\updvardef]\ .
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We first show that
\begin{align*}
\paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright.\asentformdiffleft.\asentformdiffright}\ = \ \restrictto{(\sumconst\cdot\ahomsol)[\termvar]\ }{\updates}\ .
\end{align*}
The equation says that the number of updates produced directly by $\anngvas$ is as expected by the scaled homogeneous solution. 
With Lemma~\ref{Lemma:EEKConverse} and $\ptof{\anngvas}{\prodvar, \termvar}$, it suffices to realize that 
\begin{align*}
&\ \paramparikhof{\prods}{\aprodseqpumpanngvas}+\paramparikhof{\prods}{\aprodseqdiffanngvas}\\ 
\argument{Definition $\aprodseqdiffanngvas$}=&\ \paramparikhof{\prods}{\aprodseqpumpanngvas}+ (\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\\
 =&\ (\sumconst\cdot \ahomsol)[\prodvar]\ .\\
\end{align*}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now consider the childNGVAS $\anngvasp$ with restriction $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$. 
The task is to show that $\aprodseqpumpterms$ and $\aprodseqdiffterms$ together create precisely $(\sumconst\cdot\ahomsol)[\updvardef]$ many updates 
in the runs derived from the $\anngvasp$ instances. 
By $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we have
\begin{align*}
(\sumconst\cdot\ahomsol)[\updvardef]\ =\ \baseeffectdef\cdot (\sumconst\cdot\ahomsol)[\termvar[\anngvasp]] - \periodeffectdef\cdot (\sumconst\cdot\ahomsol)[\periodeffectvardef]\ .
\end{align*}
With the argument from the previous paragraph, we know that $\aprodseqpumpanngvas$ and $\aprodseqdiffanngvas$ together create precisely $(\sumconst\cdot\ahomsol)[\termvar[\anngvasp]]$ many instances of $\anngvasp$. 
Moreover, the run we derive from such an instance using $\aprodseqpumpterms$ and $\aprodseqdiffterms$ contains at least the number of updates prescribed by the base vector $\baseeffectdef$. 
The run may contain further updates that together make up copies of the period vectors. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
It remains to check that the expected number of copies of the period vectors $(\sumconst\cdot\ahomsol)[\periodeffectvardef]$  coincides with the number of copies produced by $\aprodseqpumpterms$ and $\aprodseqdiffterms$. 
In $\aprodseqpumpterms$, we produce $\periodeffectpumpdef$ many copies.
In $\aprodseqdiffterms$, there is a single instance of $\anngvasp$ that produces copies of the period vectors. By the induction hypothesis, it produces $(\embedconst\cdot \ahomsol)[\periodeffectvardef]-\periodeffectpumpdef$ copies with $\baseeffectchoicedef'$ plus an additional $\enableconstdef\cdot \scaleconstpdef\cdot \periodeffectchoicedef'$ many copies. 
Then 
\begin{align*}
&\ \periodeffectpumpdef\quad +\quad  (\embedconst\cdot \ahomsol)[\periodeffectvardef]-\periodeffectpumpdef\\
&\quad +\quad \enableconstdef\cdot \scaleconstpdef\cdot \periodeffectchoicedef'\\
\argument{$\enableconst=\enableconstdef\cdot \scaleconstpdef$} =& \ (\embedconst\cdot \ahomsol)[\periodeffectvardef] + \enableconst\cdot \periodeffectchoicedef'\\
\argument{Definition $\periodeffectchoicedef'$} =& \ (\embedconst\cdot \ahomsol)[\periodeffectvardef] + (\enableconst\cdot \ahomsol)[\periodeffectvardef]\\
\argument{Definition $\sumconst$} =& \ (\sumconst\cdot \ahomsol)[\periodeffectvardef]\ . 
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Pumping}
We now make the reaching run fireable by surrounding the reaching derivation by repetitions of the pumping derivation and the difference derivation.  
Here is what we know.
The runs $\upseq$ and $\downseq$ generated by the pumping derivation have a strictly positive resp.~a strictly negative effect on the unbounded counters.
Together, the runs $\upseq.\downseq$ and $\diffrunleft.\diffrunright$ from the pumping derivation and from the difference derivation have effect zero on the unbounded counters.
This means $\upseq.\diffrunleft.\diffrunright$ will have a strictly positive effect on the unbounded counters.
Repeating the pumping and the difference derivation in a naive way then yields
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^k}\upseq^k.\startnonterm.\downseq^k\ 
\xrightarrow{\aprodseqdiff^k}&\ \upseq^k.\diffrunleft^k.\startnonterm.\diffrunright^k.\downseq^k \\
\xrightarrow{\aprodseqreach}&\ \upseq^k.\diffrunleft^k.\reachrun.\diffrunright^k.\downseq^k\ .
\end{align*}
The problem is that $\diffrunleft$ and $\diffrunright$ are not placed next to each other, but we first generate the copies of $\diffrunleft$ and later the copies of $\diffrunright$. 
Unfortunately, there is no guarantee that $\upseq.\diffrunleft$ has a positive effect on the unbounded counters.  \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
The way out is to use the wide tree theorem on the difference derivation. 
Then the hurdle required by the copies of the difference run will only grow logarithmically in the number of tokens produced by the pumping run.
This will eventually make the run fireable. 
We turn to the details.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We first argue that the wide tree theorem applies. 
By definition, the NGVAS~$\anngvas$ is non-linear, strongly connected, and only has useful non-terminals. 
We already observed that $\prodvec = \paramparikhof{\prods}{\aprodseqdiffanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
We can thus arrange $\aconst$ copies of $\prodvec$ in a parse tree $\atreeofdef$ of height $\ceilof{1+\log \aconst}\cdot \normof{\prodvec}$, for every $\aconst\geq 1$. 
Let the yield by $\yieldof{\atreeofdef}=\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}$. 
The theorem moreover guarantees that for every prefix $\asentform$ of $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$, the number of incomplete copies of $\termvec=\effof{\terms}\cdot \prodvec$ is bounded by $\ceilof{1+\log \aconst}$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the derivation we are after, it remains to turn every copy of $\termvec$ in $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$ into a run using $\aprodseqdiffterms$. 
We have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^{\aconst}}\upseq^{\aconst}.\startnonterm.\downseq^{\aconst}\xrightarrow{\text{wide tree theorem}}&\ \upseq^{\aconst}.\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqdiffterms^{\aconst}}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\startnonterm.\arun_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqreach}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\reachrun.\arun_{\aconst, 2}.\downseq^{\aconst}\ =\ \iterrundef\ .
\end{align*}
These are runs $\iterrundef$ we are after.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
It remains to determine a constant~$\aconst_0$ from which the runs $\iterrundef$ stay non-negative. 
We estimate the hurdle we have to meet with the up-pumping sequence. 
We first consider the incomplete copies of~$\termvec$. 
We iterate over all sentential forms~$\asentform$ that could result from them and over all runs $\arun$ that could be derived from $\asentform$ using $\aprodseqdiffterms$, and determine the maximal hurdle:
\begin{align*}
\maxhurdlediff\ &= \ \max\setcond{\hurdleof{\arun}}{\paramparikhof{\terms}{\asentform}<\termvec\text{ and } \asentform\xrightarrow{\aprodseqdiffterms}\arun}\ .
\end{align*}
We slightly abuse the notation here. 
Actually, we do not use the full $\aprodseqdiffterms$ but only the productions for the childNGVAS~$\anngvasp$ that occur in~$\asentform$. 
For one instance of $\anngvasp$, there is a choice of whether to derive $\baserundef$ or $\arun'^{(\enableconst)}_{\anngvasp}$. 
The above notation is meant to cover all cases. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
Recall that $\upseq.\diffrunleft.\diffrunright$ has a strictly positive effect on the unbounded counters. 
This means a complete copy of $\termvec$ does not add to the hurdle. 
So the maximal hurdle we have to expect due to incomplete copies of $\termvec$ is $\maxhurdlediff\cdot \ceilof{1+\log \aconst}$. 
To enable the above run, we still have to add $\hurdleof{\reachrun}$.
With this analysis, the run  $\iterrundef$ will stay non-negative as long as $\aconst\geq \aconst_0$, with $\aconst_0$ the least natural number satisfying
\begin{align*}
\aconst_0\quad \geq\quad \maxhurdlediff\cdot \ceilof{1+\log \aconst_0}\ +\ \hurdleof{\reachrun}\ . \\
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that each run $\iterrundef$ with $\aconst\geq \aconst_0$ has the properties formulated in the iteration lemma: 
it solves reachability and uses a number of updates that is as desired.
Thanks to the marking equations, we can study these properties on a Parikh equivalent run. 
We use
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\reachrun.\diffrunright^\aconst.\downseq^{\aconst}}\ =\ \ \paramparikhof{\updates}{\iterrundef}\ .
\end{align*}
To see the equality, note that the tree $\atreeofdef$ has the same productions as $\aprodseqdiffanngvas^k$. 
By Lemma~\ref{Lemma:EEKConverse}, we have $\paramparikhof{\terms}{\asentformdiffleft^\aconst.\asentformdiffright^\aconst}=\paramparikhof{\terms}{\asentform_{\aconst, 1}.\asentform_{\aconst, 2}}$. 
We then apply the same derivations to the childNGVAS in these sentential forms.
 \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that we solve reachability. 
Since $\asol'$ is a solution to the characteristic equations and $\sumconst\cdot \ahomsol$ as well as $\maxconst\cdot \ahomsol$ are solutions to the homogeneous variant of the characteristic equations,  also $\asol''=\asol'+\aconst\cdot \sumconst\cdot \ahomsol$ solves the charateristic equations.
Due to $\meof{\anngvas}{\invar, \updvar, \outvar}$, this in particular means $\asol''[\invar]+\effof{\updates}\cdot \asol''[\updvar]=\asol''[\outvar]$. 
By \eqref{Equation:UpdatesReach}, we have  $\paramparikhof{\updates}{\reachrun}=\asol'[\updvar]$. 
By \eqref{Equation:UpdatesPumpDiff}, the equality  $\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}=\sumconst\cdot \ahomsol[\updvar]$ holds.
Hence, 
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\reachrun.\diffrunright^\aconst.\downseq^{\aconst}}=\asol''[\updvar]\ .
\end{align*} 
This means the Parikh vector satisfies the marking equation.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We have to show that the number of updates in the run has the form $\baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$, for some $\scaleconst$. 
We just argued that the number of updates is $\asol''[\updvar]$, so we can calculate as follows:
\begin{align*}
&\ \asol''[\updvar]\\
\argument{Definition $\asol''$}=&\ \asol'[\updvar]+\aconst\cdot \sumconst\cdot \ahomsol[\updvar]\\
\argument{Definition $\asol'$}=&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot \sumconst\cdot \ahomsol[\updvar]\\
\argument{Definition $\sumconst$}=&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot (\embedconst+\enableconst)\cdot \ahomsol[\updvar]\\
\argument{(R3) for $\embedconst$}=&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot (\aconst_1\cdot\maxconst+\enableconst)\cdot \ahomsol[\updvar]\\
\argument{Definition $\enableconst$}=&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot (\aconst_1\cdot\maxconst+\aconst_2\cdot \maxconst)\cdot \ahomsol[\updvar]\\
=&\ \asol[\updvar]+(1+\aconst\cdot (\aconst_1+\aconst_2))\cdot \maxconst\cdot \ahomsol[\updvar]\\
\argument{$\asol[\updvar]=\baseeffectchoice$}=&\ \baseeffectchoice+(1+\aconst\cdot (\aconst_1+\aconst_2))\cdot \maxconst\cdot \ahomsol[\updvar]\\
\argument{$\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$}=&\ 
\baseeffectchoice+(1+\aconst\cdot (\aconst_1+\aconst_2))\cdot \maxconst \cdot \periodeffect\cdot \periodeffectchoice\ .
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

\subsection{Linear Case}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

%\rfm{Warum die Menge $R$: Iterieren unten und oben klappt sonst nicht unabhängig voneinander.}



==> iterationlemma_sim.tex <==
\section{Iteration Lemma}\label{Section:IterationLemma}
\begin{theorem}
Let $\anngvas$ be perfect with $\restrictions = \baseeffect+\periodeffect^*$. 
Let $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Then there are $\initconst, \scaleconst\geq 1$ so that for every $\aconst\geq \initconst$ there is a run $\iterrun{\aconst}\in\runsof{\anngvas}$ with $\acontextin\fires{\iterrun{\aconst}}\acontextout$ and $\paramparikhof{\updates}{\iterrun{\aconst}} =  \baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
We proceed by Noetherian induction on the nesting depth and consider the non-linear case first.
Consider $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Perfectness \perfectnesssol gives us a solution $\asol$ to $\chareq{\anngvas}$ with $\asol[\updvar]=\baseeffectchoice$ and a full homogeneous solution $\ahomsol$ to $\homchareq{\anngvas}$ with $\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsection{Non-Linear Case}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Reaching Derivation}
We define $\asol' = \asol+ \maxconst\cdot \ahomsol$ as a new solution to $\chareq{\anngvas}$ ($\ahomsol$ is homogeneous) that is large enough to embed non-negative runs for all instances of all childNGVAS. 
The situation is the following. 
The derivation induced by $\asol'$ will introduce several instances of the terminal symbols $\anngvasp\in\terms$. 
Each instance $\anngvasp$ is a childNGVAS that now has to provide its own derivation. 
There are two requirements on the derivations of $\anngvasp$ we are looking for.
\begin{itemize}
\item[(1)] The run given by the derivation has to be fireable.  
\item[(2)] The derivations of all $\anngvasp$ instances together have to give the number of updates $\at{\asol'}{\updvardef}$, in order to guarantee the reachability property we are after.   
\end{itemize}
To achieve (1), our plan is to use the perfectness property~\perfectnessbase for all instances of $\anngvasp$ except one. 
Property~\perfectnessbase gives us a derivable run that is guaranteed to be enabled in the input marking and correspond to the base vector $\baseeffectdef$ of the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$. 
This, however, does not yet guarantee~(2). 
The solution $\asol'$ may also ask for repetitions of the period vectors in~$\periodeffectdef$. 
For the one instance of $\anngvasp$ that we left out, we obtain the non-negative run by invoking the induction hypothesis with appropriate $\baseeffectchoicedef$ and~$\periodeffectchoicedef$. 
The universal quantification over these vectors in the theorem thus makes it possible to hand over outer constraints on the repetition count of the period vectors to the childNGVAS. 
We turn to the details.
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

We first define $\maxconst$.
Let $\anngvasp\in\terms$ with $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$.  
To invoke the induction hypothesis, we let $\baseeffectchoicedef$ include the base vector of the restriction $\baseeffectdef$ and repetitions of the period vectors as required by $\asol$. 
For $\periodeffectchoicedef$, we follow the full homogeneous solution:
\begin{align*}
\baseeffectchoicedef\ &=\ \baseeffectdef + \periodeffectdef\cdot \asol[\periodeffectvardef]\\
\periodeffectchoicedef\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
As $\anngvasp$ is perfect by (P6) and $\periodeffectchoicedef\geq 1$ by (P3), we can invoke the induction hypothesis. 
It yields $\initconstdef$ and $\scaleconstdef$ so that for every $\aconst\geq \initconstdef$ we have a run $\iterrundefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrundefof{\aconst}}=\baseeffectchoice_{\anngvasp} +  \periodeffectdef \cdot \aconst\cdot \scaleconstdef\cdot \periodeffectchoicedef$.
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

Recall that $\asol'=\asol+\maxconst\cdot \ahomsol$. 
This means the choice of $\maxconst$ has to be independent of the childNGVAS: for every~$\anngvasp$ there has to be $\maxconstdef\geq \initconstdef$ so that $\maxconst=\maxconstdef\cdot \scaleconstdef$ holds. 
An appropriate choice for $\maxconst$ is 
\begin{align*}
\max\setcond{\initconstdef, \initconstppdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstdef\cdot \scaleconstppdef\ .
\end{align*}
The definition makes sure $\maxconst$ is divisible by every $\scaleconstdef$, and after the division we are left with $\maxconstdef\geq \initconstdef$. 
That we also need the $\initconstppdef$ and the $\scaleconstppdef$ will become clear when we discuss the offset derivation further below. 
Note that since the $\initconstdef$ and the $\scaleconstdef$ are positive by the induction hypothesis, $\asol'$ will contain at least one copy of $\ahomsol$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We show that $\asol'$ induces a derivation and discuss its properties.
Since~$\asol'$ solves Esparza-Euler-Kirchhoff, since it contains a copy of $\ahomsol$, and since $\ahomsol[\prodvar]\geq 1$ by~\perfectnessprods in perfectness, we can invoke Theorem~\ref{Theorem:EEK} to obtain a derivation $\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach$. 
By Lemma~\ref{Lemma:EEKConverse}, $\asentformreach$ is a sequence of terminal symbols in $\anngvas$. 
Thanks to $\ptof{\anngvas}{\avar_{\prods}, \avar_{\terms}}$, we even have $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$.  
Each terminal in $\asentformreach$ is an update $\anupd\in\Z^{\adim}$ or a childNGVAS $\anngvasp$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We still have to derive runs for the childNGVAS~in~$\asentformreach$. 
Together, we then have 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach
\text{ and }\reachrun\in\runsof{\asentformreach}.
\end{align*}
Recall that $\runsof{\asentformreach}$ concatenates runs of the terminals in $\asentformreach$, so $\reachrun=\arun_1\ldots\arun_{\cardof{\asentformreach}}$.  
If $\at{\asentform}{\mathit{i}}$ is an update $\anupd$, then $\arun_i=\anupd$. 
If $\at{\asentform}{\mathit{i}}$ is the first instance of a childNGVAS $\anngvasp$, then $\arun_i=\arun_{\anngvasp}^{(\maxconstdef)}$ as defined above.  
If $\at{\asentform}{\mathit{i}}$ is another occurrence of $\anngvasp$, then we use \perfectnessbase and get $\arun_i=\baserundef$ with effect $\baseeffectdef$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

Thanks to the marking equation $\meof{\anngvas}{\invar, \updvar, \outvar}$, the number of updates given by $\at{\asol'}{\avar_{\updates}}$ transforms 
$\at{\asol'}{\invar}\sqsubseteq \acontextin$ into $\at{\asol'}{\outvar}\sqsubseteq\acontextout$. 
In the appendix, we show that $\reachrun$ has precisely this number of updates:
\begin{align}
\paramparikhof{\updates}{\reachrun}\ = \ \at{\asol'}{\avar_{\updates}}\ .\tag{UPDATES-REACH}\label{Equation:UpdatesReach} 
\end{align}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The run $\reachrun$ is not guaranteed to stay non-negative. 
Neither do the updates in $\asentformreach$ guarantee non-negativity, nor do the runs of the childNGVAS guarantee non-negativity on the counters from $\adimset$. 
We now address this problem. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Pumping Derivation and Embedding}
To enable $\reachrun$, the idea is to surround it by a number of up-pumping and down-pumping runs.  
So we wish to repeatedly apply the pumping derivation $\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq$ that exists by~\perfectnesspumpingnospace.  
Unfortunately, we cannot even insert one copy of $\aprodseqpump$ without running the risk of jeopardizing reachability. 
The way out is to embed the pumping derivation into a homogeneous solution. 
Embedding the pumping derivation into a homogeneous solution means we provide another derivation 
$\startnonterm\xrightarrow{\aprodseqdiff}\diffrunleft.\startnonterm.\diffrunright$ that should be understood as the difference between the homogeneous solution and the pumping derivation. 
Formally, the two derivations together,  
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq\xrightarrow{\aprodseqdiff}\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq \ ,
\end{align*}
have the effect prescribed by the homogeneous solution. 
In this section, we make the notion of embedding precise. 
%We make the embedding precise, the construction of an appropriate homogeneous solution and the definition of $\aprodseqdiff$. 
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------

We first inspect the pumping runs. 
There is a derivation $\startnonterm \xrightarrow{\aprodseqpumpanngvas} \asentformpumpleft.\startnonterm.\asentformpumpright$ so that $\upseq.\downseq$ belongs to $\runsof{\asentformpumpleft.\asentformpumpright}$. 
By the definition of $\runsof{\asentform}$, we know that the run derived for $\at{(\asentform_1.\asentform_2)}{\anindex}=\anngvasp$ satisfies $\restrictionsdef$. 
Moreover, by Lemma~\ref{Lemma:EEKConverse}, $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

The homogeneous solution $\ahomsol$ we are given may not be large enough to embed $\aprodseqpump$.  
We scale it to $\sumconst\cdot\ahomsol$ with $\sumconst=\embedconst+\enableconst$. 
The constant $\embedconst$ should be understood as the least natural number large enough so that $\embedconst\cdot \ahomsol$ embeds $\aprodseqpump$. 
Embedding $\aprodseqpump$ is made formal with two requirements we give next. 
These requirements are monotonic: if they hold for $\embedconst\cdot \ahomsol$, then they will hold for $\sumconst\cdot \ahomsol$. 
The first requirement is that we want to be able to subtract $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ from $\at{(\embedconst\cdot \ahomsol)}{\prodvar}$.
Even more, in the difference we want to retain a copy of each production to be able to invoke Esparza-Euler-Kirchhoff.  
This means $\embedconst$ has to be large enough so that 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\prodvar} - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1\ .\tag{R1}\label{Equation:EmbeddingProductions}
\end{align} 
This can be achieved as the productions belong to the support, due to \perfectnessprodsnospace.
An important consequence is 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\termvar} - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\geq 0\ . \tag{$*$}\label{Equation:EmbeddingConsequence}
\end{align} 
The next requirement is that $\embedconst\cdot \ahomsol$ has to cover the updates in $\upseq.\downseq$. 
For the updates that are already present in $\asentformpumpleft.\asentformpumpright$, we have the inequality $\at{(\embedconst\cdot \ahomsol)}{\updvar} - \paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright} \geq 0$. 
This is due to~\eqref{Equation:EmbeddingConsequence} combined with $\computeupdatesof{\anngvas}{\termvar, \updvar}$. 
We also have to cover the updates produced by the instances of the childNGVAS in $\asentformpumpleft.\asentformpumpright$.  
Consider the childNGVAS~$\anngvasp$ with $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$.  
By~\eqref{Equation:EmbeddingConsequence} and $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we are sure $\at{(\embedconst\cdot \ahomsol)}{\updvardef}$ contains precisely one copy of the base vector $\baseeffectdef$ for every instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
However, $\aprodseqpump$ may also produce copies of the period vectors. 
Let $\periodeffectpumpdef\in\N^{\periodeffectdef}$ count the period vectors in all runs that belong to an instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
For every childNGVAS $\anngvasp\in\terms$, we want 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\periodeffectvardef} - \periodeffectpumpdef\geq 0\ .\tag{R2} \label{Equation:EmbeddingEffect}
\end{align} 
This can be achieved as the period vectors of all childNGVAS belong to the support, \perfectnesschildperiodsnospace. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Difference Derivation}
We now define the production sequence $\aprodseqdiff$. 
We proceed in two steps and first define the productions in $\anngvas$ followed by the productions in the childNGVAS and their descendants, $\aprodseqdiff = \aprodseqdiffanngvas.\aprodseqdiffterms$. 
As we move along, we define the constant $\enableconst$ that has been missing. 
Recall that the goal is to turn the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ into a non-negative run. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The production sequence $\aprodseqdiffanngvas$ should derive a terminal word in $\anngvas$. 
We plan to obtain it with an invokation of Esparza-Euler-Kirchhoff. 
To see that the result applies, note that $(\sumconst\cdot \ahomsol)[\prodvar]$ solves $\homeekof{\anngvas}{\prodvar}$, because $\ahomsol[\prodvar]$ does. 
Moreover, we argued above that also $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
Together, we get that the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
By Requirement~\eqref{Equation:EmbeddingProductions} on $\embedconst$, we have $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1$. 
Theorem~\ref{Theorem:EEK} thus yields $\startnonterm\xrightarrow{\aprodseqdiffanngvas} \asentformdiffleft.\startnonterm.\asentformdiffright$ with $\paramparikhof{\prods}{\aprodseqdiffanngvas} = (\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now construct the production sequence $\aprodseqdiffterms$ that turns the instances of the childNGVAS in $\asentformdiffleft.\asentformdiffright$ into non-negative runs: 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqdiffanngvas}\asentformdiffleft.\startnonterm.\asentformdiffright\xrightarrow{\aprodseqdiffterms}\diffrunleft.\startnonterm.\diffrunright\ . 
\end{align*}
We proceed as in the construction of the reaching run in the previous section.
For the first instance of the childNGVAS~$\anngvasp$ in~$\asentformdiffleft.\asentformdiffright$, we use the derivation of a run $\iterrunpdefenable$ that is given by the induction hypothesis. 
The task of this run is to compensate the $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0$ excess in period vectors from the pumping derivation, and the definition will be given in a moment. 
For the remaining occurrences of $\anngvasp$, we use the derivation of the run $\baserundef$ that we have by (P4).\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To construct $\iterrunpdefenable$ that compensates the excess in period vectors, we invoke the induction hypothesis with the following vectors: 
\begin{align*}
\baseeffectchoicedef'\ &=\ \baseeffectdef + \periodeffectdef\cdot [ (\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef]\\
\periodeffectchoicedef'\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
The definition uses Requirement~\eqref{Equation:EmbeddingEffect} on $\embedconst$, the choice of period vectors $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef$ has to be non-negative. 
As $\anngvasp$ is perfect by~(P6) and as $\periodeffectchoicedef'\geq 1$ by (P3), the induction hypothesis applies and yields $\initconstpdef$ and $\scaleconstpdef$ so that for every $\aconst\geq \initconstpdef$ we have a run $\iterrunpdefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunpdefof{\aconst}}=\baseeffectchoice_{\anngvasp}' +  \periodeffectdef\cdot \aconst \cdot \scaleconstpdef\cdot \periodeffectchoicedef'$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We define $\enableconst$ in analogy to $\maxconst$ from above as 
\begin{align*}
\enableconst\ =\ \max\setcond{\initconstpdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstpdef\ .
\end{align*}
The $\enableconstdef$ we have been looking for is $\enableconst$ divided by $\scaleconstpdef$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To sum up, we now have $\startnonterm\rightarrow^*\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq$ using the production sequence $\aprodseqpump.\aprodseqdiff$ with $\aprodseqpump = \aprodseqpumpanngvas.\aprodseqpumpterms$ and $\aprodseqdiff=\aprodseqdiffanngvas.\aprodseqdiffterms$. 
We check that the number of updates in the terminal sequence is the one expected by $\sumconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}\ =\
(\sumconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-PUMP-DIFF}\label{Equation:UpdatesPumpDiff}
\end{align} 

% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Offset Derivation}
If we surround the reaching derivation with $\aconst$ many repetitions of the pumping derivation and the difference derivation, we obtain $\maxconst +\aconst\cdot \sumconst$ many repetitions of the homogeneous solution. 
This does not yield the $\aconst\cdot \scaleconst$ number of repetitions of  $\periodeffectchoice$ that we promised in the induction hypothesis, because the $\maxconst$ factor acts as an offset. 
We have to insert another $\aconst-1$ copies of $\maxconst\cdot \ahomsol$ to arrive at $\aconst\cdot (\sumconst+\maxconst)$ many repetitions of the homogeneous solution. 
We now show how to construct what we call an offset derivation, a derivation that corresponds to $\maxconst\cdot \ahomsol$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the offset derivation, we define the production sequence $\aprodseqoffset=\aprodseqoffsetanngvas.\aprodseqoffsetterms$. 
We obtain $\aprodseqoffsetanngvas$  from $(\maxconst\cdot\ahomsol)[\prodvar]$ using Esparza-Euler-Kirchhoff. 
The corresponding derivation $\startnonterm\xrightarrow{\aprodseqoffsetanngvas}\asentformoffsetleft.\startnonterm.\asentformoffsetright$ satisfies $(\maxconst\cdot\ahomsol)[\termvar]=\paramparikhof{\terms}{\asentformoffsetleft.\asentformoffsetright}$. 
The sequence $\aprodseqoffsetterms$ is a concatenation of sequences  $\aprodseqoffsettermsindex$, one for every terminal in $\asentformoffsetleft.\asentformoffsetright$. 
For updates, these sequences are empty. 
For instances of childNGVAS $\anngvasp$ that are not the first ones, we use (P4) in perfectness. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the first instance of $\anngvasp$, we invoke the induction hypothesis with 
\begin{align*}
\baseeffectchoicedef''\ =\ \baseeffectdef \qquad\text{and}\qquad 
\periodeffectchoicedef''\ =\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
It yields $\initconstppdef$ and $\scaleconstppdef$ so that for all $\aconst\geq \initconstppdef$ there is a run $\iterrunppdefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunppdefof{\aconst}}=\baseeffectchoice_{\anngvasp}'' +  \periodeffectdef\cdot \aconst \cdot \scaleconstppdef\cdot \periodeffectchoicedef''$. 
We now define $\offsetconstdef$ as $\maxconst$ divided by $\scaleconstppdef$. 
This yields an integer, because $\maxconst$ is defined as a product with $\scaleconstppdef$. 
Moreover, we have $\offsetconstdef\geq \initconstppdef$ as we included the $\initconstppdef$ in the definition of $\maxconst$. 
For the first instance of~$\anngvasp$, we then use the derivation of the run $\iterrunppdefoffset$.
\\\\
Together, we now have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqoffsetanngvas}\asentformoffsetleft.\startnonterm.\asentformoffsetright\xrightarrow{\aprodseqoffsetterms}\offsetrunleft.\startnonterm.\offsetrunright\ .\\
\end{align*}
It remains to check that the number of updates in $\offsetrunleft.\offsetrunright$ is as expected by $\maxconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\offsetrunleft.\offsetrunright}\ =\
(\maxconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-OFFSET}\label{Equation:UpdatesOffset}
\end{align}
The reasoning is very similar to the reasoning for the reaching derivation and the reasoning for the combination of pumping and difference derivation. 
The critical point is to show that the repetitions of the period vectors are as expected. 
The vector $\baseeffectchoicedef''$ does not contain copies of the period vectors.
Hence, we only get copies prescribed by $\offsetconstdef\cdot \scaleconstppdef\cdot \periodeffectchoicedef''$. 
As $\offsetconstdef\cdot \scaleconstppdef=\maxconst$ and $\periodeffectchoicedef''\ =\ \ahomsol[\periodeffectvardef]$, we are done. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Pumping}
We now make the reaching run fireable by surrounding the reaching derivation by repetitions of the pumping derivation, the difference derivation, and the offset derivation.  
Here is what we know.
\rfm{This is overly simplified and written with a counter in mind that is concrete in the input and output marking, but contained in the set of unbounded counters. While this qualification is needed, the text may transport the idea well.}
The runs $\upseq$ and $\downseq$ generated by the pumping derivation have a strictly positive resp.~a strictly negative effect on the unbounded counters.
Together, the runs $\upseq.\downseq$ and $\diffrunleft.\diffrunright$ from the pumping derivation and from the difference derivation have effect zero on the unbounded counters.
This means $\upseq.\diffrunleft.\diffrunright$ will have a strictly positive effect on the unbounded counters.
Also $\offsetrunleft.\offsetrunright$ has a zero effect on the unbounded counters. 
Repeating the pumping, the difference, and the offset derivation in a naive way then yields
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^k}&\ \upseq^k.\startnonterm.\downseq^k\\
\xrightarrow{\aprodseqdiff^k}&\ \upseq^k.\diffrunleft^k.\startnonterm.\diffrunright^k.\downseq^k \\
\xrightarrow{\aprodseqoffset^{k-1}}&\ \upseq^k.\diffrunleft^k.\offsetrunleft^{k-1}.\startnonterm.\offsetrunright^{k-1}.\diffrunright^k.\downseq^k \\
\xrightarrow{\aprodseqreach}&\ \upseq^k.\diffrunleft^k.\offsetrunleft^{k-1}.\reachrun.\offsetrunright^{k-1}.\diffrunright^k.\downseq^k\ .
\end{align*}
The problem is that $\diffrunleft$ and $\diffrunright$ are not placed next to each other, but we first generate the copies of $\diffrunleft$ and later the copies of $\diffrunright$. 
Unfortunately, there is no guarantee that $\upseq.\diffrunleft$ has a positive effect on the unbounded counters. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

The way out is to use the wide tree theorem on the difference derivation. 
Then the hurdle required by the copies of the difference run will only grow logarithmically in the number of tokens produced by the pumping run.
This will eventually enable the run. 
We turn to the details. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

We first argue that the wide tree theorem applies. 
By definition, the NGVAS~$\anngvas$ is non-linear, strongly connected, and only has useful non-terminals. 
We already observed that $\prodvec = \paramparikhof{\prods}{\aprodseqdiffanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
We can thus arrange $\aconst$ copies of $\prodvec$ in a parse tree $\atreedef$ of height $\ceilof{1+\log \aconst}\cdot \normof{\prodvec}$, for every $\aconst\geq 1$. 
Let the yield by $\yieldof{\atreedef}=\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}$. 
The theorem moreover guarantees that for every prefix $\asentform$ of $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$, the number of incomplete copies of $\termvec=\effof{\terms}\cdot \prodvec$ is bounded by $\ceilof{1+\log \aconst}$.
It remains to turn every copy of $\termvec$ in $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$ into a run using $\aprodseqdiffterms$. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

The run $\offsetrunleft$ may also have a negative effect on the unbounded counters.
What makes the situation different is that $\offsetrunleft.\offsetrunright$ use their own copies of the homogeneous solution while $\diffrunleft.\diffrunright$ share their copies with $\upseq.\downseq$. 
This means we can repeat $\upseq$ a number of times $\abound$ extra, and we select $\abound\geq \hurdleof{\offsetrunleft}$.

The runs $\iterrun{\aconst}$ we are after result from the following derivation: 
\begin{align*}
\startnonterm \xrightarrow{\aprodseqpump^{\aconst\cdot \abound}}&\ \upseq^{\aconst\cdot \abound}.\startnonterm.\downseq^{\aconst\cdot \abound}\\
\xrightarrow{\text{wide tree}}&\ \upseq^{\aconst\cdot \abound}.\asentform_{\aconst\cdot \abound, 1}.\startnonterm.\asentform_{\aconst\cdot \abound, 2}.\downseq^{\aconst\cdot \abound}\\
\xrightarrow{\aprodseqdiffterms^{\aconst}}&\ \upseq^{\aconst\cdot \abound}.\arun_{\aconst\cdot \abound, 1}.\startnonterm.\arun_{\aconst\cdot \abound, 2}.\downseq^{\aconst\cdot \abound}\\
\xrightarrow{\aprodseqoffset}&\ \upseq^{\aconst\cdot \abound}.\arun_{\aconst\cdot \abound, 1}.\offsetrunleft^{\aconst-1}.\startnonterm.\offsetrunright^{\aconst-1}.\arun_{\aconst\cdot \abound, 2}.\downseq^{\aconst\cdot \abound}\\
\xrightarrow{\aprodseqreach}&\ \upseq^{\aconst\cdot \abound}.\arun_{\aconst\cdot \abound, 1}.\offsetrunleft^{\aconst-1}.\reachrun.\offsetrunright^{\aconst-1}.\arun_{\aconst\cdot \abound, 2}.\downseq^{\aconst\cdot \abound}\ .
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

It remains to determine a constant~$\aconst_0$ from which the runs $\iterrun{\aconst}$ stay non-negative. 
We estimate the hurdle we have to meet with the up-pumping sequence. 
We first consider the incomplete copies of~$\termvec$. 
We iterate over all sentential forms~$\asentform$ that could result from them and over all runs $\arun$ that could be derived from $\asentform$ using $\aprodseqdiffterms$, and determine the maximal hurdle $\maxhurdlediff$ as 
\begin{align*}
\max\setcond{\hurdleof{\arun}}{\paramparikhof{\terms}{\asentform}<\termvec\text{ and } \asentform\xrightarrow{\aprodseqdiffterms}\arun}\ .
\end{align*}
We slightly abuse the notation here. 
Actually, we do not use the full $\aprodseqdiffterms$ but only the productions for the childNGVAS~$\anngvasp$ that occur in~$\asentform$. 
For one instance of $\anngvasp$, there is a choice of whether to derive $\baserundef$ or $\arun'^{(\enableconst)}_{\anngvasp}$. 
The above notation is meant to cover all cases. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

Recall that $\upseq.\diffrunleft.\diffrunright$ has a strictly positive effect on the unbounded counters. 
This means a complete copy of $\termvec$ does not add to the hurdle.
So the maximal hurdle we have to expect due to incomplete copies of $\termvec$ is $\maxhurdlediff\cdot \ceilof{1+\log \aconst}$. 
To enable the above run, we still have to add $\hurdleof{\reachrun}$.
With this analysis, the run  $\iterrun{\aconst}$ will stay non-negative as long as $\aconst\geq \aconst_0$, with $\aconst_0$ the least natural number satisfying
\begin{align*}
\aconst_0\quad \geq\quad \maxhurdlediff\cdot \ceilof{1+\log \aconst_0}\ +\ \hurdleof{\reachrun}\ . \\
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that each run $\iterrun{\aconst}$ with $\aconst\geq \aconst_0$ has the properties formulated in the iteration lemma: 
it solves reachability and uses a number of updates that is as desired.
Thanks to the marking equations, we can study these properties on a $\paramparikh{\updates}$-equivalent run. 
We use
\begin{align*}
\upseq^{\aconst\cdot \abound}.\diffrunleft^{\aconst\cdot \abound}.\offsetrunleft^{k-1}.\reachrun.\offsetrunright^{k-1}.\diffrunright^{\aconst\cdot \abound}.\downseq^{\aconst\cdot \abound}\ .
\end{align*}
To see Parikh equivalence with $\iterrun{\aconst}$, note that the tree $\atreedef$ has the same productions as $\aprodseqdiffanngvas^k$. 
By Lemma~\ref{Lemma:EEKConverse}, we have $\paramparikhof{\terms}{\asentformdiffleft^\aconst.\asentformdiffright^\aconst}=\paramparikhof{\terms}{\asentform_{\aconst, 1}.\asentform_{\aconst, 2}}$. 
We then apply the same derivations to the childNGVAS in these sentential forms.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that we solve reachability. 
Since $\asol'$ is a solution to the characteristic equations and $\sumconst\cdot \ahomsol$ as well as $\maxconst\cdot \ahomsol$ are solutions to the homogeneous variant of the characteristic equations,  also $\asol''=\asol'+\aconst\cdot \sumconst\cdot \ahomsol+(\aconst-1)\cdot \maxconst\cdot \ahomsol$ solves the charateristic equations.
Due to $\meof{\anngvas}{\invar, \updvar, \outvar}$, this in particular means $\asol''[\invar]+\effof{\updates}\cdot \asol''[\updvar]=\asol''[\outvar]$. 
By \eqref{Equation:UpdatesReach}, we have  $\paramparikhof{\updates}{\reachrun}=\asol'[\updvar]$. 
By \eqref{Equation:UpdatesPumpDiff}, the equality  $\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}=\sumconst\cdot \ahomsol[\updvar]$ holds.
Finally, by \eqref{Equation:UpdatesOffset}, we have $\paramparikhof{\updates}{\offsetrunleft.\offsetrunright}=\maxconst\cdot \ahomsol[\updvar]$.
Hence, 
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\offsetrunleft^{\aconst-1}.\reachrun.\offsetrunright^{\aconst-1}.\diffrunright^\aconst.\downseq^{\aconst}}=\asol''[\updvar]\ .
\end{align*} 
This means the Parikh vector satisfies the marking equation.
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

We have to show that the number of updates in the run has the form $\baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$, for some $\scaleconst$. 
We just argued that the number of updates is $\asol''[\updvar]$, so we can calculate as follows:
\begin{align*}
&\ \asol''[\updvar]\\
=&\ \argument{Definition $\asol''$}\\
&\ \asol'[\updvar]+\aconst\cdot \abound\cdot \sumconst\cdot \ahomsol[\updvar]+(\aconst-1)\cdot \maxconst\cdot \ahomsol[\updvar]\\
=&\ \argument{Definition $\asol'$}\\
&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot \abound\cdot \sumconst\cdot \ahomsol[\updvar]\\
&\quad +(\aconst-1)\cdot \maxconst\cdot \ahomsol[\updvar]\\
=&\ \argument{$\asol[\updvar]=\baseeffectchoice$}\\
&\ \baseeffectchoice+\aconst \cdot (\maxconst+\abound\cdot \sumconst)\cdot\ahomsol[\updvar]\\
=&\ \argument{$\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$}\\
&\ \baseeffectchoice+\aconst \cdot (\maxconst+\abound\cdot \sumconst)\cdot\periodeffect\cdot \periodeffectchoice\ .
\end{align*}



==> iterationlemma_wttwice.tex <==
\section{Iteration Lemma}\label{Section:IterationLemma}
\begin{theorem}
Let $\anngvas$ be perfect with $\restrictions = \baseeffect+\periodeffect^*$. 
Let $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Then there are $\initconst, \scaleconst\geq 1$ so that for every $\aconst\geq \initconst$ there is a run $\iterrun{\aconst}\in\runsof{\anngvas}$ with $\acontextin\fires{\iterrun{\aconst}}\acontextout$ and $\paramparikhof{\updates}{\iterrun{\aconst}} =  \baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
We proceed by Noetherian induction on the nesting depth and consider the non-linear case first.
Consider $\baseeffectchoice\in\restrictions$ and $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Perfectness \perfectnesssol gives us a solution $\asol$ to $\chareq{\anngvas}$ with $\asol[\updvar]=\baseeffectchoice$ and a full homogeneous solution $\ahomsol$ to $\homchareq{\anngvas}$ with $\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsection{Non-Linear Case}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Reaching Derivation}
We define $\asol' = \asol+ \maxconst\cdot \ahomsol$ as a new solution to $\chareq{\anngvas}$ ($\ahomsol$ is homogeneous) that is large enough to embed non-negative runs for all instances of all childNGVAS. 
The situation is the following. 
The derivation induced by $\asol'$ will introduce several instances of the terminal symbols $\anngvasp\in\terms$. 
Each instance $\anngvasp$ is a childNGVAS that now has to provide its own derivation. 
There are two requirements on the derivations of $\anngvasp$ we are looking for.
\begin{itemize}
\item[(1)] The run given by the derivation has to be fireable.  
\item[(2)] The derivations of all $\anngvasp$ instances together have to give the number of updates $\at{\asol'}{\updvardef}$, in order to guarantee the reachability property we are after.   
\end{itemize}
To achieve (1), our plan is to use the perfectness property~\perfectnessbase for all instances of $\anngvasp$ except one. 
Property~\perfectnessbase gives us a derivable run that is guaranteed to be enabled in the input marking and correspond to the base vector $\baseeffectdef$ of the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$. 
This, however, does not yet guarantee~(2). 
The solution $\asol'$ may also ask for repetitions of the period vectors in~$\periodeffectdef$. 
For the one instance of $\anngvasp$ that we left out, we obtain the non-negative run by invoking the induction hypothesis with appropriate $\baseeffectchoicedef$ and~$\periodeffectchoicedef$. 
The universal quantification over these vectors in the theorem thus makes it possible to hand over outer constraints on the repetition count of the period vectors to the childNGVAS. 
We turn to the details.
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

We first define $\maxconst$.
Let $\anngvasp\in\terms$ with $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$.  
To invoke the induction hypothesis, we let $\baseeffectchoicedef$ include the base vector of the restriction $\baseeffectdef$ and repetitions of the period vectors as required by $\asol$. 
For $\periodeffectchoicedef$, we follow the full homogeneous solution:
\begin{align*}
\baseeffectchoicedef\ &=\ \baseeffectdef + \periodeffectdef\cdot \asol[\periodeffectvardef]\\
\periodeffectchoicedef\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
As $\anngvasp$ is perfect by (P6) and $\periodeffectchoicedef\geq 1$ by (P3), we can invoke the induction hypothesis. 
It yields $\initconstdef$ and $\scaleconstdef$ so that for every $\aconst\geq \initconstdef$ we have a run $\iterrundefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrundefof{\aconst}}=\baseeffectchoice_{\anngvasp} +  \periodeffectdef \cdot \aconst\cdot \scaleconstdef\cdot \periodeffectchoicedef$.
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

Recall that $\asol'=\asol+\maxconst\cdot \ahomsol$. 
This means the choice of $\maxconst$ has to be independent of the childNGVAS: for every~$\anngvasp$ there has to be $\maxconstdef\geq \initconstdef$ so that $\maxconst=\maxconstdef\cdot \scaleconstdef$ holds. 
An appropriate choice for $\maxconst$ is 
\begin{align*}
\max\setcond{\initconstdef, \initconstppdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstdef\cdot \scaleconstppdef\ .
\end{align*}
The definition makes sure $\maxconst$ is divisible by every $\scaleconstdef$, and after the division we are left with $\maxconstdef\geq \initconstdef$. 
That we also need the $\initconstppdef$ and the $\scaleconstppdef$ will become clear when we discuss the offset derivation further below. 
Note that since the $\initconstdef$ and the $\scaleconstdef$ are positive by the induction hypothesis, $\asol'$ will contain at least one copy of $\ahomsol$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We show that $\asol'$ induces a derivation and discuss its properties.
Since~$\asol'$ solves Esparza-Euler-Kirchhoff, since it contains a copy of $\ahomsol$, and since $\ahomsol[\prodvar]\geq 1$ by~\perfectnessprods in perfectness, we can invoke Theorem~\ref{Theorem:EEK} to obtain a derivation $\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach$. 
By Lemma~\ref{Lemma:EEKConverse}, $\asentformreach$ is a sequence of terminal symbols in $\anngvas$. 
Thanks to $\ptof{\anngvas}{\avar_{\prods}, \avar_{\terms}}$, we even have $\paramparikhof{\terms}{\asentformreach}=\asol'[\avar_{\terms}]$.  
Each terminal in $\asentformreach$ is an update $\anupd\in\Z^{\adim}$ or a childNGVAS $\anngvasp$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We still have to derive runs for the childNGVAS~in~$\asentformreach$. 
Together, we then have 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqreachanngvas}\asentformreach
\text{ and }\reachrun\in\runsof{\asentformreach}.
\end{align*}
Recall that $\runsof{\asentformreach}$ concatenates runs of the terminals in $\asentformreach$, so $\reachrun=\arun_1\ldots\arun_{\cardof{\asentformreach}}$.  
If $\at{\asentform}{\mathit{i}}$ is an update $\anupd$, then $\arun_i=\anupd$. 
If $\at{\asentform}{\mathit{i}}$ is the first instance of a childNGVAS $\anngvasp$, then $\arun_i=\arun_{\anngvasp}^{(\maxconstdef)}$ as defined above.  
If $\at{\asentform}{\mathit{i}}$ is another occurrence of $\anngvasp$, then we use \perfectnessbase and get $\arun_i=\baserundef$ with effect $\baseeffectdef$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

Thanks to the marking equation $\meof{\anngvas}{\invar, \updvar, \outvar}$, the number of updates given by $\at{\asol'}{\avar_{\updates}}$ transforms 
$\at{\asol'}{\invar}\sqsubseteq \acontextin$ into $\at{\asol'}{\outvar}\sqsubseteq\acontextout$. 
In the appendix, we show that $\reachrun$ has precisely this number of updates:
\begin{align}
\paramparikhof{\updates}{\reachrun}\ = \ \at{\asol'}{\avar_{\updates}}\ .\tag{UPDATES-REACH}\label{Equation:UpdatesReach} 
\end{align}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The run $\reachrun$ is not guaranteed to stay non-negative. 
Neither do the updates in $\asentformreach$ guarantee non-negativity, nor do the runs of the childNGVAS guarantee non-negativity on the counters from $\adimset$. 
We now address this problem. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Pumping Derivation and Embedding}
To enable $\reachrun$, the idea is to surround it by a number of up-pumping and down-pumping runs.  
So we wish to repeatedly apply the pumping derivation $\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq$ that exists by~\perfectnesspumpingnospace.  
Unfortunately, we cannot even insert one copy of $\aprodseqpump$ without running the risk of jeopardizing reachability. 
The way out is to embed the pumping derivation into a homogeneous solution. 
Embedding the pumping derivation into a homogeneous solution means we provide another derivation 
$\startnonterm\xrightarrow{\aprodseqdiff}\diffrunleft.\startnonterm.\diffrunright$ that should be understood as the difference between the homogeneous solution and the pumping derivation. 
Formally, the two derivations together,  
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump}\upseq.\startnonterm.\downseq\xrightarrow{\aprodseqdiff}\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq \ ,
\end{align*}
have the effect prescribed by the homogeneous solution. 
In this section, we make the notion of embedding precise. 
%We make the embedding precise, the construction of an appropriate homogeneous solution and the definition of $\aprodseqdiff$. 
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------

We first inspect the pumping runs. 
There is a derivation $\startnonterm \xrightarrow{\aprodseqpumpanngvas} \asentformpumpleft.\startnonterm.\asentformpumpright$ so that $\upseq.\downseq$ belongs to $\runsof{\asentformpumpleft.\asentformpumpright}$. 
By the definition of $\runsof{\asentform}$, we know that the run derived for $\at{(\asentform_1.\asentform_2)}{\anindex}=\anngvasp$ satisfies $\restrictionsdef$. 
Moreover, by Lemma~\ref{Lemma:EEKConverse}, $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

The homogeneous solution $\ahomsol$ we are given may not be large enough to embed $\aprodseqpump$.  
We scale it to $\sumconst\cdot\ahomsol$ with $\sumconst=\embedconst+\enableconst$. 
The constant $\embedconst$ should be understood as the least natural number large enough so that $\embedconst\cdot \ahomsol$ embeds $\aprodseqpump$. 
Embedding $\aprodseqpump$ is made formal with two requirements we give next. 
These requirements are monotonic: if they hold for $\embedconst\cdot \ahomsol$, then they will hold for $\sumconst\cdot \ahomsol$. 
The first requirement is that we want to be able to subtract $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ from $\at{(\embedconst\cdot \ahomsol)}{\prodvar}$.
Even more, in the difference we want to retain a copy of each production to be able to invoke Esparza-Euler-Kirchhoff.  
This means $\embedconst$ has to be large enough so that 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\prodvar} - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1\ .\tag{R1}\label{Equation:EmbeddingProductions}
\end{align} 
This can be achieved as the productions belong to the support, due to \perfectnessprodsnospace.
An important consequence is 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\termvar} - \paramparikhof{\terms}{\asentformpumpleft.\asentformpumpright}\geq 0\ . \tag{$*$}\label{Equation:EmbeddingConsequence}
\end{align} 
The next requirement is that $\embedconst\cdot \ahomsol$ has to cover the updates in $\upseq.\downseq$. 
For the updates that are already present in $\asentformpumpleft.\asentformpumpright$, we have the inequality $\at{(\embedconst\cdot \ahomsol)}{\updvar} - \paramparikhof{\updates}{\asentformpumpleft.\asentformpumpright} \geq 0$. 
This is due to~\eqref{Equation:EmbeddingConsequence} combined with $\computeupdatesof{\anngvas}{\termvar, \updvar}$. 
We also have to cover the updates produced by the instances of the childNGVAS in $\asentformpumpleft.\asentformpumpright$.  
Consider the childNGVAS~$\anngvasp$ with $\restrictionsdef=\baseeffectdef+\periodeffectdef^*$.  
By~\eqref{Equation:EmbeddingConsequence} and $\computeupdatesof{\anngvas}{\termvar, \updvar}$, we are sure $\at{(\embedconst\cdot \ahomsol)}{\updvardef}$ contains precisely one copy of the base vector $\baseeffectdef$ for every instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
However, $\aprodseqpump$ may also produce copies of the period vectors. 
Let $\periodeffectpumpdef\in\N^{\periodeffectdef}$ count the period vectors in all runs that belong to an instance of~$\anngvasp$ in $\asentformpumpleft.\asentformpumpright$. 
For every childNGVAS $\anngvasp\in\terms$, we want 
\begin{align}
\at{(\embedconst\cdot \ahomsol)}{\periodeffectvardef} - \periodeffectpumpdef\geq 0\ .\tag{R2} \label{Equation:EmbeddingEffect}
\end{align} 
This can be achieved as the period vectors of all childNGVAS belong to the support, \perfectnesschildperiodsnospace. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsubsection{Difference Derivation}
We now define the production sequence $\aprodseqdiff$. 
We proceed in two steps and first define the productions in $\anngvas$ followed by the productions in the childNGVAS and their descendants, $\aprodseqdiff = \aprodseqdiffanngvas.\aprodseqdiffterms$. 
As we move along, we define the constant $\enableconst$ that has been missing. 
Recall that the goal is to turn the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ into a non-negative run. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
The production sequence $\aprodseqdiffanngvas$ should derive a terminal word in $\anngvas$. 
We plan to obtain it with an invokation of Esparza-Euler-Kirchhoff. 
To see that the result applies, note that $(\sumconst\cdot \ahomsol)[\prodvar]$ solves $\homeekof{\anngvas}{\prodvar}$, because $\ahomsol[\prodvar]$ does. 
Moreover, we argued above that also $\paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
Together, we get that the difference $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
By Requirement~\eqref{Equation:EmbeddingProductions} on $\embedconst$, we have $(\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}\geq 1$. 
Theorem~\ref{Theorem:EEK} thus yields $\startnonterm\xrightarrow{\aprodseqdiffanngvas} \asentformdiffleft.\startnonterm.\asentformdiffright$ with $\paramparikhof{\prods}{\aprodseqdiffanngvas} = (\sumconst\cdot \ahomsol)[\prodvar] - \paramparikhof{\prods}{\aprodseqpumpanngvas}$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We now construct the production sequence $\aprodseqdiffterms$ that turns the instances of the childNGVAS in $\asentformdiffleft.\asentformdiffright$ into non-negative runs: 
\begin{align*}
\startnonterm\xrightarrow{\aprodseqdiffanngvas}\asentformdiffleft.\startnonterm.\asentformdiffright\xrightarrow{\aprodseqdiffterms}\diffrunleft.\startnonterm.\diffrunright\ . 
\end{align*}
We proceed as in the construction of the reaching run in the previous section.
For the first instance of the childNGVAS~$\anngvasp$ in~$\asentformdiffleft.\asentformdiffright$, we use the derivation of a run $\iterrunpdefenable$ that is given by the induction hypothesis. 
The task of this run is to compensate the $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef\geq 0$ excess in period vectors from the pumping derivation, and the definition will be given in a moment. 
For the remaining occurrences of $\anngvasp$, we use the derivation of the run $\baserundef$ that we have by (P4).\\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To construct $\iterrunpdefenable$ that compensates the excess in period vectors, we invoke the induction hypothesis with the following vectors: 
\begin{align*}
\baseeffectchoicedef'\ &=\ \baseeffectdef + \periodeffectdef\cdot [ (\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef]\\
\periodeffectchoicedef'\ &=\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
The definition uses Requirement~\eqref{Equation:EmbeddingEffect} on $\embedconst$, the choice of period vectors $(\embedconst\cdot \ahomsol)[\periodeffectvardef] - \periodeffectpumpdef$ has to be non-negative. 
As $\anngvasp$ is perfect by~(P6) and as $\periodeffectchoicedef'\geq 1$ by (P3), the induction hypothesis applies and yields $\initconstpdef$ and $\scaleconstpdef$ so that for every $\aconst\geq \initconstpdef$ we have a run $\iterrunpdefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunpdefof{\aconst}}=\baseeffectchoice_{\anngvasp}' +  \periodeffectdef\cdot \aconst \cdot \scaleconstpdef\cdot \periodeffectchoicedef'$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
We define $\enableconst$ in analogy to $\maxconst$ from above as 
\begin{align*}
\enableconst\ =\ \max\setcond{\initconstpdef}{\anngvasp\in\terms}\cdot \prod_{\anngvasp\in\terms}\scaleconstpdef\ .
\end{align*}
The $\enableconstdef$ we have been looking for is $\enableconst$ divided by $\scaleconstpdef$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
To sum up, we now have $\startnonterm\rightarrow^*\upseq.\diffrunleft.\startnonterm.\diffrunright.\downseq$ using the production sequence $\aprodseqpump.\aprodseqdiff$ with $\aprodseqpump = \aprodseqpumpanngvas.\aprodseqpumpterms$ and $\aprodseqdiff=\aprodseqdiffanngvas.\aprodseqdiffterms$. 
We check that the number of updates in the terminal sequence is the one expected by $\sumconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}\ =\
(\sumconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-PUMP-DIFF}\label{Equation:UpdatesPumpDiff}
\end{align} 

% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Offset Derivation}
If we surround the reaching derivation with $\aconst$ many repetitions of the pumping derivation and the difference derivation, we obtain $\maxconst +\aconst\cdot \sumconst$ many repetitions of the homogeneous solution. 
This does not yield the $\aconst\cdot \scaleconst$ number of repetitions of  $\periodeffectchoice$ that we promised in the induction hypothesis, because the $\maxconst$ factor acts as an offset. 
We have to insert another $\aconst-1$ copies of $\maxconst\cdot \ahomsol$ to arrive at $\aconst\cdot (\sumconst+\maxconst)$ many repetitions of the homogeneous solution. 
We now show how to construct what we call an offset derivation, a derivation that corresponds to $\maxconst\cdot \ahomsol$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the offset derivation, we define the production sequence $\aprodseqoffset=\aprodseqoffsetanngvas.\aprodseqoffsetterms$. 
We obtain $\aprodseqoffsetanngvas$  from $(\maxconst\cdot\ahomsol)[\prodvar]$ using Esparza-Euler-Kirchhoff. 
The corresponding derivation $\startnonterm\xrightarrow{\aprodseqoffsetanngvas}\asentformoffsetleft.\startnonterm.\asentformoffsetright$ satisfies $(\maxconst\cdot\ahomsol)[\termvar]=\paramparikhof{\terms}{\asentformoffsetleft.\asentformoffsetright}$. 
The sequence $\aprodseqoffsetterms$ is a concatenation of sequences  $\aprodseqoffsettermsindex$, one for every terminal in $\asentformoffsetleft.\asentformoffsetright$. 
For updates, these sequences are empty. 
For instances of childNGVAS $\anngvasp$ that are not the first ones, we use (P4) in perfectness. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the first instance of $\anngvasp$, we invoke the induction hypothesis with 
\begin{align*}
\baseeffectchoicedef''\ =\ \baseeffectdef \qquad\text{and}\qquad 
\periodeffectchoicedef''\ =\ \ahomsol[\periodeffectvardef]\ .
\end{align*}
It yields $\initconstppdef$ and $\scaleconstppdef$ so that for all $\aconst\geq \initconstppdef$ there is a run $\iterrunppdefof{\aconst}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\iterrunppdefof{\aconst}}=\baseeffectchoice_{\anngvasp}'' +  \periodeffectdef\cdot \aconst \cdot \scaleconstppdef\cdot \periodeffectchoicedef''$. 
We now define $\offsetconstdef$ as $\maxconst$ divided by $\scaleconstppdef$. 
This yields an integer, because $\maxconst$ is defined as a product with $\scaleconstppdef$. 
Moreover, we have $\offsetconstdef\geq \initconstppdef$ as we included the $\initconstppdef$ in the definition of $\maxconst$. 
For the first instance of~$\anngvasp$, we then use the derivation of the run $\iterrunppdefoffset$.
\\\\
Together, we now have
\begin{align*}
\startnonterm\xrightarrow{\aprodseqoffsetanngvas}\asentformoffsetleft.\startnonterm.\asentformoffsetright\xrightarrow{\aprodseqoffsetterms}\offsetrunleft.\startnonterm.\offsetrunright\ .\\
\end{align*}
It remains to check that the number of updates in $\offsetrunleft.\offsetrunright$ is as expected by $\maxconst\cdot \ahomsol$: 
\begin{align}
\paramparikhof{\updates}{\offsetrunleft.\offsetrunright}\ =\
(\maxconst\cdot \ahomsol)[\updvar]\ .\tag{UPDATES-OFFSET}\label{Equation:UpdatesOffset}
\end{align}
The reasoning is very similar to the reasoning for the reaching derivation and the reasoning for the combination of pumping and difference derivation. 
The critical point is to show that the repetitions of the period vectors are as expected. 
The vector $\baseeffectchoicedef''$ does not contain copies of the period vectors.
Hence, we only get copies prescribed by $\offsetconstdef\cdot \scaleconstppdef\cdot \periodeffectchoicedef''$. 
As $\offsetconstdef\cdot \scaleconstppdef=\maxconst$ and $\periodeffectchoicedef''\ =\ \ahomsol[\periodeffectvardef]$, we are done. 
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsubsection{Pumping}
We now make the reaching run fireable by surrounding the reaching derivation by repetitions of the pumping derivation, the difference derivation, and the offset derivation.  
Here is what we know.
\rfm{This is overly simplified and written with a counter in mind that is concrete in the input and output marking, but contained in the set of unbounded counters. While this qualification is needed, the text may transport the idea well.}
The runs $\upseq$ and $\downseq$ generated by the pumping derivation have a strictly positive resp.~a strictly negative effect on the unbounded counters.
Together, the runs $\upseq.\downseq$ and $\diffrunleft.\diffrunright$ from the pumping derivation and from the difference derivation have effect zero on the unbounded counters.
This means $\upseq.\diffrunleft.\diffrunright$ will have a strictly positive effect on the unbounded counters.
Also $\offsetrunleft.\offsetrunright$ has a zero effect on the unbounded counters. 
Repeating the pumping, the difference, and the offset derivation in a naive way then yields
\begin{align*}
\startnonterm\xrightarrow{\aprodseqpump^k}&\ \upseq^k.\startnonterm.\downseq^k\\
\xrightarrow{\aprodseqdiff^k}&\ \upseq^k.\diffrunleft^k.\startnonterm.\diffrunright^k.\downseq^k \\
\xrightarrow{\aprodseqoffset^{k-1}}&\ \upseq^k.\diffrunleft^k.\offsetrunleft^{k-1}.\startnonterm.\offsetrunright^{k-1}.\diffrunright^k.\downseq^k \\
\xrightarrow{\aprodseqreach}&\ \upseq^k.\diffrunleft^k.\offsetrunleft^{k-1}.\reachrun.\offsetrunright^{k-1}.\diffrunright^k.\downseq^k\ .
\end{align*}
The problem is that $\diffrunleft$ and $\diffrunright$ are not placed next to each other, but we first generate the copies of $\diffrunleft$ and later the copies of $\diffrunright$. 
Unfortunately, there is no guarantee that $\upseq.\diffrunleft$ has a positive effect on the unbounded counters. 
For $\offsetrunleft$ and $\offsetrunright$, we have the same problem. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
The way out is to use the wide tree theorem on the difference derivation and on the offset derivation. 
Then the hurdle required by the copies of the difference run and the offset run will only grow logarithmically in the number of tokens produced by the pumping run.
This will eventually make the run fireable. 
We turn to the details.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We first argue that the wide tree theorem applies. 
By definition, the NGVAS~$\anngvas$ is non-linear, strongly connected, and only has useful non-terminals. 
We already observed that $\prodvec = \paramparikhof{\prods}{\aprodseqdiffanngvas}$ solves $\homeekof{\anngvas}{\prodvar}$. 
We can thus arrange $\aconst$ copies of $\prodvec$ in a parse tree $\atreedef$ of height $\ceilof{1+\log \aconst}\cdot \normof{\prodvec}$, for every $\aconst\geq 1$. 
Let the yield by $\yieldof{\atreedef}=\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}$. 
The theorem moreover guarantees that for every prefix $\asentform$ of $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$, the number of incomplete copies of $\termvec=\effof{\terms}\cdot \prodvec$ is bounded by $\ceilof{1+\log \aconst}$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We now consider the offset derivation.
We have $\paramparikhof{\prods}{\aprodseqoffsetanngvas}=(\maxconst\cdot \ahomsol)[\prodvar]=\prodvec'$. 
As $\maxconst\cdot\ahomsol$ is a solution to homogeneous variant of the characteristic equations, $\prodvec'$ in particular solves $\homeekof{\anngvas}{\prodvar}$. 
We can thus arrange $\aconst-1$ copies of $\prodvec'$ in a parse tree $\atreepdefminus$ of height $\ceilof{1+\log (\aconst-1)}\cdot \normof{\prodvec'}$, for every $\aconst\geq 2$. 
Let the yield by $\yieldof{\atreepdefminus}=\asentformp_{\aconst, 1}.\startnonterm.\asentformp_{\aconst, 2}$. 
The theorem moreover guarantees that for every prefix $\asentformp$ of $\asentformp_{\aconst, 1}.\asentformp_{\aconst, 2}$, the number of incomplete copies of $\termvec'=\effof{\terms}\cdot \prodvec'$ is bounded by $\ceilof{1+\log (\aconst-1)}$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
For the derivation we are after, it remains to turn every copy of $\termvec$ in $\asentform_{\aconst, 1}.\asentform_{\aconst, 2}$ into a run using $\aprodseqdiffterms$, and every copy of $\termvec'$ in $\asentformp_{\aconst, 1}.\asentformp_{\aconst, 2}$ into a run using $\aprodseqoffsetterms$. 
We have
\begin{align*}
\startnonterm \xrightarrow{\aprodseqpump^{\aconst}}&\ \upseq^{\aconst}.\startnonterm.\downseq^{\aconst}\\
\xrightarrow{\text{wide tree theorem}}&\ \upseq^{\aconst}.\asentform_{\aconst, 1}.\startnonterm.\asentform_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqdiffterms^{\aconst}}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\startnonterm.\arun_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\text{wide tree theorem}}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\asentformp_{\aconst-1, 1}.\startnonterm.\asentformp_{\aconst-1, 2}.\arun_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqoffsetterms^{\aconst-1}}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\arun_{\aconst-1, 1}'.\startnonterm.\arun_{\aconst-1, 2}'.\arun_{\aconst, 2}.\downseq^{\aconst}\\
\xrightarrow{\aprodseqreach}&\ \upseq^{\aconst}.\arun_{\aconst, 1}.\arun_{\aconst-1, 1}'.\reachrun.\arun_{\aconst-1, 2}'.\arun_{\aconst, 2}.\downseq^{\aconst}\ =\ \iterrun{\aconst}\ .
\end{align*}
These are runs $\iterrun{\aconst}$ we are after.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
It remains to determine a constant~$\aconst_0$ from which the runs $\iterrun{\aconst}$ stay non-negative. 
We estimate the hurdle we have to meet with the up-pumping sequence. 
We first consider the incomplete copies of~$\termvec$. 
We iterate over all sentential forms~$\asentform$ that could result from them and over all runs $\arun$ that could be derived from $\asentform$ using $\aprodseqdiffterms$, and determine the maximal hurdle $\maxhurdlediff$ as 
\begin{align*}
\max\setcond{\hurdleof{\arun}}{\paramparikhof{\terms}{\asentform}<\termvec\text{ and } \asentform\xrightarrow{\aprodseqdiffterms}\arun}\ .
\end{align*}
We slightly abuse the notation here. 
Actually, we do not use the full $\aprodseqdiffterms$ but only the productions for the childNGVAS~$\anngvasp$ that occur in~$\asentform$. 
For one instance of $\anngvasp$, there is a choice of whether to derive $\baserundef$ or $\arun'^{(\enableconst)}_{\anngvasp}$. 
The above notation is meant to cover all cases. 
In analogy, we define $\maxhurdleoffset$ as
\begin{align*}
\max\setcond{\hurdleof{\arun}}{\paramparikhof{\terms}{\asentform}<\termvec\text{ and } \asentform\xrightarrow{\aprodseqoffsetterms}\arun}\ . 
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

Recall that $\upseq.\diffrunleft.\diffrunright$ has a strictly positive effect on the unbounded counters. 
This means a complete copy of $\termvec$ does not add to the hurdle.
So the maximal hurdle we have to expect due to incomplete copies of $\termvec$ is $\maxhurdlediff\cdot \ceilof{1+\log \aconst}$. 
Similarly, the maximal hurdle we have to expect due to incomplete copies of $\termvec'$ is $\maxhurdlediff\cdot \ceilof{1+\log(\aconst-1)}$. 
To enable the above run, we still have to add $\hurdleof{\reachrun}$.
We also add $1$ for $\aconst-1$ to stay non-negative. 
With this analysis, the run  $\iterrun{\aconst}$ will stay non-negative as long as $\aconst\geq \aconst_0$, with $\aconst_0$ the least natural number satisfying
\begin{align*}
\aconst_0\quad \geq\quad (\maxhurdlediff+\maxhurdleoffset)\cdot \ceilof{1+\log \aconst_0}\ +\ \hurdleof{\reachrun}\ +\ 1. \\
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that each run $\iterrun{\aconst}$ with $\aconst\geq \aconst_0$ has the properties formulated in the iteration lemma: 
it solves reachability and uses a number of updates that is as desired.
Thanks to the marking equations, we can study these properties on a Parikh equivalent run. 
We use
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\offsetrunleft^{k-1}.\reachrun.\offsetrunright^{k-1}.\diffrunright^\aconst.\downseq^{\aconst}}\ =\ \ \paramparikhof{\updates}{\iterrun{\aconst}}\ .
\end{align*}
To see the equality, note that the tree $\atreedef$ has the same productions as $\aprodseqdiffanngvas^k$.
By Lemma~\ref{Lemma:EEKConverse}, we have $\paramparikhof{\terms}{\asentformdiffleft^\aconst.\asentformdiffright^\aconst}=\paramparikhof{\terms}{\asentform_{\aconst, 1}.\asentform_{\aconst, 2}}$. 
We then apply the same derivations to the childNGVAS in these sentential forms.
A similar argument holds for $\atreepdefminus$. \\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We argue that we solve reachability. 
Since $\asol'$ is a solution to the characteristic equations and $\sumconst\cdot \ahomsol$ as well as $\maxconst\cdot \ahomsol$ are solutions to the homogeneous variant of the characteristic equations,  also $\asol''=\asol'+\aconst\cdot \sumconst\cdot \ahomsol+(\aconst-1)\cdot \maxconst\cdot \ahomsol$ solves the charateristic equations.
Due to $\meof{\anngvas}{\invar, \updvar, \outvar}$, this in particular means $\asol''[\invar]+\effof{\updates}\cdot \asol''[\updvar]=\asol''[\outvar]$. 
By \eqref{Equation:UpdatesReach}, we have  $\paramparikhof{\updates}{\reachrun}=\asol'[\updvar]$. 
By \eqref{Equation:UpdatesPumpDiff}, the equality  $\paramparikhof{\updates}{\upseq.\diffrunleft.\diffrunright.\downseq}=\sumconst\cdot \ahomsol[\updvar]$ holds.
Finally, by \eqref{Equation:UpdatesOffset}, we have $\paramparikhof{\updates}{\offsetrunleft.\offsetrunright}=\maxconst\cdot \ahomsol[\updvar]$.
Hence, 
\begin{align*}
\paramparikhof{\updates}{\upseq^{\aconst}.\diffrunleft^\aconst.\offsetrunleft^{\aconst-1}.\reachrun.\offsetrunright^{\aconst-1}.\diffrunright^\aconst.\downseq^{\aconst}}=\asol''[\updvar]\ .
\end{align*} 
This means the Parikh vector satisfies the marking equation.\\\\
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
We have to show that the number of updates in the run has the form $\baseeffectchoice + \periodeffect\cdot \aconst\cdot\scaleconst\cdot \periodeffectchoice$, for some $\scaleconst$. 
We just argued that the number of updates is $\asol''[\updvar]$, so we can calculate as follows:
\begin{align*}
&\ \asol''[\updvar]\\
=&\ \argument{Definition $\asol''$}\\
&\ \asol'[\updvar]+\aconst\cdot \sumconst\cdot \ahomsol[\updvar]+(\aconst-1)\cdot \maxconst\cdot \ahomsol[\updvar]\\
=&\ \argument{Definition $\asol'$}\\
&\ \asol[\updvar]+\maxconst\cdot\ahomsol[\updvar]+\aconst\cdot \sumconst\cdot \ahomsol[\updvar]+(\aconst-1)\cdot \maxconst\cdot \ahomsol[\updvar]\\
=&\ \argument{$\asol[\updvar]=\baseeffectchoice$}\\
&\ \baseeffectchoice+\aconst \cdot (\maxconst+\sumconst)\cdot\ahomsol[\updvar]\\
=&\ \argument{$\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$}\\
&\ \baseeffectchoice+\aconst \cdot (\maxconst+\sumconst)\cdot\periodeffect\cdot \periodeffectchoice\ .
\end{align*}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

\subsection{Linear Case}
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

%\rfm{Warum die Menge $R$: Iterieren unten und oben klappt sonst nicht unabhängig voneinander.}



==> iterationlemmabackup.tex <==
\section{Iteration Lemma}
\begin{theorem}
Let $\anngvas$ be perfect with restriction $\restrictions = \baseeffect+\periodeffect^*$. 
Let $\baseeffectchoice\in\restrictions$ and let $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$. 
Assume $\chareq{\anngvas}$ is feasible. 
Then there is $\aconst_0\in\N$ so that for every $\aconst\geq \aconst_0$ there is a run $\arun^{(\aconst)}\in\runsof{\agram}$ with $\acontextin\fires{\arun^{(\aconst)}}\acontextout$ and $\paramparikhof{\updates}{\arun^{(k)}} = \baseeffectchoice + \periodeffect\cdot \aconst\cdot \periodeffectchoice$. %\in \restrictions$ so that $\paramparikhof{\updates}{\arun^{k}}\geq \avec + k \sum\asetvec$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
We proceed by Noetherian induction and consider the non-linear case first.\\
Let $\asol$ be the solution that exists by the hypothesis.\\ 
Let $\ahomsol$ be a full homogeneous solution that exists by perfectness.\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\subsection{Non-Linear Case}
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\paragraph*{Base Run}
We first modify the solution $\asol$ so that it admits non-negative runs for the childNGVAS.\\
Consider the childNGVAS $\anngvasp\in\terms$.\\
By (P4) in perfectness, the base vector $\baseeffectdef$ of the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*$ can be fired.\\
As a consequence, the characteristic system $\chareq{\anngvasp}$ is feasible.\\ 
We are thus in a position to invoke the induction hypothesis for $\anngvasp$.\\
Let $\baseeffectchoice_{\anngvasp}=\baseeffectdef + \periodeffectdef\cdot \asol[\periodeffectvardef]$.\\
Note that $\ahomsol[\periodeffectvardef]\geq 1$ by (P3) in perfectness.\\
The induction hypothesis yields a repetition count $\aconst_{0, \anngvasp}$ so that for every $\aconst\geq \aconst_{0, \anngvasp}$ we have a run $\arun^{(\aconst)}_{\anngvasp}\in \runsof{\anngvasp}$ with updates $\paramparikhof{\updates}{\arun^{(\aconst)}_{\anngvasp}}=\baseeffectchoice_{\anngvasp} +  \periodeffectdef\cdot \aconst \cdot \ahomsol[\periodeffectvardef]$. \\
Let $\maxconst = \max_{\anngvasp\in\terms}\aconst_{0, \anngvasp}$ and assume $\maxconst\geq 1$. \\
Let  $\asol' = \asol+ \maxconst\cdot \ahomsol$.\\ 
Note that $\asol'$ still solves the characteristic equations.\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We have $\ahomsol[\prodvar]\geq 1$ by (P2) in perfectness.\\
Since $\asol'$ contains a copy of $\ahomsol$ and solves Esparza-Euler-Kirchhoff, we can invoke Theorem~\ref{Theorem:EEK} to find a derivation $\startnonterm\xrightarrow{\aprodseqreach}\asentform$ that yields a sequence of terminal symbols in $\anngvas$. \\
Each terminal in $\asentform$ is an update $\anupd\in\Z^{\adim}$ or a childNGVAS $\anngvasp$, and the instances of $\anngvasp$ together contribute $\asol'[\avar_{\anngvasp, \updates}]$ to the overall number of updates $\asol'[\updvar]$. \\
The marking equation guarantees that the overall number of updates transforms the input marking $\asol'[\invar]$ to the output marking $\asol'[\outvar]$.\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We complete the above derivation to a terminal derivation.\\
Consider the childNGVAS $\anngvasp$, for which we need the updates $\asol'[\avar_{\anngvasp, \updates}]$ given by $\asol'[\anngvasp]$-many derivations. \\
For all of these derivations except one, we rely on (P4).\\
It provides a non-negative run with updates  $\baseeffectdef$.\\
According to $\computeupdatesof{\anngvasp}{\termvar, \updvar}$, what is left is to find a single run with effect $\baseeffectdef+\periodeffect\cdot \asol'[\periodeffectvardef]$. \\
We already argued above that the induction hypothesis for $\anngvasp$ yields a run $\arun^{(\maxconst)}_{\anngvasp}\in \runsof{\anngvasp}$.\\
It remains to check the number of updates:
\begin{align*}
\paramparikhof{\updates}{\arun^{(\maxconst)}_{\anngvasp}} &= \baseeffectchoice_{\anngvasp}+\periodeffectdef\cdot \maxconst\cdot \ahomsol[\periodeffectvardef]\\
 &= \baseeffectdef+\periodeffectdef\cdot \asol[\periodeffectvardef]+ \periodeffectdef \cdot \maxconst\cdot \ahomsol[\periodeffectvardef]\\
&= \baseeffectdef + \periodeffectdef\cdot \asol'[\periodeffectvardef]\ .
\end{align*}

We now have 
\begin{alignat*}{5}
\startnonterm\rightarrow^*\asentform\rightarrow^* \arun_1\ldots \arun_{\cardof{\asentform}} = \arun, 
\end{alignat*}
where $\arun_i$ is $\arun_{\anngvasp}^{(\maxconst)}$ for one instance $\asentform_i$ of $\anngvasp$, $\arun_i$ is the run with effect $\baseeffectdef$ for all other instances $\asentform_i$ of $\anngvasp$, and $\arun_i$ is simply $\asentform_i$ if $\asentform_i$ is an update.\\
Moreover, $\arun$ is guaranteed to solve reachability.\rfm{refer to in- and out-marking.}\\ 
Unfortunately, $\arun$ is not guaranteed to stay non-negative.\\
We now address this problem.
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\paragraph*{Pumping}
The plan is to produce a number of up- and down-pumping sequences that is large enough to enable $\arun$. 
This means we wish to repeatedly apply the production sequence $\aprodseqpump$ that exists by perfectness (P5). 
We can assume $\aprodseqpump=\aprodseqanngvas.\aprodseqanngvascomplement$ so that $\aprodseqanngvas$ contains the productions that belong to $\anngvas$ and $\aprodseqanngvascomplement$ contains the production that belong to the subNGVAS. 
In particular, $\startnonterm \xrightarrow{\aprodseqanngvas} \alpha_1.\startnonterm.\alpha_2$ with $\alpha_1, \alpha_2\in\terms^*$. 
We can thus apply Lemma~\ref{Lemma:EEKConverse} and conclude that $\paramparikhof{\prods}{\aprodseqanngvas}$ solves $\homeekof{\anngvasp}{\prodvar}$. \\\\
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
Unfortunately, we cannot simply repeat $\aprodseqpump$ without jeopardizing reachability, the fact that the yield of $\aprodseqreach$ takes the input marking to the output marking.\\
The way out is to embed the repetition of $\aprodseqpump$ into a homogeneous solution.\\
Let $\ahomsol=k\cdot \ahomsol'$ contain $k\in\N$ copies of the homogeneous solution.\\
We choose $k$ so that $\adiffsol = (\ahomsol - \paramparikhof{\prods}{\aprodseqanngvas})[\prodvar]\geq 1$.\\
\rfm{W\"ahle $k$ gro\ss\ genug, dass man die Schranke aus der IV \"uberschreitet. Dann ist man hier schon enabled. Ben\"otigt, dass die Perioden der Kinder im Support liegen.}
The idea is that $\ahomsol$ allows us to add a repetition of $\aprodseqanngvas$, and we are still sure to solve reachability as long as we add a production sequence that corresponds to $\adiffsol$.
\rfm{Updates in the pumping sequences have to be part of the support.}\\\\

% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\rfm{Wide tree theorem.}The first thing to observe is that $\adiffsol$ is again a homogeneous solution.\\ 
The reason is that $\ahomsol'$ is a homogeneous solution and, as we just observed, also $\paramparikhof{\prods}{\aprodseqanngvas}$ is.\\
We can thus apply Esparza-Euler-Kirchhoff and obtain a production sequence $\aprodseqdiff$ with $\paramparikhof{\prods}{\aprodseqdiff}=\adiffsol[\prodvar]$.\\

% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
\subsection{Linear Case}




% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------
% ---------------------------------------------------------------------------

\rfm{Warum die Menge $R$: Iterieren unten und oben klappt sonst nicht unabhängig voneinander.}



==> ngvas_complex_context.tex <==
\section{Nested GVAS}
This is the data structure we rely on for our decision procedure. 
From now on, we fix the dimension to be $\adim$.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\subsection{Definition}
A \emph{nested GVAS} (NGVAS) is a triple $\anngvas=(\agram, \contextinformation, \boundednessinformation)$ with $\agram=(\nonterms, \terms, \prods, \startnonterm)$ a CFG in wCNF that is strongly connected and only has useful non-terminals. 
The choice of the set of terminal symbols depends on the \emph{nesting depth}, a natural number that is associated with the NGVAS. 
An NGVAS of nesting depth $0$ has as terminals counter updates in~$\Z^{\adim}$.
An NGVAS of nesting depth $i+1$ has as terminals \ek{non-empty sets of NGVAS} of nesting depth at most~$i$. 
We call an NGVAS that occurs \ek{in} a terminal symbol of $\anngvas$ a child.
We call an NGVAS that occurs \ek{in} a terminal symbol in one of the NGVAS defined within $\anngvas$ a subNGVAS, so every child is a subNGVAS but not the other way around. 
We expect that all subNGVAS have mutually disjoint sets of terminals and non-terminals. 
\rfm{Check whether we still do the following.}
We lift terminology and notation for the grammar $\agram$ to the NGVAS $\anngvas$. 
For example, we may say $\anngvas$ is linear when we mean $\agram$ is linear, or write $\anngvas.\startnonterm$ for the start non-terminal $\agram.\startnonterm$.  

Throughout the development, we will distinguish the case where the NGVAS is non-linear from the case where it is linear.
In the non-linear case, the wide tree theorem simplifies pumping. 
In the linear case, we have to assume more elaborate pumping information.  
If the NGVAS is linear, we assume the productions take the shape $\prods=\prodsleft\discup\prodscenter\discup\prodsright$. 
The center is a singleton $\prodscenter=\set{\anontermcenter\rightarrow \anngvaspcenterleft.\anngvaspcenterright}$. 
We also split the terminals $\terms = \termsleft\discup\termscenterleft\discup\termscenterright\discup\termsright$ so that $\termsleft$ and $\termsright$ are the terminals produced by $\prodsleft$ resp. $\prodsright$ to the left resp. to the right of a non-terminal. 
In the center, we have the expected $\termscenterleft=\set{\anngvaspcenterleft}$ and $\termscenterright=\set{\anngvaspcenterright}$.
We refer to $\set{\myleft, \mycenterleft, \mycenterright, \myright}$ as the set of directions, and use $\mydir$ to refer to an element in the set.  
We can already explain the need for the singleton production in the center.
If there were more productions that consumed a non-terminal, no production sequence could contain all of them. 
Theorem~\ref{Theorem:EEK} and Lemma~\ref{Lemma:EEKConverse} would not apply. 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------

The second component in an NGVAS is called the \emph{context information} and takes the form
 $\contextinformation=(\restrictions,  \acontext)$. 
 Let $\updates$ be the set of all counter updates that appear in $\anngvas$ or in a subNGVAS. 
The \emph{restriction} $\restrictions$ is a linear set of updates $\avec+\asetvec^*\subseteq\N^{\updates}$ that limits the effects of possible derivations and that serves as an interface between the NGVAS and its children. 
%
We will also understand the restriction as the equation  $\updvar-\asetvec\cdot \periodvar = \avec$ in $\updvar\in\N^{\updates}$ and $\periodvar\in\N^{\asetvec}$, and write it as~$\restrictions(\updvar, \periodvar)$. 
%
We also need a homogeneous variant of the restriction, denoted by $\homrestrictions(\updvar, \periodvar)$ and defined as $\updvar-\asetvec\cdot \periodvar = 0$, meaning we replace the base vector on the right-hand side by $0$. 
%
The second component $\acontext=(\acontextin, \acontextout)\in\Nomega^{2\adim}$ consists of so-called \emph{input} and \emph{output markings} $\acontextin$ and $\acontextout$.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------

The last component is called the \emph{boundedness information}.  
Its purpose is to track the values of counters which remain bounded in (an over-approximation of) the reaching runs. 
The definition is different for non-linear and for linear NGVAS. 
In the non-linear case, we have $\boundednessinformation = (\adimset, \infun, \outfun)$. 
We have a set of dimensions $\adimset\subseteq [1, \adim]$ and functions 
\begin{align*}
\infun, \outfun:\nonterms\discup\terms\rightarrow \omega^{\adimset}\times \N^{[1, \adim]\setminus \adimset}
\end{align*}
that assign to each non-terminal and terminal an input and an output marking.   
In these markings, the counters from $\adimset$ have value $\omega$, meaning $\adimset$ represents the unbounded counters and all non-terminals and terminals agree on them. 
The assignments should be consistent as follows. 
For the terminals that are updates~$\anupd$, we expect $\outof{\anupd}=\inof{\anupd}+\anupd$. 
\ek{For the childNGVAS $\anngvasp$ that stems from the terminal $\aterm\in\terms$}, the markings that we track have to be the input and the output from the context information, \ek{$\inof{\aterm}=\anngvasp.\acontextin$} and \ek{$\outof{\aterm}=\anngvasp.\acontextout$}. 
If we understand $\anngvasp.\acontextin$ and $\anngvasp.\acontextout$ as reachability information, then \ek{the corresponding $\inof{\aterm}$ and $\outof{\aterm}$} properly capture it. 
The reachability information in the terminals is lifted to the non-terminals. 
For every production $\anonterm\rightarrow\asentform_1.\asentform_2$, consistency requires
$\inof{\anonterm}=\inof{\asentform_1}$, $\outof{\asentform_1}=\inof{\asentform_2}$, and $\outof{\asentform_2}=\outof{\anonterm}$. 
Note that the second equality makes it possible to concatenate reaching runs in $\asentform_1$ and $\asentform_2$, as far as the bounded counters are concerned. 
For the start non-terminal, consistency requires $\acontextin\sqsubseteq \inof{\startnonterm}$ and $\acontextout\sqsubseteq \outof{\startnonterm}$, the 
input and output markings we track take the values from the context information, or they are more abstract and use~$\omega$. 
A consequence is $\omegaof{\acontextin}, \omegaof{\acontextout}\subseteq \adimset$. 
%The last consistency requirement is that the childNGVAS should start with $\adimset$ as the set of unbounded counters, for every $\anngvasp\in\terms$ we have $\omegaof{\anngvasp.\acontextin}=\adimset=\omegaof{\anngvasp.\acontextout}$. 

In the linear case, we have boundedness information for the left and the right side of the derivation, $\boundednessinformation = (\boundednessinformationleft, \boundednessinformationright)$.  
There is no boundedness information for the center as the production cannot be used repeatedly.  
For $\boundednessinformationleft = (\adimsetleft, \inleftfun, \outleftfun)$, we have a set of counters $\adimsetleft\subseteq [1, \adim]$ that should be assumed to be unbounded. 
We assign input markings to non-terminals and terminals on the left. 
Output markings are only assigned to terminals on the left: 
\begin{alignat*}{5}
\inleftfun:&\ \termsleft\discup\nonterms&&\ \rightarrow \omega^{\adimsetleft}\times \N^{[1, \adim]\setminus\adimsetleft}\\
\outleftfun:&\ \termsleft&&\ \rightarrow \omega^{\adimsetleft}\times \N^{[1, \adim]\setminus\adimsetleft}\ .
\end{alignat*} 
To formulate consistency, we need to assign an input to the non-terminal from the context production. 
We use $\inleftof{\anontermcontext}=\anngvaspcenterleft.\acontextin$. 
With this in place, the consistency requirement is as expected, and so is the definition for the right side. 
The last part of the consistency requirement is that 
\rfm{$\omegaof{\acontextin}\cap\omegaof{\acontextout}\subseteq\omegaof{\acontextinint}\cap \omegaof{\acontextoutint}$}

The NGVAS inherits the notion of a language from the underlying grammar, $\langof{\anngvas}=\langof{\agram}$. 
We also associate with the NGVAS a set of runs. 
The number of updates in these runs should satisfy the given restrictions, not only for $\anngvas$ but for all subNGVAS. 
The definition is by Noetherian induction \ek{(second line is new)}: 
\begin{align*}
&\runsof{\anngvas}\tinyspace =\tinyspace \setcond{\arun}{\exists \asentform\in\langof{\anngvas}.\tinyspace \arun\in\runsof{\asentform}\wedge \paramparikhof{\updates}{\arun}\in\restrictions}\tinyspace \\
&\runsof{\setcond{\anngvas_{i}}{i\in I}}\tinyspace =\tinyspace\bigcup_{i\in I}\runsof{\anngvas_{i}}.
\end{align*}
Here, $\runsof{\asentform}=\runsof{\seqat{\asentform}{1}}\ldots \runsof{\seqat{\asentform}{\cardof{\asentform}}}$, meaning we concatenate the sets of runs associated with the terminals in~$\asentform$. 
If a terminal is an update, we use $\runsof{\anupd}=\set{\anupd}$. 
If a terminal is a \ek{set of} childNGVAS, \ek{its language is the union of childNGVAS with} lower nesting depth and so the set of runs is defined by the induction hypothesis.
%If a terminal is a \ek{set of} childNGVAS, it has a lower nesting depth and so the set of runs is defined by the induction hypothesis.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\subsection{Characteristic Equations: Non-Linear Case}
Consider the non-linear NGVAS $\anngvas=(\agram, \restrictions, \acontext, \boundednessinformation)$. 
%
We approximate the set of runs that solve reachability with the \emph{characteristic system of equations} $\chareq{\anngvas}$ defined as
\begin{align*}
\eekof{\agram}{\prodvar} \wedge \evaleqof{\acontextin, \acontextout}{\prodvar, \updvar, \invar, \outvar} 
\wedge
\restrictions(\updvar, \periodvar)\tinyspace . 
\end{align*}
The equations $\evaleq{\acontextin, \acontextout}$ evaluate reachability as follows: 
\begin{align*}
\ptof{}{\prodvar, \termvar}\
&\wedge\ 
\computeupdatesof{\anngvas}{\termvar, \updvar}\
\wedge\ \meof{\updates}{\avar_{\myin}, \updvar, \avar_{\myout}}\\
&\wedge\ 
\invar \sqsubseteq \acontextin\ \wedge\
\outvar \sqsubseteq \acontextout\ .
\end{align*}
\rfm{Update text.} \ek{Need to add variables for or define EEK in a way that considers terminals as sets of childNGVAS.}
We have variables $\prodvar\in\N^{\prods}$ that determine how often each production should be taken. 
This choice has to satisfy Esparza-Euler-Kirchhoff. 
The productions lead to a number of terminal symbols given by~$\termvar\in\N^{\terms}$.  
We introduce variables $\updvar\in\N^{\updates}$ that store how often each update should be used, in $\anngvas$ and in the subNGVAS.  
The constraint $\computeupdatesof{\anngvas}{\termvar, \updvar}$ fills $\updvar$ with appropriate values, and we elaborate on it in a moment.
The choice of updates has to satisfy the restriction, and so $\periodvar$ states how often each period in that linear set will be used. 
We have variables $\invar$ and $\outvar$ that store the input and output markings for which the approximation of reachability holds.
They have to coincide with the given $\acontextin$ and $\acontextout$ whenever these are concrete, and can obtain arbitrary non-negative values where $\acontextin$ and $\acontextout$ hold $\omega$. 
We make sure the input and output variables are related by the marking equation.

The constraint $\computeupdatesof{\anngvas}{\termvar, \updvar}$ has to meet the following specification: the variables $\updvar$ store how often each counter update from $\updates$ is used in a run that can be derived from the number of terminal symbols $\termvar$.  
The challenge is to include the updates generated by subNGVAS.
To determine their number, we access the restrictions of the immediate childNGVAS. 
Consider $\anngvasp\in\terms$ with the restriction $\restrictions_{\anngvasp}=\baseeffectdef+\periodeffectdef^*\subseteq \N^{\updates}$. 
We introduce variables $\avar_{\anngvasp, \updates}$ that store the total number of updates used in a set of runs derivable from instances of~$\anngvasp$. 
The number of instances, and so the number of runs, is given by $\termvar[\anngvasp]$.
To make sure each run can be derived, we use the restriction.  
For every run, we have a copy of the base vector. 
Moreover, we have variables $\periodeffectvardef\in\N^{\periodeffectdef}$ determining how often each period vector should be taken. 
The variables $\updvar$ are then filled by addition, and we make sure not to forget the updates $\restrictto{\termvar}{\updates}$ done by $\anngvas$. 
We define $\computeupdatesof{\anngvas}{\termvar, \updvar}$ as
\begin{align*}
\bigwedge_{\anngvasp\in\terms} \ 
\updvardef - \baseeffectdef\cdot \termvar[\anngvasp] - \periodeffectdef\cdot \periodeffectvardef\ &=\ 0\\
 \updvar- \restrictto{\termvar}{\updates} - \sum_{\anngvasp\in\terms} \updvardef\ &=\ 0\ .
\end{align*}

We also need a \emph{homogeneous variant} $\homchareq{\anngvas}$
 of the characteristic equations,  
\begin{align*}
\homeekof{\agram}{\prodvar}\ \wedge \ 
\evaleqof{\zeroof{\acontextin}, \zeroof{\acontextout}}{\prodvar, \updvar,\tinyspace &\invar, \outvar} \\
 \wedge& \ \homrestrictions(\updvar, \periodvar)\ .
\end{align*}
We check reachability between the zero versions of the input and output markings, and we use the homogeneous variant of the restriction. 
The homogeneous characteristic equations are defined such that if $\asol$ solves $\chareq{\anngvas}$ and $\ahomsol$ solves $\homchareq{\anngvas}$, then also $\asol+\ahomsol$ solves $\chareq{\anngvas}$. 
To be explicit, we consider $\N$ solutions. 
Using well-quasi ordering arguments, one can then show that the variables which are unbounded in the solution space of $\chareq{\anngvas}$ are precisely the variables that receive a positive value in some homogeneous solution. 
% 
This leads to the definition of the \emph{support} of the characteristic equations, denoted by $\suppof{\homchareq{\anngvas}}$:
\begin{align*}
\setcond{\avar\in\varsof{\homchareq{\anngvas}}}{\exists \ahomsol.\ \ahomsol\text{ solves }\homchareq{\anngvas}\wedge \ahomsol(\avar)>0}\ .
\end{align*}
As the solution space of $\homchareq{\anngvas}$ is closed under addition, there always is a \emph{full homogeneous solution} that gives a positive value to all variables in the support. 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\subsection{Characteristic Equations: Linear Case}
Consider the linear NGVAS $\anngvas=(\agram, \restrictions, \acontext, \boundednessinformation)$. 
In this case, the context information takes the form 
\begin{align*}
\acontext = (\acontextinleft, \acontextoutleft=\acontextincenter, \acontextoutcenter=\acontextinright, \acontextoutright)\ .
\end{align*} 
\begin{align*}
(\acontextinleft, \acontextoutleft=\acontextincenterleft, \acontextoutcenterleft=\acontextincenterright, \acontextoutcenterright=\acontextinright, \acontextoutright)\ .
\end{align*}
In the linear case, we do not have the wide tree theorem available for pumping.
To overcome this problem, the first step is to let the characteristic equations require a stronger form of reachability. 
Recall that we split the sets of productions $\prods = \prodsleft\discup\prodscenter\discup\prodsright$ and terminals $\terms=\termsleft\discup\termscenter\discup\termsright$ so that the productions from $\prodsdir$ only produce terminals in~$\termsdir$ (at the expected side of the non-terminal). 
Moreover, recall that there is only one production that consumes a non-terminal, $\prodscenter=\set{\centerprod}$ is a singleton. 
If there were more center productions, there would be no production sequence that contains all of them. 
The terminals produced in each direction $\mydir$ should solve reachability from $\acontextindir$ to $\acontextoutdir$. 
We have only variables $\prodvarleft$ and $\prodvarright$ for the productions on the left and on the right. 
We do not have a variable for the center production.
Such a variable would be bounded in the solution space, and therefore complicate the perfectness condition. 
To ease the notation, we define the following vectors: 
\begin{alignat*}{5}
\prodvecleft &= (\prodvarleft, 0, 0^{\prodsright})\qquad&\qquad
\prodveccenter &= \centerprodvec\\
\prodvecright &= (0^{\prodsleft}, 0, \prodvarright) \qquad &\qquad \prodvec &= (\prodvarleft, 1, \prodvarright)\ .
\end{alignat*}
We define $\chareq{}$ as  
% --------------------------------------------------------------------------
% --------------------------------------------------------------------------
% --------------------------------------------------------------------------
% --------------------------------------------------------------------------
\begin{align*}
\eekof{}{\prodvec}\wedge \bigwedge_{\mydir}&
\evaleqof{\acontextindir, \acontextoutdir}{\prodvecdir, \updvardir, \invardir, \outvardir}
\end{align*}
\vspace{-0.5cm}
\begin{alignat*}{5}
\wedge\quad \outvarleft - \invarcenter &= 0\quad &\wedge \quad &\updvar - \sum_{\mydir} \updvardir = 0\\
\wedge\quad \outvarcenter - \invarright &= 0 \quad &\wedge \quad &\restrictions(\updvar, \periodvar)\ .
\end{alignat*}
Each instance of $\evaleq{}$ has its own copy $\termvardir$, $\periodeffectvardefdir$, and $\updvardefdir$ of the variables $\termvar$, $\periodeffectvardef$, and $\updvardef$, respectively. 
In $\computeupdatesof{\anngvas}{\termvardir, \updvardir}$, the conjunction only iterates over $\termsdir$, and so does the sum. 
With $\outvarleft - \invarcenter = 0$, the output marking we obtain for reachability on the left coincides with the input marking for the center, and so runs for the two directions can be connected.
We check the restriction on the sum of the updates obtained in the three directions.

We again have a homogeneous variant of the characteristic equations. 
We remove the occurrence of the center production, 
$\prodvecleftzero=\prodvecleft$, $\prodvecrightzero=\prodvecright$, $\prodveccenterzero=0$, $\prodveczero=(\prodvarleft, 0, \prodvarright)$.
The definition is then as expected:
\begin{align*}
\homeekof{}{\prodveczero}\wedge \bigwedge_{\mydir}&
\evaleqof{\zeroof{\acontextindir}, \zeroof{\acontextoutdir}}{\prodvecdirzero, \updvardir, \invardir, \outvardir}
\end{align*}
\vspace{-0.4cm}
\begin{alignat*}{5}
\wedge\quad \outvarleft - \invarcenter &= 0\quad &\wedge \quad &\updvar - \sum_{\mydir} \updvardir = 0\\
\wedge\quad \outvarcenter - \invarright &= 0 \quad &\wedge \quad &\homrestrictions(\updvar, \periodvar)\ .
\end{alignat*}
Consider the homogeneous reachability constraint for the center.
Since we have no productions, the variable $\termvarcenter$ will be zero. 
However, we will still collect updates, namely for the period vectors of the children. 
The support is as before. 



==> overview.tex <==

\newcommand{\HybridizationRelation}[0]{\trianglelefteq}
\newcommand{\vectSet}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\RelationClass}[0]{\mathcal{C}}
\newcommand{\ReachabilityRelation}[0]{\vectSet{R}}

\subsection{Overview on the Proof of Theorem \ref{TheoremGVASReachDecidable}}
In this section we provide an overview and intuition on the proof of Theorem \ref{TheoremGVASReachDecidable}.

We started from a smaller problem, which helps for providing intuition: Is there some smaller class \(\updates\) of updates such that we can decide \gvassreach?

However, even for small classes, every proof attempt ran into the following problem: Let \(\ReachabilityRelation(\agram) \subseteq \N^d \times \N^d\) be the \emph{reachability relation}, i.e.\ the set of pairs of markings \(\amark_1, \amark_2\) s.t. there is $\arun\in\langof{\agram}$ so that $\amark_1\fires{\arun}\amark_2$. GVAS may fundamentally \emph{nest procedures} in the following sense: Once a GVAS \(\agram\) is defining some reachability relation \(\ReachabilityRelation(\agram) \subseteq \N^d \times \N^d\), then another GVAS \(\agram'\) may use \(\ReachabilityRelation(\agram)\) as an update (i.e.\ an update is now relation \(\subseteq \N^d \times \N^d\)). This led to the following question, whose answer allowed us to solve the problem:

\begin{quote}
Is there a class \(\RelationClass\) of relations \(\subseteq \N^d \times \N^d\), such that for every GVAS \(\agram\) with updates \(\updates \subseteq \RelationClass\), also \(\ReachabilityRelation(\agram) \in \RelationClass\)?
\end{quote}

I.e.\ we ask for a property which transfers from terminals to the GVAS reachability relation. We came up with the following solution, which happens to include all VASS updates (and hence solve problem \gvassreach):

\begin{definition} \label{DefinitionGoodOverapproximation}
Let \(\vectSet{X} \subseteq \vectSet{L} \subseteq \N^d \times \N^d\) be relations. Then \(\vectSet{L}\) is a \emph{nice overapproximation} of \(\vectSet{X}\) (written \(\vectSet{X} \HybridizationRelation \vectSet{L}\)) if 
\begin{enumerate}
\item \(\vectSet{X}\) is monotone, 
\item \(\vectSet{L}=\avec+\asetvec^{\ast}\) is linear and 
\item for every \(\vect{x} \in \vectSet{L}\) and every \(\vect{w} \in \asetvec^{\ast}+\sum_{\avec \in \asetvec}\avec\), there exists \(N \in \N\) such that \(\vect{x}+N \vect{w}+ \N \vect{w} \subseteq \vectSet{X}\). 
\end{enumerate}
\end{definition}
\begin{definition}
Let \(\RelationClass\) be a class of relations. Then \(\RelationClass\) is \emph{approximable} if there is an algorithm which given \(\vectSet{X} \in \RelationClass\) and a semilinear relation \(\vectSet{S}\) outputs \(\vectSet{X}_1, \dots, \vectSet{X}_r \in \RelationClass\) and linear relations \(\vectSet{L}_1, \dots, \vectSet{L}_r\) s.t. \(\vectSet{X} \cap \vectSet{S}=\bigcup_{i=1}^r \vectSet{X}_i\) and \(\forall\ 1 \leq i \leq r\) we have \(\vectSet{X}_i \HybridizationRelation \vectSet{L}_i\).
\end{definition}

Let us provide sufficient intuition on these two important properties. First of all, clearly any monotone linear relation like a VASS update \(+\vect{u}\) is a nice overapproximation of itself. However, relations \(\vectSet{X}\) with a nice overapproximation may be highly non-semilinear: For example \(\{(x,y) \mid y\leq x^2\} \subseteq \N \times \N\) has the nice overapproximation \(\N \times \N\): Since the vector \(\vect{w}\) has to take every period at least once, it is easy to find an appropriate \(N\) for every \(\vect{x}, \vect{w}\). Another important observation is that only \emph{non-empty relations} have a nice overapproximation.

Approximability then says that given some relation \(\vectSet{X} \in \RelationClass\) and its ``section'' (as in intersection with \(\vectSet{S}\)) we want to analyze, we can get a decomposition \(\vectSet{X} \cap \vectSet{S}=\bigcup_{i=1}^r \vectSet{X}_i\) and corresponding nice overapproximations. Now let us officially state that approximability is \emph{the} magical property:

\begin{theorem}\label{TheoremApproximabilityOfGVAS}
Let \(\RelationClass\) be an approximable class of relations. 

Then the class \(\RelationClass'\) of all reachability relations of GVAS with updates in \(\RelationClass\) is approximable.
\end{theorem}

This clearly suffices to prove Theorem \ref{TheoremGVASReachDecidable}:

\begin{proof}[Proof of Thm. \ref{TheoremGVASReachDecidable}]
The class of VASS updates is approximable, since they are monotone linear relations. By Theorem \ref{TheoremApproximabilityOfGVAS}, therefore also GVAS reachability relations are approximable. Hence to check whether \((\amark_1, \amark_2) \in \ReachabilityRelation(\agram)\), we approximate \(\ReachabilityRelation(\agram)\) along the semilinear relation \(\{(\amark_1, \amark_2)\}\) to obtain \(\vectSet{X}_1, \dots, \vectSet{X}_r\) with \(\bigcup_{i=1}^r \vectSet{X}_i=\ReachabilityRelation(\agram) \cap \{(\amark_1, \amark_2)\}\). Now if \(r>0\), then since relations with a nice overapproximation are non-empty, we now that \((\amark_1, \amark_2) \in \ReachabilityRelation(\agram)\), and otherwise \((\amark_1, \amark_2) \not \in \ReachabilityRelation(\agram)\).
\end{proof}

Hence in the rest of the paper we prove Theorem \ref{TheoremApproximabilityOfGVAS}. Step 1 of the proof loops back to the problem at the start: We explained that a GVAS \(\agram'\) using \(\ReachabilityRelation(\agram)\) as subprocedure was difficult to deal with. Now it is the opposite: If we can isolate a class \(\RelationClass'\) of subprocedures and prove it is approximable, then we can forget about the specific implementation of \(\RelationClass'\) and view the procedure calls as \emph{atomic actions}. This leads us in later sections to the data structure of nested GVAS, which is an implementation of the following observation:

\begin{lemma}
In the proof of Theorem \ref{TheoremApproximabilityOfGVAS}, we may without loss of generality assume that \(\agram\) is strongly-connected.
\end{lemma}

Next observe that strongly-connected grammars fall into one of two cases: Either \(\agram\) is linear or non-linear. Both these two cases have their advantages and disadvantages, and we will separately deal with them going forwards. In the case of linear grammars and nestings thereof, GVAS reachability is in fact already known to be decidable. However, since we have to prove approximability, which is stronger than deciding reachability, we have to deal with that case again regardless.

In this overview we only consider the other, fully unknown case of non-linear grammars \(\agram\). In this case we will, similar to deciding reachability in normal VAS, search for runs of the following form: \[\amark_1 \to^{\ast} \text{Large}_k \to^{\ast} \text{Large}_k' \to^{\ast} \amark_2,\] where \(\text{Large}_k, \text{Large}_k'\) are gigantic configurations of linear size in some parameter \(k\). Proving that one can reach arbitrarily gigantic configurations (not caring which configuration exactly) is an easier class of reachability queries called coverability. There is a later section focussed on coverability, in this overview we focus on the other part: How to now prove that \(\text{Large}_k \to^{\ast} \text{Large}_k'\) for all large enough \(k\)? 

The informal idea is the following: Ensure the configurations are large, such that the VAS does not care about the word \(\asentform\) anymore, only that the tree producing it has \emph{low height}. Finally, because the grammar is non-linear, one can produce (most) long words \(\asentform\) via trees of logarithmic height.

More formally, the idea is as follows, for the details see Section \ref{Section:IterationLemma}: We start with a vector \(\avarp_k\in\N^{\updates}\) such that \(\meof{\updates}{\text{Large}_k, \avarp_k, \text{Large}_k'}\) fulfills the marking equation, and from \(\avarp_k\) obtain a tree \(\atreedef\) with \(\yieldof{\atreedef}=\asentform_k\) and \(\paramparikhof{\updates}{\asentform_k}=\avarp_k\) via Theorem \ref{Theorem:EEK}. So far these steps are similar to VAS, one important novelty is next: We \emph{take advantage of non-linearity}: By Theorem \ref{TheoremWideTree}, if a word \(\asentform_k\) can be derived by a tree with parikh image $\paramparikhof{\prods}{\atreedef}=k \cdot \avec_{\prods}\), then some permutation \(\pi(\asentform_k)\) of \(\asentform_k\) can be derived by a tree of height \emph{logarithmic} in \(k\). In terms of the VAS, the height of the tree will correspond to the hurdle $\hurdleof{\arun}$ of the corresponding run \(\arun\). Hence we have \(\text{Large}_k \xrightarrow{\pi(\asentform_k)}\) in the VAS for all large enough \(k\), because \(\text{Large}_k\) grows linearly in \(k\), while the hurdle of the run scales logarithmically in \(k\). Importantly, the permuted word \(\pi(\asentform_k)\) still has the same effect in the VAS as \(\asentform_k\), and hence \(\text{Large}_k \xrightarrow{\pi(\asentform_k)}\text{Large}_k'\), as \(\paramparikhof{\updates}{\asentform_k}=\avarp_k\) was a solution to the marking equation.



==> perf_conditions.tex <==
\subsection{Perfectness (MEANT FOR THE AUTHORS)}
We define perfectness conditions on NGVAS that allow us to construct reaching runs. 
The corresponding iteration lemma is our first technical achievement. 
Let $\anngvas=(\agram, \restrictions, \acontext, \boundednessinformation)$ have the restriction $\restrictions = \baseeffect+\periodeffect^*$.
Let the sets of unbounded counters be $\adimsetleft, \adimsetright\subseteq [1, \adim]$ with  $\adimsetleft=\adimsetright$ in the non-linear case.  
We call $\anngvas$ \emph{perfect}, if \perfectnesssol to \perfectnesschildren hold: 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\begin{description}[leftmargin=0cm, labelsep=-0.05cm,itemsep=4pt]
\item[\perfectnesssol] For every $\baseeffectchoice\in\restrictions$ there is a solution $\asol$ to $\chareq{\anngvas}$ with $\asol[\updvar]=\baseeffectchoice$. 
For every $\periodeffectchoice\in\N^{\periodeffect}$ with $\periodeffectchoice\geq 1$ there is a full homogeneous solution $\ahomsol$ to $\homchareq{\anngvas}$ with $\ahomsol[\updvar]=\periodeffect\cdot \periodeffectchoice$. 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnesscounters] All unbounded counters in a reachability constraint are in the support. This is understood in two parts.
\begin{itemize}
    \item[\perfectnesscountersctx] We have $\at{\invar}{\omegaof{\acontextin}}, \at{\outvar}{\omegaof{\acontextout}}\subseteq \suppof{\homchareq{\anngvas}}$.
    \item[\perfectnesscountersin] If $\anngvas$ is linear, $\at{\invardir}{\omegaof{\acontextindir}}, \at{\outvardir}{\omegaof{\acontextoutdir}}\subseteq\suppof{\homchareq{\anngvas}}$ for $\mydir\in\set{\mycenterleft, \mycenterright}$. 
\end{itemize} 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnesschildren] All subNGVAS $\anngvasp\in \anngvas$ are perfect. 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnessbase] The base effects of all childNGVAS are enabled, for all $\anngvasp\in\terms$ with restriction $\baseeffectdef+\periodeffectdef^*$ there is $\baserundef\in\runsof{\anngvasp}$ with $\paramparikhof{\updates}{\baserundef}=\baseeffectdef$.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnesschildperiodsbd] For linear $\anngvas$, and center childNGVAS $\anngvasp\in\terms$, and $\mydir\in\set{\mycenterleft, \mycenterright}$ we have $\periodeffectvardef, \periodeffectvardefdir\subseteq\suppof{\homchareq{\anngvas}}$.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\ek{I merged two conditions, these always appear together}
%\item[\perfectnesschildperiodsunb]  All period vectors in the restrictions of all childNGVAS $\anngvasp\in\terms$ that can be produced in cycles are in support. That is, for all $\mydir$ we have $\periodeffectvardef, \periodeffectvardefdir\subseteq \suppof{\homchareq{\anngvas}}$. 
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnessprods]  All productions, as well as all period vectors in the restrictions of childNGVAS $\anngvasp\in\terms$ that can be produced in cycles are in support. That is, for all $\mydir$ we have $\prodvar, \periodeffectvardef, \periodeffectvardefdir\subseteq \suppof{\homchareq{\anngvas}}$.
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\item[\perfectnesspumpingint]
This requirement only applies in the linear case and is our second measure to circumvent the wide tree thereom. 
It says that there are internal down-pumping and up-pumping runs. 
There are runs $\downseqint.\upseqint\in\runsof{\asentformpumpleftint.\asentformpumprightint}$ resulting from $\startnonterm\rightarrow \asentformpumpleftint.\startnonterm.\asentformpumprightint$ and markings $\inmarkint, \outmarkint\in\N^{\adim}$ with $\inmarkint\sqsubseteq \acontextincenterleft, \outmarkint\sqsubseteq \acontextoutcenterright$ so that $\inmarkint\fires{\revof{\downseqint}}\amark_3$ and $\outmarkint\fires{\upseqint}\amark_4$. 
The runs have an effect $(\amark_3-\inmarkint)[\adimsetleft\setminus \omegaof{\acontextinint}]\geq 1$ and $(\amark_4-\outmarkint)[\adimsetright\setminus \omegaof{\acontextoutint}]\geq 1$. 

\item[\perfectnesspumping]
There are up-pumping and down-pumping runs. 
There are runs $\upseq.\downseq\in\runsof{\asentformpumpleft.\asentformpumpright}$ resulting from a derivation $\startnonterm\rightarrow \asentformpumpleft.\startnonterm.\asentformpumpright$ and 
there are markings  $\inmark, \outmark\in\N^{\adim}$ with $\inmark\sqsubseteq \acontextin$ and $\outmark\sqsubseteq \acontextout$ so that $\inmark\fires{\upseq}\amark_1$ and $\outmark\fires{\revof{\downseq}}\amark_2$. 
The runs have a strictly positive effect on counters that become $\omega$ in $\adimsetleft$ but are not $\omega$ in the input marking respectively a strictly negative effect on the counters that are $\omega$ in $\adimsetright$ but not  $\omega$ in the output marking, $\at{(\amark_1-\inmark)}{\adimsetleft\setminus \omegaof{\acontextin}}\geq 1$ and, due to the reversal, $\at{(\amark_2-\outmark)}{\adimsetright\setminus \omegaof{\acontextout}}\geq 1$. 
 % ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
% ----------------------------------------------------------------------------------
\end{description}

==> perfectnessbackup.tex <==
\section{Perfectness}
Let $\anngvas=(\agram, \restrictions, \acontext, \boundednessinformation)$ be an NGVAS and $\adimset\subseteq [1, d]$ the set of counters that may obtain arbitrarily high values.  
We call $\anngvas$ \emph{perfect}, if the following holds
\begin{itemize}
\item[(P0)] For every $\baseeffectchoice\in\restrictions$ there is a solution $\asol$ to $\charof{\anngvas}$ with $\asol[\anupdvec]=\baseeffectchoice$. 
\item[(P1)] All unbounded counters in the input and output markings $\acontextin$ and $\acontextout$ belong to the support: $\invar[\omegaof{\acontextin}], \outvar[\omegaof{\acontextout}]\subseteq \suppof{\chareq{\anngvas}}$. 
\item[(P2)] All productions of $\agram$ are in the support, $\prodvar\subseteq\suppof{\chareq{\anngvas}}$.
\item[(P3)] All period vectors in the restrictions of all childNGVAS belong to the support, for all $\anngvasp\in\terms$ we have $\periodeffectvardef\subseteq \suppof{\chareq{\anngvas}}$.  
\item[(P4)] The base effects of all childNGVAS are firable: for all $\anngvasp\in\terms$ with restriction $\baseeffectdef+\periodeffectdef^*$ there is $\arun\in\runsof{\anngvasp.\agram}$ with $\anngvasp.\acontextin\fires{\arun}\anngvasp.\acontextout$ and $\paramparikhof{\updates}{\arun}=\baseeffectdef$.
\item[(P5)] There is a derivation $\startnonterm\xrightarrow{\aprodseqpump} \upseq.\startnonterm.\downseq$ giving up/down-pumping sequences $\upseq, \downseq\in\updates^*$. 
There are markings $\amark_{\myin}, \amark_{\myout}\in\N^{\adim}$ with $\amark_{\myin}\sqsubseteq \acontextin$ and $\amark_{\myout}\sqsubseteq \acontextout$ that allow us to execute the sequences $\amark_{\myin}\fires{\upseq}\amark_1$ and $\amark_{\myout}\fires{(-\downseq)^{-1}}\amark_2$. 
Moreover, the sequences have a strictly positive effect on counters that become $\omega$ in $\adimset$ but are not yet $\omega$ in the input and output markings: $(\amark_1-\amark_{\myin})[\adimset\setminus \omegaof{\acontextin}]\geq 1$ and $(\amark_2-\amark_{\myout})[\adimset\setminus \omegaof{\acontextout}]\geq 1$.
\item[(P6)] All subNGVAS $\anngvasp\in \anngvas$ are perfect. 
\end{itemize}

==> proof_outline_complexity.tex <==
\subsection{Complexity}
It remains to define the rank of an NGVAS and analyze the complexity of our decision procedure. 
For the latter, we employ a precise analysis of recursive procedures, which we believe will be of independent interest.
%  ---------------------------------------------------------
%  ---------------------------------------------------------
%  ---------------------------------------------------------
%  ---------------------------------------------------------
\subsubsection{Bad Partially Nested Sequences} \label{SubSubsectionPartiallyNestedSequences}

Recursions with ranks from \(\N^{\beta}\) for  \(\beta \in \N\) are common in the context of infinite-state systems, and there are generic tools for analyzing their complexity: \emph{controlled bad sequences} for tail recursions~\cite{FigueiraFSS11} and \emph{controlled bad nested sequences} for full (non-tail) recursions~\cite{LerouxPS14}. 
Theorem VI.1 in \cite{LerouxPS14} gives Hyper-Ackermann time bounds for full recursions. 

There is, however, a problem with these generic tools: they analyze all procedures equally but do not consider the case where some procedures are tail-recursive and others are fully recursive. 
To take into account this distinction, we now introduce controlled bad \emph{partially nested} sequences, a subclass of controlled bad nested sequences that admit a finer complexity analysis.  

\newcommand{\astack}{\mathit{s}}
\newcommand{\ansf}{\mathit{y}}
\newcommand{\setfun}{\mathit{P}}
\newcommand{\afun}{\mathit{f}}
\newcommand{\afunp}{\mathit{g}}
\newcommand{\aglob}{\mathit{u}}
\newcommand{\aglobp}{\mathit{v}}
\newcommand{\aloc}{\mathit{a}}
\newcommand{\alocp}{\mathit{b}}
\newcommand{\grank}{\mathit{r}}
\newcommand{\grankof}[1]{\mathit{r}(#1)}
\newcommand{\gdom}{\mathsf{U}}
\newcommand{\ldomof}[1]{\mathsf{A}_{#1}}
\newcommand{\ldomdef}{\ldomof{\afun}}
\newcommand{\wfdom}{\mathsf{X}}
\newcommand{\lwfdomof}[1]{\wfdom_{#1}}
\newcommand{\lwfdomdef}{\lwfdomof{\afun}}
\newcommand{\funrank}[1]{\mathit{r}_{#1}}
\newcommand{\funrankof}[2]{\funrank{#1}(#2)}
\newcommand{\funrankdef}{\funrank{\afun}}
\newcommand{\funrankdefof}[1]{\funrankdef(#1)}

\newcommand{\domsf}{\mathsf{Y}}
\newcommand{\aheight}{\mathit{h}}

\newcommand{\controlfun}{\mathit{c}}
\newcommand{\controlfunof}[1]{\controlfun(#1)}
\newcommand{\initbound}{\mathit{m}}

\newcommand{\infnormof}[1]{|\!|#1|\!|_{\infty}}
\newcommand{\leqlex}{\leq_{\mathit{lex}}}

\newcommand{\fastgrowof}[1]{\mathfrak{F}_{#1}}

\newcommand{\amainrank}{\mathit{x}}
\newcommand{\anauxrank}{\mathit{z}}

\newcommand{\acomp}{\tau}
\newcommand{\absof}[1]{\alpha(#1)}
\newcommand{\aseq}{\sigma}

We explain the programming model that we use for our complexity analysis.  
The essential characteristic of our decision procedure is that (i) it is heavily recursive but (ii) the recursive functions all have the same type, they map NGVAS to sets of NGVAS.
To capture this, we define a recursive program as a finite set of functions $\setfun$ that all have type $\gdom\rightarrow \powof{\gdom}$ for some domain~$\gdom$.  
During its computation, each function $\afun\in\setfun$ may transform the input, meaning it has access to state from $\gdom$. 
Moreover, the function may maintain auxiliary state from some domain $\ldomdef$. 
An example for such auxiliary state is the Karp-Miller tree. 
We do not need to be precise about the syntax of programs and can also be rough about the semantics.  
In fact, even the domains we just introduced will be abstracted away by ranking functions. 
This high level of abstraction is needed to deal with objects as complicated as NGVAS and functions as complicated as $\postfuncN{\anngvas}$. 
We only need stack frames $\ansf=(\aglob, \afun, \aloc)$ which consist of state $\aglob\in\gdom$, the current function $\afun\in\setfun$, and auxiliary state $\aloc\in\ldomdef$. 
A stack is then a finite sequence of stack frames $\astack=\ansf_0\ldots \ansf_k$ with $\ansf_k$ being topmost.  

We are interested in proving the termination of such recursive programs. 
To this end, we assume to have a ranking function \(\grank:\gdom\rightarrow \wfdom\) that maps the state from $\gdom$ into a well-founded total order $\wfdom$. 
With $\gdom$ being NGVAS, the function $\grank$ will define their rank. 
Moreover, for every function \(\afun \in \setfun\), we need a ranking function \(\funrankdef:\ldomdef\rightarrow\lwfdomdef\) that maps the auxliary state into another well-founded total order. While this auxiliary ranking function $\funrankdef$ may be chosen depending on the function $\afun\in\setfun$, we expect that all functions in the program agree on $\grank$, and we refer to it as the main rank. 
Finally, we assume to have a total order $\prec$ on the functions in program $\setfun$. 

The goal of our complexity analysis is to separate recursive from tail-recursive behavior.
We achieve this by constraining the transition relation $\astack_1\rightarrow \astack_2$ between stacks, and analyzing computations that adhere to these constraints.  
An invariant of our transitions is that they do not increase the main rank.  
Moreover, recursive calls have to (i) reduce the main rank or (ii) call a function that is smaller in the total order on functions.  
The consequence is that transitions which only reduce the auxiliary rank cannot be recursive calls: computation on the auxiliary state has to be tail-recursive. 
We admit the following.     
\begin{enumerate}
\item A tail-recursive step $\astack.(\aglob, \afun, \aloc)\rightarrow \astack.(\aglobp, \afun, \alocp)$ and a return step from a recursive function $\astack.(\aglob, \afun, \aloc).(\aglob', \afun', \aloc')\rightarrow \astack.(\aglobp, \afun, \alocp)$, provided the main rank does not go up and a rank goes down: $\grankof{\aglob}\geq\grankof{\aglobp}\wedge (\grankof{\aglob}>\grankof{\aglobp}\vee \funrankdefof{\aloc} >\funrankdefof{\alocp})$. 
\item A recursive call  $\astack.(\aglob, \afun, \aloc)\rightarrow \astack.(\aglob, \afun, \aloc).(\aglobp, \afunp, \alocp)$, provided the main rank does not go up, and the main rank goes down or the callee is smaller,  $\grankof{\aglob}\geq\grankof{\aglobp}\wedge (\grankof{\aglob}>\grankof{\aglobp}\vee \afun\succ \afunp)$. 
\end{enumerate}
Note that the auxiliary state can be chosen freely if we can ensure the main rank goes down.

It is readily checked that from every initial stack every computation in our model terminates. 
The reason is that a computation is a sequence in \(\wfdom \times \setfun \times \bigcup_{f} \lwfdomdef\) that is strictly decreasing in the lexicographic ordering, and this ordering is well-founded. 
This is enough to show termination of our decision procedure. 

To estimate the complexity, we need notions from fast-growing complexity. 
By further abstracting from stack frames and even stacks, we arrive at the nested sequences from~\cite{LerouxPS14}. 
Towards this abstraction, note that our termination analysis does not need the domains $\gdom$ and $\ldomdef$, but only the well-founded total orders. 
We fix them to $(\N^{\beta}, \leqlex)$.   
Then (the abstract version of) a stack frame is an element from \(\domsf=\N^{\beta_1} \times \setfun \times \N^{\beta_2}\). 
We also abstract away the stack content and only keep the topmost stack frame and the height of the stack. 
With this, (the abstract version of) a stack is an element $(\ansf, \aheight)\in\domsf\times\N$. 
The abstraction of a computation is a \emph{nested sequence}, a sequence of stacks $(\ansf_0, \aheight_0).(\ansf_1, \aheight_1)\ldots$ whose height changes as expected, $\aheight_{k+1} \in \aheight_k + \{-1,0,1\}$ for all $k\in\N$. 
To capture the requirement that every transition decreases the rank, it has become common to formulate the contrary, the moment of termination. 
A nested sequence is \emph{good}~\cite{LerouxPS14}, if there are indices $k<m$ so that $\ansf_k \leqlex \ansf_m$ and $\aheight_{k+1}, \dots, h_m \geq \aheight_k$. 
It is \emph{bad} if it is not good. 

Our complexity analysis determines a bound on the length of bad nested sequences. 
This also yields a bound on the termination time for our programming model, in particular for our decision procedure, with the following argument. 
For every computation $\acomp=\astack_0\rightarrow\astack_1\rightarrow\ldots$ in a program, the abstraction $\absof{\acomp}=(\ansf_0, \aheight_0).(\ansf_1, \aheight_1)\ldots$is a bad nested sequence.
To see this, note that the definition of a good sequence essentially negates the enabledness conditions of all transitions in our model. 

To determine a bound on the length of bad sequences, we need some means to control the way in which transitions can modify the ranks~\cite{FigueiraFSS11}. 
Let $\controlfun \colon \N \to \N$ be a strictly increasing (control)  function and let $\initbound \in \N$ be a bound on the size of the initial stack. 
The nested sequence $(\ansf_0, \aheight_0).(\ansf_1, \aheight_1)\ldots$ is \emph{$(\controlfun, \initbound)$-controlled}~\cite{LerouxPS14} if $\sizeof{\ansf_k} \leq \controlfun^{(k)}(\initbound)$ for all \(k\in\N\). Here, we use \(\controlfun^{(k)}\) for the \(k\)-fold application of \(\controlfun\). 
Note that the boundedness of the stack frames is not built into our programming model. 
So to employ controlled sequences for the complexity analysis, we need to argue that our transitions respect the bounds. 
This, however, will be unproblematic as we will admit general primitive-recursive control functions. 

Recall that \(\wfdom=\N^{\beta_1}\) and \(\lwfdomdef=\N^{\beta_2}\).
Even if we control the transitions to only increment and decrement the counters in the rank, the best upper bound on the length of controlled bad sequences that can be shown with techniques in the literature is $\fastgrowof{\cardof{\setfun}\cdot \omega^{\beta_1+\beta_2}}$, obtained from \cite[Theorem VI.1]{LerouxPS14}. 
Here, $\fastgrowof{\alpha}$ stems from the hierarchy of fast-growing functions, and we refer the reader to~\cite{Schmitz16} for details.  
With our analysis, transitions are allowed to take an arbitrary primitive-recursive amount of time, and we can improve the upper bound to \(\fastgrowof{\omega^{\beta_1}}\). Observe that this eliminates the dependence on \(\beta_2\) and on \(\cardof{\setfun}\). 

What allows us to improve the analysis is the fact that, in our programming model, computation on the auxiliary rank has to be tail-recursive. 
Note that this has not been taken into account in the above definition of nested sequences.  
Recall that $\domsf=\N^{\beta_1} \times \setfun \times \N^{\beta_2}$. 
%We introduce the restriction as follows. 
% -----------------------------------------------------
% -----------------------------------------------------
% -----------------------------------------------------
% -----------------------------------------------------
\begin{definition}
A nested sequence $(\ansf_0, \aheight_0).(\ansf_1, \aheight_1)\ldots$ is \emph{partially nested} if $\ansf_k=(\amainrank, \afun, \anauxrank_k)$ and $\ansf_{k+1}=(\amainrank, \afun, \anauxrank_{k+1})$ implies \(\aheight_{k+1} \leq \aheight_k\), for all $k\in\N$.
\end{definition}
% -----------------------------------------------------
% -----------------------------------------------------
We are allowed to analyze the length of controlled bad  partially nested sequences, because the abstraction $\absof{\acomp}$ of a computation $\acomp$ in our model is not only a bad nested sequence but actually a bad partially nested sequence.
The bound we obtain with this analysis will also be precise, as we have the following. 
For every bad partially nested sequence sequence $\aseq=(\ansf_0, \aheight_0).(\ansf_1, \aheight_1)\ldots$ there is a computation $\acomp=\astack_0\rightarrow\astack_1\rightarrow\ldots$ so that $\aseq=\absof{\acomp}$.
% -----------------------------------------------------
% -----------------------------------------------------
% -----------------------------------------------------
% -----------------------------------------------------

We explain how partially nested sequences eliminate the dependence on \(\beta_2\) and \(\cardof{\setfun}\). 
Consider the case where \(\beta_1=1\) and so \(\domsf=\N \times \setfun \times \N^{\beta_2}\). 
Assume we start with value \(k\in\N\) for the main rank. 
Then a partially nested sequence can be modelled as a tail recursion with a rank in \(\N^{(k+1) \cardof{\setfun} \cdot \beta_2}\), with the following argument.
At every moment in the sequence, the call stack has height at most \((k+1) \cardof{\setfun}\). 
We can store the \((k+1)\cardof{\setfun}\) auxiliary ranks that lie on the stack in a long tuple. 
Using the bad sequence analysis of \cite[Prop. 5.2]{FigueiraFSS11}, we arrive at a complexity of \(\fastgrowof{(k+1)\cardof{\setfun} \cdot \beta_2}\subseteq \fastgrowof{\omega}\).  
In fact, already \(\beta_1 = 1 = \beta_2=\cardof{\setfun}\) would lead to \(\fastgrowof{\omega}\), as one can directly implement the Ackermann function. 
The consequence is that the details \(\beta_2\) and \(\cardof{\setfun}\) vanish once we round up to the next power of \(\omega\), which will always be \(\omega^{\beta_1}\).

\begin{theorem} \label{TheoremLengthBoundBadPartiallyNestedSequences}
Let \(\beta_1, \initbound, \beta_2 \in \N\) and let \(\cardof{\setfun}\) be finite. 
Let \(\alpha\) be an ordinal and let \(\controlfun\in \fastgrowof{\alpha}\) be strictly increasing. 
Then the length of \((\controlfun, \initbound)\)-controlled bad partially nested sequences over \(\N^{\beta_1} \times \setfun \times \N^{\beta_2}\) is in $\fastgrowof{\omega^{\beta_1}+\alpha}$.
\end{theorem}

\newcommand{\LexDec}[0]{\mathsf{LexDec}}
\newcommand{\LexDecof}[1]{\LexDec(#1)}
\newcommand{\maxlength}{\mathit{L}}
\newcommand{\maxlengthof}[2]{\maxlength_{#1}(#2)}
\newcommand{\vect}[1]{\mathbf{#1}}
\begin{proof}
The first observation is that we can get rid of $\setfun$. 
We set \(\beta_2'=\beta_2 \cdot \cardof{\setfun}\) and store the auxiliary ranks of one call for every function \(\afun\) in a common larger rank from \(\N^{\beta_2'}\). 

The proof has two steps: we analyze the shape of worst-case controlled bad partially nested sequence to obtain a recursive formula, and then we fiddle with the numbers to arrive at exactly the definition of the fast-growing functions \(\fastgrowof{\alpha}\).

Given an ordinal \(\alpha< \omega^{\omega}\) in Cantor normal form, let $\min(\alpha)$ % \in \{0,\dots, d-1\}\) 
be the smallest exponent \(i\) so that \(\alpha\) contains \(\omega^i\). 
We define the worst-case \emph{lexicographic decrement} as the function \(\LexDecof{\alpha, n}=\alpha-\omega^{min(\alpha)}+\sum_{j<\min(\alpha)} \omega^{j}\cdot n\). 
So from $\LexDecof{\omega^3+\omega^2\cdot 5, n}=\omega^3+\omega^2\cdot 4 + \omega\cdot n + n$. 
%It takes \(\alpha\) and a number \(n \in \N\) as input and lexicographically decrements \(\alpha\) in such a way that the maximum norm does not exceed \(n\).

Let \(\maxlengthof{\amainrank, \anauxrank,\controlfun}{\initbound}\) be the maximal length of an \((\controlfun,\initbound)\)-controlled bad partially nested sequence starting at \((\amainrank, \anauxrank) \in \N^{\beta_1} \times \N^{\beta_2'}\). 
We obtain a recursive formula for \(\maxlengthof{\amainrank, \anauxrank, \controlfun}{\initbound}\) by considering the worst-case behavior the bad sequence can show. 
A step in the sequence may execute a push on the stack, and thereby turn \((\amainrank, \anauxrank, \aheight=0)\) into \((\LexDecof{\amainrank, \controlfunof{\initbound}}, \controlfunof{\initbound}, \aheight=1)\).
We then execute a bad nested sequence on this smaller new value.  
After a large amount of time \(t\), we return to \((\amainrank, \LexDecof{\anauxrank, \controlfun^{(t)}(\initbound)}, \aheight=0)\) and perform a bad nested sequence from there.

By formalizing this argument, one obtains the so-called \emph{descent equation} \(\maxlengthof{\amainrank, \anauxrank, \controlfun}{\initbound}=l_1+l_2\), where 
\begin{align*}
l_1 &=\maxlengthof{\LexDec(\amainrank, \controlfun(\initbound)), \controlfun(\initbound), \controlfun}{\controlfun(\initbound)} \\
l_2 &=\maxlengthof{\amainrank, \LexDec(\anauxrank, \controlfun^{(l_1+1)}(\initbound)),\controlfun}{\controlfun^{l_1+1}(\initbound)}
\end{align*} are respectively the lengths of the first and second half of the worst-case sequence above.

The main reason this equation is difficult is because every part deals with nested sequences. We will now obtain a simpler recursive formula only using lengths of non-nested sequences via an idea motivated by the \(\beta_1=1\) case: For \(\beta_1=1\), starting at \(k\), we can bound \(\maxlength_{k, \anauxrank, \controlfun}\) by a non-nested sequence in \(\N^{\beta_2}\) whose control function is \(\maxlength_{k-1, \anauxrank, \controlfun}\). 

The core of the proof is hence the following: We define a new control function \(\controlfun_{\amainrank} \colon \N \to \N, \initbound \mapsto 2 \cdot \maxlengthof{\LexDec(\amainrank, \controlfun(\initbound)), \controlfun(\initbound), \controlfun}{\controlfun(\initbound)}\), i.e.\ we map \(\initbound\) to twice the size of \(l_1\). Observe in particular that \(l_1\) indeed does not depend on \(\anauxrank\). The above worst-case partially nested sequence \emph{gives rise} to a \((\controlfun_{\amainrank}, \initbound)\)-controlled \emph{non-nested} bad sequence in \(\N^{\beta_2}\) by considering the subsequence of all entries where \(\amainrank=\amainrank_0\) retains the original value and \(\aheight=0\). This allows us to obtain a bound on \(\controlfun_{\amainrank}\) and then \(\maxlengthof{\amainrank, \anauxrank, \controlfun}{\initbound}\) by using usual non-nested bad sequence bounds.

Let \(\maxlengthof{nn,\beta_2,\controlfun}{\initbound}\) be the length of the longest \((\controlfun, \initbound)\)-controlled bad non-nested sequence in \(\N^{\beta_2}\), here \(nn\) stands for ``non-nested''. The above shows \(\maxlengthof{\amainrank, \anauxrank, \controlfun}{\initbound} \leq (\maxlengthof{nn, \beta_2, \controlfun_{\amainrank}}{\initbound})^2,\) where we have to square because the new sequence only contains the \(h=0\) steps. In the worst-case, between all \(h=0\) nodes we again have \(\maxlengthof{nn, \beta_2, \controlfun_{\amainrank}}{\initbound}\) many steps each. Let \(\alpha_{\amainrank}\) be an ordinal s.t. \(\controlfun_{\amainrank} \in \mathfrak{F}_{\alpha_{\amainrank}}\). Using the usual bound for non-nested bad sequences, this formula shows \(\maxlength_{\amainrank, \anauxrank,\controlfun} \in \mathfrak{F}_{\alpha_{\amainrank}+\beta_2}\). It hence remains to obtain a bound on \(\alpha_{\amainrank}\). 

As last part of the proof, we hence prove by induction on \((\N^{\beta_1}, \leq_{\text{lex}})\) that \(\alpha_{\amainrank} \leq \amainrank \beta_2+\alpha\). The main step is to write a recursive formula formula for \(\controlfun_{\amainrank}\) as follows, following immediately from the above.
\begin{align*}
\controlfun_{\amainrank}(\initbound)&=_{\text{def}} 2 \cdot \maxlengthof{\LexDec(\amainrank, \controlfun(\initbound)), \controlfun(\initbound), \controlfun}{\controlfun(\initbound)}\\
&\leq (\maxlengthof{nn, \beta_2, \controlfun_{\LexDec(\amainrank, \controlfun(\initbound))}}{\initbound})^2.
\end{align*}
To show \(\alpha_{\amainrank} \leq \amainrank \beta_2+\alpha\), the actual proof is a computation which is almost the same as in \cite[Theorem VI.1]{LerouxPS14}. Instead of repeating it, let us explain the intuitive reason. By inspecting the definition of the fast-growing functions \(F_{\amainrank}\), we observe that they can equivalently be defined as \(F_{\amainrank}(\initbound):=F_{\LexDec(\amainrank, \initbound-1)}^{(\initbound)}(\initbound)\). I.e.\ the difference between \(\controlfun_{\amainrank}\) and \(F_{\amainrank}\) is that the definition of \(F_{\amainrank}\) consists of repeated application, while \(\controlfun_{\amainrank}\) performs a larger lexicographic decrement \(\LexDec(\alpha, \controlfun(\initbound))\) (and contains squaring and length of a non-nested sequence). To compensate the latter, we need \(F_{\amainrank \beta_2 + \alpha}\) instead of \(F_{\amainrank}\) for it to be an upper bound on \(\controlfun_{\amainrank}\).
\end{proof}






\subsubsection{Rank of an NGVAS}\label{Section:OutlineRanks}
Let \(d\) be the number of counters. 
The rank of an NGVAS belongs to the set \(\N^{d+3} \times \N^{4d+1}\) which we order lexicographically, or equivalently the rank is an ordinal \(\leq \omega^{5d+4}\). The split as \(\N^{d+3} \times \N^{4d+1}\) corresponds to the \(\beta_1\) and \(\beta_2\) in Theorem \ref{TheoremLengthBoundBadPartiallyNestedSequences}: Our procedures will only be fully recursive in the front part of the rank. 

The main components of the rank are similar to VASS, i.e.\ use the dimension of the cycle space as Leroux and Schmitz in \cite{LerouxS19}. Before we define this in detail, let us first explain where the split between the recursive and non-recursive part comes from by comparing to VASS \cite{LerouxS19} and VASS with nested zero tests/bounded index PVASS \cite{Reinhardt08, AtigG11, GuttenbergCL25}. The perf function for VASS is in fact tail-recursive, hence the rank is purely the second type. More interesting are VASS with nested zero tests/finite-index PVASS: While Reinhardt in \cite{Reinhardt08} used a very complicated rank, \cite{GuttenbergCL25} recently simplified it to the following: The corresponding function perf uses arbitrary recursion in terms of the index of the grammar, however the index \emph{never increases} throughout the computation. Hence the rank is \(\N^1 \times \N^{\beta_2}\), where the fully recursive part is given by the index of the underlying grammar. The latter part is the rank of a ``C-eVASS'' obtained by viewing lower index PVASS as atomic operations. \cite{GuttenbergCL25} therefore obtained an Ackermann upper-bound for reachability in VASS with nested zero tests/finite-index PVASS.

We will implement the latter rank one-to-one in NGVAS: The last component of the recursive NGVAS rank will be an index of a certain grammar, and the tail-recursive rank will be given by viewing a substructure of the NGVAS as a KLM sequence. Remember that an NGVAS is a nesting of strongly-connected context-free grammars (with some extra information). Every SCC can be either linear or non-linear, and the main part of our rank will only consider non-linear SCCs. For linear SCCs, we will define a notion of index by viewing any subNGVAS of a non-linear NGVAS as an alphabet letter. This trivially creates a grammar without non-linear SCCs, i.e.\ a finite-index grammar.

Formally, the rank $\rankof{\anngvas}\in\N^{5d+4}$ of an NGVAS $\anngvas$ is understood as a product $\rankof{\anngvas}=(\recrankof{\anngvas}, \itrankof{\anngvas})\in\N^{d+3}\times\N^{4d+1}$.
To make the order clear, we also express the rank as an ordinal where earlier components correspond to larger exponents.
I.e.\ we have $\rankof{\anngvas}=\omega^{4d+1}\cdot\recrankof{\anngvas}+\itrankof{\anngvas}$.

Both ranks are based on the dimensionality of the vector spaces spanned by cycle effects, similarly to the VASS rank by Leroux and Schmitz \cite{LerouxS19}. We proceed to define cycle spaces first. A \emph{cycle} on a non-terminal \(\anonterm\) is a derivation \(\anonterm \to^{\ast} w \anonterm w'\) for some words \(w, w' \in (\Z^d)^{\ast}\). In particular the cycle space of an SCC \(Q'\) depends on all SCCs \(Q''\) which can be reached from \(Q'\) \emph{while} still leaving a non-terminal in SCC \(Q'\). E.g. a production \(A \to AB\) causes the cycle space of \(A\) to depend on \(B\), while a production \(A \to B\) cannot be used in a cycle unless \(A\) is non-linear. 

We define the cycle space as the vector space spanned by the effects of the left halfs of cycles, i.e.\ 
\[\cyclespaceof{\anngvas}=\text{span} \{\vaseffof{w} \mid S \to wSw'\}.\]
We use only the left effects since we will mainly be considering the cycle space for non-linear components, where left and right cycle spaces coincide.
%The last (and therefore most important) component is \(d-|\unconstrained|\). Essentially, counters \(i \in \unconstrained\) have to be \(\omega\) in every context (even of childNGVAS) by definition of \(\unconstrained\), only the restrictions can impact them. The terminology for this type of counter is \(\Z\)-counter, and they are essentially harmless. Hence we actually have an NGVAS of lower dimension \(d-|\unconstrained|\). 
%This NGVAS should then have a lower rank. 

We can now return to the definition of \(\recrankof{\anngvas}\), which consists of three components.
%
Expressed as ordinal,
%
$$\recrankof{\anngvas}=\omega^{d+2}\cdot|\constrained|\;+\;\omega\cdot\srankof{\anngvas}\;+\;\grmindexof{\anngvas}.$$
The most significant component is $|\constrained|$, the number of constrained counters.
%
This guarantees Lemma \ref{LemmaBasicRankProperties}.

The second component $\srankof{\anngvas}$ is the maximal-branch rank.
%
In order to define this rank, we first assign to the top-level NGVAS and to every descendant \(\anngvasp\) a local rank \(\lrankof{\anngvasp}\). 
If the NGVAS \(\anngvasp\) is linear, then we define \(\lrankof{\anngvasp}=0\). Otherwise we define \(\lrankof{\anngvasp}:=\omega^{\dim(\cyclespaceof{\anngvasp})}\cdot |\anngvasp.N| \) as the number of non-terminals of the NGVAS in the \((\dim(\cyclespaceof{\anngvasp}))\)-th entry.
%Intuitively, the vector space dimension measures the number of independent cycle effects, and removing enough cycles from an SCC reduces \(\lrankof{\anngvasp}\).
%
We obtain $\srankof{\anngvas}$ by summing along paths from the top-level NGVAS down to an NGVAS of nesting depth zero \((\anngvasp_0, \dots, \anngvasp_m)\) and taking the maximum in the lexicographic ordering/as ordinal, \ 
$$\srankof{\anngvas}=\max_{\substack{(\anngvasp_0, \dots, \anngvasp_m)\text{ is a }\\ \text{ path in the NGVAS}}} \sum_{i=0}^m \lrankof{\anngvasp_i}.$$
As an example, if a grammar has two branches, one has a non-terminal of dimension \(1\) and \(2\) and the other has \(100\) non-terminals of dimension \(1\), then the first branch is the maximal one, hence the rank is \(\omega^2+\omega\). 

There are two important pieces of intuition regarding the maximal-branch rank. The first is that when applying the decomposition of Section \ref{Section:OutlinePumping} on a \(2\)-dimensional SCC, this has the potential to create an arbitrary, in particular arbitrarily deep, nesting of \(1\)-dimensional grammars. Therefore a single \(2\)-dimensional non-terminal should be considered worse than an arbitrary grammar where every cycle space has dimension \(1\). This is guaranteed by this definition.

Moreover, the maximal-branch rank is the best measure of the \emph{depth} of the call-tree of perf: No matter how many branches a grammar has, this does not lengthen any given branch of computation. Of course the width of the grammar is also relevant, but the intuition is that we can deal with every branch one after the other, hence the number of branches will be (indirectly) part of the linear rank \(\itrankof{\anngvas}\in\N^{4d+1}\).

Finally, the last component $\grmindexof{\anngvas}$ measures the index of call trees $\anngvas$ may generate before calling a non-linear NGVAS.
%%
%We have $\grmindexof{\anngvas}=0$ if $\anngvas$ has nesting depth zero or is non-linear.
%%
%If $\anngvas$ is linear, the index $\grmindexof{\anngvas}$ is the largest of $1+\max_{\anngvasp\in\trms}{\grmindexof{\anngvasp}}$, and $\min(\grmindexof{\anngvasp_{\lefttag}}, \grmindexof{\anngvasp_{\righttag}})+1$.\rfm{Left and right are not defined, and altogether I have a hard time reading out of this the index definition I am used to.}
%%
%This means that if $\anngvas$ can produce two or more terminals with index $i$ in the same tree, then $\anngvas$ itself has index $i+1$.
Let \(G\) be the grammar obtained by considering 1) every subNGVAS which is not on a maximal branch, and 2) every subNGVAS of a non-linear NGVAS as being alphabet letters. Since this grammar does not have non-linear SCCs, it has some finite index, and we let \(\grmindexof{\anngvas}:=index(G)\).

The iterative rank $\itrankof{\anngvas}\in\N^{4d+1}$ is only non-zero for linear NGVAS. One can prove that there is a unique maximal branch $(\anngvasp_{0}, \ldots, \anngvasp_{m})$ of \(\anngvas\) s.t. \(\anngvasp_0=\anngvas\) and \(index(\anngvasp_{l})=index(\anngvas)\) for every \(l\): Namely, if there were two children of index \(k\), then we ourselves would have index \(k+1\). We then interpret \((\anngvasp_{0}, \ldots, \anngvasp_{m})\) as a KLM-sequence with $2d$ counters, and assign it the rank of Leroux and Schmitz \cite{LerouxS19}.\rfm{Explain the convolution idea.}
%
We refer the reader to the appendix for details.



















\subsection{Analyzing PVASS using Theorem \ref{TheoremLengthBoundBadPartiallyNestedSequences}}

In this section we explain how to apply Theorem \ref{TheoremLengthBoundBadPartiallyNestedSequences} bounding the length of bad partially nested sequences to NGVAS. 

The basic design principle is that all procedures are fully recursive in \(\recrankof{\anngvas}\), and only in \(\recrankof{\anngvas}\). The other components of the termination argument, like the linear rank \(\itrankof{\anngvas}\), termination arguments inside a function, etc., will all fall into the local rank \(\N^{\beta_2}\).

Let us start with a very simple procedure and how to analyze it: The procedure to guarantee property \perfectnesssol stating that all children are perfect simply performs one perf call for every child. Of course this contains multiple recursive calls to perf, but this is unavoidable for every procedure. The important part is that \emph{all} these recursive calls apply perf to a child, i.e.\ an NGVAS \(\anngvasp\) whose recursive rank \(\recrankof{\anngvasp}\) is smaller, \(\recrankof{\anngvasp} < \recrankof{\anngvas}\). 

Hence the better way to view this procedure is to consider such perf calls to lower recursive rank as atomic operations, and then the procedure for property \perfectnesssol is only a for loop, or equivalently a tail recursion. In terms of Definition \ref{DefinitionBadPartiallyNestedSequence}, we start at \(\mathbf{y}_0:=(\recrankof{\anngvas}, Clean_{\perfectnesssolnospace}, \# \text{ children})\), the rank of the current NGVAS, the name of the current function and an extra component storing the number of remaining iterations of the for loop. The next entry in the sequence is \(\mathbf{x}_1=(\recrankof{\anngvasp}, perf, \dots)\), the rank of the first child, perf and whatever as third part. In terms of Section \ref{SubSubsectionPartiallyNestedSequences}, this is the third type of step: Calling a larger function with an input of lower rank (namely perf is the largest function in our setting). This is followed by a subsequence corresponding to the perf call on \(\recrankof{\anngvasp}\), and at some time step \(t\) we return to \(\mathbf{x}_t:=(\recrankof{\anngvas}, Clean_{\perfectnesssolnospace}, \# \text{children}-1)\), i.e.\ the ``remaining iterations counter'' decreased, and the bad partially nested sequence continues as expected.

In the above toy example, our analysis ``saves'' the remaining iterations counter, in the sense that in Theorem \ref{TheoremLengthBoundBadPartiallyNestedSequences}, we can put this counter into \(\beta_2\), wherefore it is not in the exponent of \(\omega\). 

A better improvement happens in the procedures for checking pumpability as in Section \ref{Section:OutlinePumping}, with the first example being the Karp-Miller-Tree procedure in Section \ref{Section:OutlinePumpingDec}. We apply similar ideas as above: The functions \(KM-tree, reach/breach \in F\) fulfill \(KM-tree>reach/breach\), hence calling reach/breach is in terms of Section \ref{SubSubsectionPartiallyNestedSequences} a call of type 2, calling a smaller function. We again view such calls as atomic, and combine it with a local rank \(\in \N^{2d+3}\) we explain in the following. This allows to save these \(2d+3\) counters with our analysis. 

We first have to explain this tuple. We store configurations as elements of \(\N^{2d+2}\): \(d\) counters for the input vector, \(d\) counters for the output vector and \(2\) counters for storing states as \((i, |Q|-i)\). For every branch of the Karp-Miller-Tree labelled by configurations \(\mathbf{c}_0, \dots, \mathbf{c}_r\) we use \(\N^{2d+2} \setminus \{\mathbf{c}_0, \dots, \mathbf{c}_r\} \uparrow\), the downward-closed set of configurations which may still be added to this branch, as branch-rank. One can view the size of a downward-closed set as an element of \(\N^{2d+2}\) by considering the \emph{type} of the downward-closed set as defined in \cite{FigueiraFSS11}. To define the type, we write a downward-closed set \(\mathbf{D}=\bigcup_{i=1}^r \N^{n_i}\) as a union of sets of the form \(\N^{n_i}\). We then define \(type(\mathbf{D}) \in \N^{2d+2}\), \(type(\mathbf{D})[d']=|\{i \mid n_i=d'\}|\) as the number of parts with a given number \(d'\) of \(\omega\)'s. E.g. \((1, \omega) \downarrow=(0, \omega) \cup (1,\omega)\) has the type \(type((1, \omega) \downarrow)[0]=0, type((1, \omega) \downarrow)[1]=2\) since it consists of two parts with one \(\omega\) each. 

The rank of a Karp-Miller-Tree is then \((\max \text{branch}, \# \text{branches in current round}) \in \N^{2d+3}\), where we take the maximum of the types in the lexicographic ordering, and a round corresponds to the fact that we build Karp-Miller-Trees in a breadth-first-search fashion, i.e.\ in one round we extend every branch by one step. This analysis of Karp-Miller is slightly different than the traditional one, and lends itself better to our complexity analysis using Theorem \ref{TheoremLengthBoundBadPartiallyNestedSequences}. 

Now we can proceed similar to the toy example: Extending a branch requires a reach/breach-call which we view as atomic operation, and then we return from the recursive call to find that the local rank \(\in \N^{2d+3}\) has decreased, since we have either finished another branch in the current round, or at the end decreased the maximal branch. This leads the \(2d+3\) counters storing the branch-rank to be part of \(\beta_2\).

The next procedure in Section \ref{Section:OutlinePumping} are the simple cases for computing reach/breach in Section \ref{Section:OutlineSimpleCases}. There is not much to say here: Using the same ideas as above this is again a tail-recursion with atomic perf calls. The main difference is that sometimes viewing the perf calls as atomic is now justified because \(|\overline{Un}|\) decreased instead of \(\recrankof{\anngvas}\) as above, but the idea remains the same.

While hard case 1 in Section \ref{Section:PostHardCase1} was harder to describe, the complexity is similar: First we compute \(f(r-1)\), which can be viewed as atomic operation since \(|\overline{Un}|\) decreases in these queries. Then we obtain \(Bd\) using some integer linear programming like bounds, i.e.\ exponential bounds. E.g. the size of \(\upseq\) depends at most exponentially on \(f(r-1)\).

Last is hard case 2 in Section \ref{Section:PostHardCase2}, which uses a similar analysis as Karp-Miller. For more details see Section \ref{SectionComplexity}.

==> wide_tree_exp.tex <==
\subsection{Wide Tree Theorem}
A parse tree organizes the application of productions in a tree.
The root is the start non-terminal, the inner nodes are non-terminals, and the yield of the parse tree is the sentential form that has been derived with the productions in the tree.  
We use $\treesof{\agram}$ for the set of all parse trees in $\agram$. 
The link to the derivation relation is 
$\langof{\agram}=\yieldof{\treesof{\agram}}$. 
We use $\paramparikhof{\prods}{\atree}\in\N^{\prods}$ for the productions used in parse tree $\atree$.  
The height of the tree is~$\heightof{\atree}$ and a single node has height $0$.
\rfm{We will have to cross-check off-by-1s.} 

We show a consequence of Theorem~\ref{Theorem:EEK} and Lemma~\ref{Lemma:EEKConverse} that is interesting in its own right.
If we have a strongly connectednon-linear grammar that is  and a solution to the homogeneous variant of Esparza-Euler-Kirchhoff, then we can iterate this solution and obtain parse trees that only grow logarithmically in height.
Actually, we will be more precise, but this needs some terminology.

Consider a parse tree $\atree$ with $\aconst\geq 1$ copies of a production vector $\prodvec\in\N^{\prods}$, meaning $\paramparikhof{\prods}{\atree}=\aconst\cdot \prodvec$. 
We introduce functions that track the provenance of leaves, the copy of $\prodvec$ that generated a given leave. 
Formally, $\prov:\leaves\rightarrow [1, \aconst]$ \emph{tracks provenance}, if $\provinvof{i}=\effof{\terms\discup\nonterms}\cdot \prodvec$ for all $i\in[1, \aconst]$. 
Consider a prefix $\asentform$ of $\yieldof{\atree}$. 
We say that copy $i$ of $\prodvec$ is \emph{complete} in $\asentform$, if $\provinvof{i}\subseteq \asentform$. 
Otherwise, if also the remainder of the yield contains symbols that stem from this copy, we say that copy $i$ is \emph{incomplete} in $\asentform$. 
We will not be interested in the precise copies that are incomplete, but only in their number.
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{theorem}[Wide Tree Theorem] \label{TheoremWideTree}
Let $\agram$ be non-linear, strongly connected, and assume all non-terminals are useful. 
Let $\prodvec\geq 1$ solve $\homeekof{\agram}{\prodvar}$. 
For every $\aconst\geq 1$, there is $\atreedef\in\treesof{\agram}$ with $\paramparikhof{\prods}{\atreedef}= \aconst\cdot \prodvec$ and $\heightof{\atreedef}\leq \ceilof{1 + \log\aconst}\cdot \normof{\avec_{\prods}}$. 
Moreover, $\atreedef$ admits a provenance tracking function so that for every prefix of the yield, the number of incomplete copies of~$\prodvec$ is bounded by $\ceilof{1+\log\aconst}$. 
\end{theorem}
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{proof}
Let us write $\arun$ for terminal sequences.  
For every non-terminal $\anonterm\in\nonterms$, we define the grammar $\agramdef$ that coincides with $\agram$ except that it has $\anonterm$ as the start non-terminal. 
Since all non-terminals are useful in $\agram$ and since $\agram$ is strongly connected, all non-terminals are useful in $\agramdef$. 
Indeed, for $\anontermp\in\nonterms$ we have
\begin{align*}
\anonterm\rightarrow^*\asentform_1.\startnonterm.\asentform_2\rightarrow^*\asentform_1.\asentformp_1\anontermp.\asentformp_2.\asentform_2\rightarrow^*\asentform_1.\arun.\asentform_2\rightarrow^*\arun'\ .
\end{align*}
The first derivation is by strong connectedness. 
The second and third derivations exist, because $\anontermp$ is useful in $\agram $. 
The last derivation uses the fact that from every non-terminal we can derive a terminal sequence, by usefulness in $\agram$. 
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------

We strengthen the statement and show that for every number of copies $\aconst\in\N$ and for every $\anonterm\in\nonterms$, we can obtain a parse tree $\atreeparamdef\in\treesof{\agramdef}$ and a provenance tracking function on $\atreeparamdef$ as promised
The notation $\atreeparamdef$ is meant to indicate that the yield of this tree has the form $\arun_1.\anonterm.\arun_2$ with $\arun_1, \arun_2\in\terms^*$, so $\anonterm$ is the single non-terminal. 
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------

{\bfseries Base case}\quad Let $\aconst=1$ and $\anonterm\in\nonterms$.  
The homogeneous variant of Esparza-Euler-Kirchhoff is independent of the choice of the start non-terminal: the equations are the same for $\agram$ and for $\agramdef$. 
Combined with the remark that all non-terminals are useful in $\agramdef$, we can invoke Theorem~\ref{Theorem:EEK} and obtain $\startnonterm\xrightarrow{\aprodseq}\asentform$ with $\paramparikhof{\prods}{\aprodseq}=\avec_{\prods}$. 
For the shape of the sentential form, Lemma~\ref{Lemma:EEKConverse} 
shows $\paramparikhof{\nonterms}{\asentform}=1_{\anonterm} + \effof{\nonterms}\cdot \avec_{\prods} = 1_{\anonterm}$. 
So $\asentform = \arun_1.\anonterm.\arun_2$ with $\arun_1, \arun_2\in\terms^*$. 
We turn this derivation sequence into a parse tree  $\atreeparam{1}{\anonterm}$. 
The height requirement is trivial and the provenance tracking function maps every symbol in the yield to $1$. 
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------

{\bfseries Step case}\quad Let $\aconst>1$ and consider $\anonterm\in\nonterms$. 
We determine the parse tree $\atreeparam{1}{\anonterm}$ as we have done in the base case.  
Let the yield be $\arun_1.\anonterm.\arun_2$. 
Since the grammar is non-linear and $\avec_{\prods}$ uses every production at least once, $\atreeparam{1}{\anonterm}$ contains a node with at least two children that are non-terminals.
One of these non-terminals may lead to the leaf $\anonterm$. 
The other, however, will lead to a production $\anontermp\rightarrow \arun$ that may add terminals $\arun\in\terms^*$ to $\arun_1$ or $\arun_2$, say $\arun_2$. 
Then the parse tree can be written as $\atreepparam{1}{\anonterm, \anontermp\rightarrow \arun}$.  
We define $\aconst_1=\floorof{\frac{k-1}{2}}$ and $\aconst_2=\ceilof{\frac{k-1}{2}}$ so that $\aconst = \aconst_1+\aconst_2+1$. 
We invoke the induction hypothesis twice, for $\anonterm$ with $\aconst_1$ and for $\anontermp$ with $\aconst_2$.
There is the special case $\aconst_1=0$, in which case we skip the first invokation. 
It yields parse trees $\atreeparam{\aconst-1}{\anonterm}\in \treesof{\agramof{\anonterm}}$ and $\atreeparam{\aconst-1}{\anontermp}\in \treesof{\agramof{\anontermp}}$ that have the properties in the strengthened statement. 
We insert these trees into $\atreepparam{1}{\anonterm, \anontermp\rightarrow \asentformp}$ and obtain
\begin{align*}
\atreeparam{\aconst}{\anonterm}=\atreepparam{1}{\atreeparam{\aconst-1}{\anonterm}, \atreeparam{\aconst-1}{\anontermp\rightarrow \asentformp}}.
\end{align*} 
Note that we moved the production $\anontermp\rightarrow \asentformp$ to the yield of $\atreeparam{\aconst-1}{\anontermp}$. 
So $\atreeparam{\aconst}{\anonterm}$ indeed has $\anonterm$ as the single non-terminal in the yield.
For the number of productions, we note that we have
\begin{align*}
\paramparikhof{\prods}{\atreeparam{\aconst}{\anonterm}}\ & =\ \paramparikhof{\prods}{\atreeparam{1}{\anonterm}}+ \paramparikhof{\prods}{\atreeparam{\aconst-1}{\anonterm}} + \paramparikhof{\prods}{\atreeparam{\aconst-1}{\anontermp}} \\
& =\ \avec_{\prods} + (2^{\aconst-1} -1) \cdot \avec_{\prods} + (2^{\aconst-1}-1)\cdot \avec_{\prods}\\
& =\ (2^{\aconst}-1)\cdot \avec_{\prods}\ .
\end{align*}
The first equation is by the definition of $\atreeparam{\aconst}{\anonterm}$, the second is the induction hypothesis. 
For the height, we argue similarly:
\begin{align*}
\heightof{\atreeparam{\aconst}{\anonterm}}\ & \leq\ \heightof{\atreeparam{1}{\anonterm}}+ \max\set{\heightof{\atreeparam{\aconst-1}{\anonterm}}, \heightof{\atreeparam{\aconst-1}{\anontermp}}} \\
& \leq \ \normof{\avec_{\prods}} + \max\set{(\aconst-1)\cdot \normof{\avec_{\prods}}, (\aconst-1)\cdot \normof{\avec_{\prods}}}\\
& =\ \aconst \cdot \normof{\avec_{\prods}}\ .\qedhere
\end{align*}

\end{proof}

